Parametric Distributionally Robust Optimisation Models for Budgeted Multi-period Newsvendor Problems

In this paper, we consider a static, multi-period newsvendor model under a budget constraint. In the case where the true demand distribution is known, we develop a heuristic algorithm to solve the problem. By comparing this algorithm with off-the-shelf solvers, we show that it generates near-optimal solutions in a short time. We then consider a scenario in which limited information on the demand distribution is available. It is assumed, however, that the true demand distribution lies within some given family of distributions and that samples can be obtained from it. We consider the cases of normal and Poisson demands. For each case, we show that using maximum likelihood estimates in place of the true parameters can lead to poor estimates of the true cost associated with an order quantity. Hence, we make use of likelihood inference to develop confidence sets for the true parameters. These are used as ambiguity sets in a distributionally robust model, where we enforce that the worst-case distribution lies in the same family as the true distribution. We solve these models by discretising the ambiguity set and reformulating them as piecewise linear models. We show that these models quickly become large as the ambiguity set grows, resulting in long computation times. To overcome this, we propose a heuristic cutting surface algorithm that exploits theoretical properties of the objective function to reduce the size of the ambiguity set. We illustrate that our cutting surface algorithm solves orders of magnitude faster than the piecewise linear model, while generating very near-optimal solutions.

==> 2A_LR_notes.tex <==
\section{Literature Review Notes (to be removed)}

Research into non-robust newsvendor problems can be classified into two categories: \textit{non-parametric} and \textit{parametric}. Both methods involve estimating parameters from past data. However, non-parametric approaches do not make any assumption on the family of distributions that the demand distribution lies in. They only make use of such quantities as mean, variance, symmetry and unimodality when creating optimal ordering policies. Parametric approaches make assumptions about the family of distributions and use this information to analyse the performance of the decisions made. Statistical properties of estimators for the parameters of the distributions often allow for probabilistic guarantees that the order quantity suggested by the model is the true order quantity.

Robust and distributionally robust methods also treat the demand distribution as unknown. However, they do not only attempt to approximate the true distribution using data but also to identify the worst-case distribution in some set. Methods from the non-robust literature can be applied to construct a nominal distribution, but this distribution is not treated as truth and is instead used to form an ambiguity set.

\subsection{Parametric Newsvendor Models}

Many authors have considered parametrised demand distributions when studying the Newsvendor problem. One paper studying a parametric newsvendor problem is by~\cite{GALLEGO2007}. They study a problem where the uncertainty in demand is very high, as measured by the coefficient of variation. They first discuss the downfalls of using the normal distribution for cases where this coefficient is large, stating that it can lead to large expected losses in profit. They state that using non-negative distributions such as the negative binomial and gamma distributions can lead to more expected profit. Hence, they analyse the optimal ordering quantities from a number of distributions and compare them. They also compute the solution from the worst-case distribution. Their study shows the normal distribution leading to large expected losses. It shows the lognormal solution making a profit where the normal distribution did not. Finally, it shows that the worst-case distribution leads to a solution with no ordering. This supports the idea that parametric distributions lead to less conservative solutions. In their recommendations, they mention that only using non-negative distributions (i.e.\ not the normal or worst-case) is recommended when there is high variability in demand.

\cite{DOLGUI2008} used parametric distributions for forecasting demand lead-time demand in an inventory system. This paper does not concern a newsvendor problem specifically, but it does discuss the benefits of using a parametric model for demand in an inventory system.  

\cite{ROSSI2014674} also study a newvendor problem under parametric demand distributions. Specifically, they use a confidence-based approach to estimate the optimal ordering quantity when the true demand distribution is not known. They discuss how the maximum likelihood and Bayesian approaches rely on asymptotics, and how this is rarely the case in practice. Their method does not rely on asymptotics, since confidence intervals can be constructed using only a small sample of the true demand. They also suggest that using a non-parametric distribution with its moments set equal to those obtained from the sample leads to conservative solutions. Their method involves using confidence intervals for the parameters of the distribution to produce a range of order quantities. The true quantity is guaranteed to lie in this range with some probability. They also provide upper and lower bounds for the associated expected cost. They apply this methodology to the binomial, Poisson and exponential distributions. 

\cite{Siegel21} also considered a parametric Newsvendor model. The focus of their paper was to use the output of the DRO model to estimate future profits. They listed many reasons as to why one should consider parametric distributions for this purpose. One key reason is that researchers from industry sellers such as Amazon had said that such distributions as Gamma and Lognormal were accurate in forecasting future demands. It is also stated in this paper that the resulting expected profit is larger when a parametric model can be reasonably assumed. This can be assessed using histograms and statistical goodness-of-fit tests. Using parametric distributions also provides a way to efficiently estimate the order quantity using, for example, the maximum likelihood estimator (MLE). This would be done by using the MLEs of the parameters to compute the resulting order quantity. Finally, they mention the benefits of using parametric distributions in evaluating the error of their estimates. This can be done via Bayesian model checking or by generating data from the parametric model.

\subsection{Multi-period Newsvendor Models}

This is a subsection where I take some notes on multi-period newsvendor models to see the solution methods that have been applied. A number of multi-period newsvendor references can be found in the review by~\cite{QIN2011361}. Other papers have been found through references of some of the papers in the following list.
\begin{enumerate}
    \item \cite{Bouakiz92}: this is an early DP approach to a multi-period newsvendor problem. They optimise over the planning period using an exponential utility function. The DP model corresponds to a periodic review model where goods are delivered immediately. This means that orders are made every day and delivered on that day. An order must be made for period $t$ before the demand for day $t$ is realised. The authors assume that the different demand RVs are IID. The model considers backlogging of excess demand. The authors show there is an optimal base-stock policy. This means that the policy just orders enough to bring the stock back to its base level at every time point. \textbf{DP model. No budget constraint.}
    \item \cite{Altintas08}: a paper mainly focussed on setting discounts for selling to a multi-period newsvendor. However, they do consider the optimal ordering policy for the newsvendor itself. The discount is given if the buyer orders above some threshold, and is not given if the order is below. The buyer's problem is treated as a DP again, where the buyer orders once per day and has to balance ordering, holding and penalty costs. They study single-period and infinite horizon models. In the first case the optimal ordering quantity is found to be a \textit{three-index policy} based on computing the optimal order quantities under the two different prices. The infinite horizon model leads to some instances where this is not optimal but it is for many parameter settings. \textbf{DP model. No budget constraint.}
    \item \cite{AHMED2007226}: A paper on extending the classical single-period single-item newsvendor problem to cover cases where the objective is a \textit{coherent risk measure}. Using this type of objective allows for methods for both risk-averse and risk-neutral models to be developed for the same model. They give results on the structure of the optimal order for the single-period problem (but no actual solution?). They treat the multi-period model as a finite-horizon DP, and again present some results on the structure of the optimal solution. \textbf{DP model. No budget constraint.}
    \item \cite{JANAKIRAMAN2013373}: a short paper presenting some new results on the newsvendor problem and the multi-period inventory problem. For the newsvendor problem, they find the best-case expected cost over a set of distributions. The set contains all distributions where the mean and variance are fixed at some value. THey find this cost to be zero. They consider a multi-period inventory model where the demands follow a Poisson process, and find that a dilation ordering of lead times implies an ordering of optimal costs. \textbf{DP, no budget constraint, general inventory models.}
    \item \cite{KIM2015139} (there are some more references here): a multi-period newsvendor problem on a finite horizon that is solved as a multi-stage stochastic program with recourse. They cite that most multi-period newsvendor models are infinite horizon, but that this may not be appropriate for perishable goods because they have a shelf life. They also cite that most multi-period newsvendor models before this one considered stationary demand. This paper is motivated by fashion retailers, where demand is highly non-stationary. Their model is quite a complex program which accounts for multiple retailers, multiple demand scenarios and multiple periods. \textbf{This paper keeps track of inventory in a similar way to our model.} Their inventory level for a given retailer includes the amount ordered in the previous period but not sold, the amount sent to that retailer from other retailers, and subtracts the demand and the amount sent to other retailers. They use a method called \textit{progressive hedging}~\citep{Rockafellar91} to solve their stochastic program. The method is based on scenario decomposition, and attempting to find a scenario independent solution by aggregating the solutions of scenario subproblems. \textbf{Stochastic programming model, inventory tracking but no budget constraint.}
    \item \cite{ZHANG2016143}: a two-product multi-period newvendor where the total demand for the two products is fixed. Each day, the vendor has to decide on how much of each item to order for tomorrow. This paper uses an online learning approach to decide on the order quantities, alongside expert advice. The decision must be made before the daily demand is realised, and afterwards the newsvendor can adjust his decision rule based on the true demand. At the end of the day, the newsvendor's gain is updated using the difference between the total revenue and cost. The authors consider a real-valued and an integer-valued ordering policy. The policies are based on the \textit{Weak Aggregating Algorithm} (WAA)~\cite{KALNISHKAN20081228}. This is an algorithm for aggregating predictions of multiple experts in an online fashion to make a prediction for demand. Each expert is assigned a weight, and after every demand is revealed these weights are updated. The weights reflect the newsvendor's trust in the expert's prediction. The WAA starts with a prior probability distribution over the set of experts, and every iteration it is updated in a Bayesian fashion. The authors use WAA to find an online ordering policy for the newsvendor, assuming that the experts order the same amount every day. They then provide a lower bound on the total profit using the ordering policy. They also test the policies using a number of computational experiments. \textbf{DP model? No budget constraint, fixed total demand.}
    \item \cite{Retsef07}: Another DP model but they do not assume the demand distribution is known. They discuss the base stock policies that are optimal for the case when the distribution is known, in order to show that it relies on knowing the true distribution. They then move to the case where this is not known, but samples can be generated. They develop SAA-like algorithms that develop policies based only on samples of demand. They give a lower bound on the number of samples required to ensure that the cost of the SAA-like solution is arbitrarily close to optimal with high probability. \textbf{DP model but with unknown distributions.}
    \item \cite{Kunnumkal08}: paper on general inventory control problems where base-stock policies are optimal. I.e.\ there exists a base stock level $s$ such that it is optimal to stock back up to $s$ in every period. I.e.\ we always order $\max\{s-x, 0\}$ if the stock level is $x$. It is not always easy to find the value of $s$ for which this policy is optimal. The authors use stochastic approximation to solve for $s$, or $s_t$ for the multiperiod newsvendor. To illustrate this issue, the authors study a multiperiod newsvendor with backlogged demands. The authors construct the MDP model and use approximations for the stochastic gradient of the value function to solve the problem. The model is again, unconstrained \textbf{DP model, no budget constraint.}
    \item \cite{Bensoussan07}: DP model with partially observed demand. Demand is only realised if it is less than the inventory level. If it is larger or equal to the inventory, we only observe that this is the case (not the value itself). Demand is modelled as a Markov process. Note that they assume $0 \le h < c < b$ (this was a condition for our solution to be valid), citing it as ``reasonable''. When the demand or the fact that it is above the inventory level is realised, the demand distribution is updated in a Bayesian-type update step. They prove there is an optimal feedback ordering quantity, and derive some of its properties. When there are finitely many demand values, they explicitly derive a ``near-optimal'' solution. \textbf{DP model, no budget constraint, partially observed demand, Bayesian learning.}
    \item \cite{Deng14}: DP model with service-dependent demand. Demand dynamically updates itself in response to service. For example, customers are less likely to return if they experience a stock-out. The authors study 4 models based on observability of demand distributions. They consider cases where the demand distribution is known, where it is not known but is statistically learned, where the seller can pay to observe it or learn it for free, and when demand data is censored. The last case is similar to~\cite{Bensoussan07} where demand is not observed if it cannot be met. Statistical learning of demand distribution is done in a Bayesian fashion, where the seller holds some belief about the demand distribution and updates it using Bayes theorem whenever demand is realised. They find that all models support the \textit{stockout cost-penalty} approach, i.e.\ penalising stockouts for the seller. \textbf{DP model, unobserved demand, learning demand distribution.} 
\end{enumerate}

This is a lot of papers, and I have not found any that are not DP models. There are more papers that consider DP models, but if we wish to continue with a static model then I don't see much benefit of covering them. Our model comes from the paper by~\cite{CHEN2017}, where the multi-period model is static. The other papers I have found that consider a static multi-period problem are:
\begin{enumerate}
    \item \cite{Mehran19}: a paper that focuses on price-dependent demand and hence setting the price of the item as well as determining optimal order quantities. The authors take a distribution-free approach (mean and variance fixed) and develop inequalities in order to re-write the objective as a function of the means and variances. There are no constraints on this model but it is a static model, and it includes a discount that is offered for leftover items at the end of the planning period. The solution is obtained using derivatives alone. \textbf{Multi-period static model with no budget constraint but decides pricing as well.}
    \item \cite{ZHANG2019117} (there are some references in this one): a multi-product, multi-period static NV which is formulated as a MINLP. Lagrangian relaxations are used to develop a strong heuristic for this problem. Demand distributions known, one for each period and each product. Model has a budget constraint. The budget constraint is relaxed using the Lagrange method and then subproblems are created for this new problem. There is one subproblem relating to the total order quantity and another related to the individual order quantities. The suppliers all provide ``unit quantity discounts'', where a discount is given according to how much is bought. The method that the authors use to solve it is a subgradient method. It entails:
    \begin{enumerate}
        \item Solving the independent subproblems relating to the days and items.
        \item Using objective value to update upper and lower bounds.
        \item Calculating a stepsize, which is defined based on the objective value and lower bound. 
        \item Update the Lagrange multipliers based on the stepsize and the difference between the amount spent and the budget for each period/item.
    \end{enumerate}
    This is repeated until the Lagrange multipliers barely change, or the maximum number of iterations is reached. In this problem, the order quantity for each period and item $Q_{it}$ is the total amount ordered of product $i$ up to period $t$. This makes it a cumulative order quantity and hence there is no summation of orders for different periods in the objective. The inventory seems to be kept track of through this cumulative order quantity. The result is that the order quantities obtained from setting derivatives equal to zero is just obtained from one inverse CDF (not the difference of two), which seems to eliminate the potential for negative solutions.  However, when calculating the individual order quantities for each period based on the optimal $Q$ solution (i.e.\ $q_t = Q_{t} - Q_{t-1}$), we may get negative values. The authors present a simple feasibility algorithm that essentially sets $q_t = 0$ if $Q_t - Q_{t-1} < 0$. It also increases some values if the used budget is less than the maximum and reduces them if it's above. \textbf{This algorithm could easily be adapted to our problem. We could use it as a baseline.}
\end{enumerate}

It seems as though the results of~\cite{Mehran19} may provide a baseline algorithm for solving our problem. This paper references the following MPNVP papers:
\begin{enumerate}
    \item \cite{MATSUYAMA2006170}: a multi-period newsvendor model with holding and backlog costs. Planning period is split into multiple ordering cycles in which orders must be made. It seems as though a cycle represents a period. They formulate the problem as deciding how much inventory to start a cycle with, and at the end of each cycle the inventory is replenished back to this level. They present a number of theorems and proofs to establish properties of the expected profit. \textbf{Hard to read, but it is a static problem with no budget constraint.}
    \item \cite{Bensoussan07}: already covered.
    \item \cite{Bisi11}: Multiperiod inventory problem with demand above the current stock level censored. Bayesian learning procedure employed to update demand distribution estimates at every iteration. They discuss a number of parametric demand distributions and find that Weibull is the only one that leads to a closed form optimal solution. \textbf{I think it's an MDP model but no access so can't tell.}
    \item \cite{XuMyopic}: Capacitated multi-period inventory problem (general, not only newsvendor). They present conditions on a myopic policy being optimal. \textbf{Cannot get access but might be useful.}
\end{enumerate}

\subsection{Distributionally Robust Newsvendor Models}

\textit{This is just some initial thoughts upon reading some papers.}

It was shown in~\cite{oneperiodrobustsol} that if the ambiguity set contains
only distributions with their means and variances fixed at some known values,
then the distributionally robust solution has a closed form, written in terms of
the model and distribution parameters. Of course, this solution is only max-min
optimal if this is the true mean and variance of demand. It also does not give
the worst-case distribution, only the amount to be ordered.
\cite{gallego_extensions} extended this model in multiple ways, including to the
multi-period and multi-item cases, and cases with random yield.
\cite{asymmetry_DRNV} extend the model to account for second-order partioned
statistics that describe asymmetry, as well as mean and variance.
\cite{DR_Multimodal} considered a multi-item DRNVP with an ambiguity set
consisting of all distributions that were multimodal, and did not assume that
the mean and variance were known. They solved this model using quadratic
decision rules. \cite{DR_variationdistance} considered a single-period,
single-item DRNVP where the ambiguity set is defined using all distributions
that are less than some distance away from a nominal distribution. They focus on
characterising the optimal solution and on the relationship the DRNVP has with
risk aversion and stochastic programming. \cite{Likelihood_RNVP} considered a
version of the problem where the ambiguity set contained all distributions that
achieved a certain level of likelihood given a set of observed demand data.

\large{\textbf{Notes on Papers}}

Firstly, there are a lot of papers on the distribution-free Newsvendor. This is where we assume the mean and variance of demand are fixed and find the minimum worst-case expected cost over all distributions with this mean and variance.
\begin{itemize}
    \item \cite{ALFARES2005465}: Extension of classical DRNVP model to account for shortage cost. Early models did not penalise for unmet demand. Similar to~\cite{gallego_extensions}, they study the distribution free newsvendor model. This refers to the mean and variance of demand being known but not the distribution itself. They model the single product case, the fixed ordering cost case (fixed cost regardless of order size), the random yield case (orders may include defective items, i.e. not everything that is ordered is saleable), and the resource-constrained multi-product case (similar to our model but with multiple items not days). They present optimal solutions in all cases. The multi-product case is solved using Lagrange multipliers. They present an algorithm for solving this model based on iteratively increasing the Lagrange multiplier. Worst-case profit is not given but a lower bound on it is. 
    \item \cite{DF_balking}: a single-period, single-item, distribution-free model with Balking. Balking is where customers decide not to buy an item, typically when stock gets low. Worst case ordering cost found using derivatives. 
    \item \cite{OUYANG20021}: Distribution free model with additional uncertainty in the lost-sales/backorder rate. They incorporate this using fuzzy sets. Before this, they state that typically a fixed fraction of demand is backordered. This paper does not treat this fraction as fixed. They also incorporate variable lead times into their model. They use KKT conditions for their model and present a solution algorithm, involving finding a solution for each lead time and then finding the worst-case for each solution.
    \item \cite{Lan15}: Another distribution-free model with Balking. This time there is a Balking cost, i.e.\ newsvendor pays a cost for each unit that is not sold due to Balking. They incorporate this in the single product and random yield models. It is essentially incorporating a linear cost for lost sales due to balking. They give an equation that must be solved for the optimal order quantity, but it doesn't seem as though they actually provide the value. They again solve using derivatives. An algorithm for solving the equation is presented.  
    \item \cite{Lee11Advertising}: Another distribution-free model. This time they study the effects of advertising. They treat the mean and variance of demand as functions of advertising expenditure. The demand is assumed to be an increasing and concave function of advertising expenditure. They studied three cases based on varying the behaviour of the coefficient of variation and the variance (constant variance, constant coefficient of variation, increasing coefficient of variation). They provide closed-form solutions for optimal advertising expenditure and ordering quantities. 
    \item \cite{AverseNV}: Distribution-free model studied under the risk-averse and ambiguity-averse context. Ambiguity-averse corresponds to the mean and variance being the only parts of the distribution of demand that are known. The risk-averse context refers to there being a risk component in the objective, which means the worst-case expected cost is adjusted according to the risk involved with the distribution selected. The authors provided a closed-form solution which is an extension of that of~\cite{oneperiodrobustsol}.
    \item \cite{LiuCarbon}: Another DF model which considers carbon emissions. Problem considers Independent Remanufacturers (IRs), which remanufacture recycled products/components/parts. They provide a model that maximises profit under 3 different trade policies (a) mandatory carbon emissions capacity, (b) carbon tax and (c) cap and trade. The models include various different costs, including holding cost, disposal cost, remanufacturing cost and carbon emission cost. The idea is to see how the three trade policies affect remanufacturing decision making. The paper seems very applied and more about the resulting decisions than contributing to theoretical literature.
    \item \cite{BAI20162}: Distribution-free model with dual sourcing. Single period, single item. Dual sourcing means that the newsvendor has two suppliers they can order from, and that emergency orders can be placed to make up unmet demand in high season. Suppliers modelled as onshore and offshore suppliers. Offshore is cheaper and slower, onshore is fast and expensive. Carbon emissions are modelled, with a different value for the first, second and emergency orders. They study 3 different models based on dual sourcing with and without carbon emissions under different trade laws on the emissions. They find closed form solutions to these problems, presented the order quantity and the worst-case cost.
\end{itemize}
Based on the above papers, there is a massive literature on the distribution-free newsvendor model. This is to say that authors seem to always assume that the mean and variance are known. They can typically derive optimal solutions to these problems using KKT conditions/derivatives. We need to continue reviewing literature to find examples of problems that are more similar to ours.  

There are some papers that take a slightly different approach. They still assume that the mean and variance are fixed but they apply a min-max regret or maximum entropy approach.
\begin{itemize}
    \item \cite{YueInformation}: DF newsvendor where they aim to maximise the Expected Value of Distributional Information (EVDI) over all distributions with a fixed mean and variance. I can't get access to this paper, but it seems to me that the EVDI is the expected gain from knowing the true distribution compared with the distribution being considered. Minimising the maximum EVDI would then be making the decision that would gain the least from knowing the full distribution in the worst-case. They provide a procedure for solving the problem.
    \item \cite{PerakisRegret}: DF problem where more than just mean and variance are known. They give symmetry and unimodality as other options for information. They derive order quantities that minimise the maximum regret from not acting optimally, i.e.\ the maximum over all potential distributions. They state that ``most'' of their solutions are tractable. They find that distributions maximising entropy perform well under the regret objective. This problem is designed to give robust solutions that are not conservative. 
    \item \cite{ZhuLimitedInformation}: DF newsvendor where they minimise the maximum regret for a given solution, which is the ratio of the cost based on limited information and the cost associated with complete information. This clearly attempts to try to create a model that gives solutions that are as close as possible to those from the full information case, while still not knowing the true distribution. The authors provide a procedure for deriving the optimal solution. 
    \item \cite{ANDERSSON2013}: DF newsvendor where the authors minimise maximum entropy. Entropy is the average level of ``surprise'' or ``uncertainty'' in the distribution. For example, the entropy of a distribution which only gives non-negative values to the very largest demands will have very low entropy, as nothing that happens can be much of a surprise. Minimising the maximum entropy therefore means that the resulting decision will be less conservative, because less extreme values must also be possible as well as those very large ones. The decision will not simply protect against the extreme demands but be robust against all possible values. 
\end{itemize}

For distance-based ambiguity sets (not fixed mean and variance), there is not so much literature. The following will be based on the literature review by~\cite{DR_variationdistance}.
\begin{itemize}
    \item They cite some of the above papers relating to the distribution free model, where some parameters of the distribution are fixed. 
    \item \cite{zhao2015data}: Another paper referring to a DRO model as a ``risk-averse stochastic program with distributional ambiguity''. They construct their ambiguity sets based on $\zeta$-structure probability metrics. This is a class of metrics such as the Kantorovich metric, Fortet-Mourier metric, Total Variation metric, Bounded Lipschitz metric, and Kolmogorov/Uniform metric. For two distributions $P, Q$, the $\zeta$-structure metric is defined as:
    \begin{equation}
        d_{\zeta}(P, Q) = \sup_{h \in \m{H}} \Big|\int_{\Omega} h \text{d}P - \int_{\Omega} h \text{d}Q \Big|.
    \end{equation}
    where $\Omega$ is the support of $P$ and $Q$, and $\m{H}$ is a family of real-valued bounded measurable functions on $\Omega$. So it is the maximum absolute difference between $\E_P(h(\omega))$ and $\E_Q(h(\omega))$. The Wasserstein distance is one such metric. For discrete distributions they are able to reformulate the problem as a stochastic program. For continuous distributions they present a sampling algorithm that repeatedly samples upper and lower bounds on the cost. They prove that these bounds converge to the optimal objective value.
    \item \cite{Likelihood_RNVP}: a paper cited in the first part of the literature review. They consider a ``likelihood robust'' newsvendor, which is a DRNVP where the ambiguity set consists of all distributions under which the observed data has at least some minimum level of likelihood. The result is quite a simply DRO model with a likelihood constraint, that they then solve by dualising the inner model as is expected. They cited the reasons for the likelihood method as being that the mean and variance are not usually known exactly, and that the worst-case distribution is not usually specifiable based on just the mean and variance. They suggest that only using the mean and variance leads to solutions that are more conservative and less realistic.
    \item \cite{JiangRiskAverse}: they consider ``risk-averse two-stage stochastic programs with distributional ambiguity'' (which just sounds like a DRO model). Among other problems, they consider a risk averse NV, where the ambiguity set is defined based on the $L^1$ distance from a nominal distribution. They include a theorem that allows them to rewrite the worst-case cost for a fixed decision using CVaR and the essential supremum of a cost function. They apply this theorem to solve the one period model to optimality, when the nominal distribution is absolutely continuous. The solution is found using the inverse CDF of the nominal distribution. They use the three-sigma rule to estimate the support for demand and use a kernel density estimate based on samples to estimate the true distribution. This may be useful when we decide how to test our methods.
    \item \cite{BertsimasRSAA}: This paper studies a robust version of sample average approximation (SAA), for solving stochastic programs. SAA is a common method for dealing with uncertainty in optimisation where we replace uncertain parameters with the average obtained from a sample. SAA has strong asymptotic guarantees but such guarantees do not usually hold for small samples. Robust SAA is designed to retain the asymptotic guarantees while also providing finite-sample performance guarantees. The authors propose RSAA as approximating the stochastic program by a data-driven DRO model. They use ambiguity sets that constrain the parameters of the distributions to be close to the sample estimates. They mention that this can then be used to form a confidence set in which the true distribution lies with some probabilistic guarantee. They define this as the set of distributions which pass a goodness-of-fit test. They study single-item and multi-item newsvendor problems, showing how their methodology applies. They compare with SAA, 2-SAA and the DRO bound from the fixed mean and variance model. They study normal, Gumbel and mixture distributions, all both bounded and unbounded. The goodness of fit test is the Kolmogorov-Smirnov test, meaning they used the KS distance.
    \item \cite{gao2017distributionally}: a more general paper on DRO with Wasserstein distance ambiguity sets. They study a single-period single-item newsvendor problem and compare the results from using a Wasserstein distance metric with those from using a $\phi$-divergence. They obtain a convex-programming reformulation using the Wasserstein distance. They use results from DRO for $\phi$ divergences to find the worst-case for this case. They only consider distributions with bounded and discrete support in this paper. 
    \item \cite{EsfahaniWasserstein}: General paper on DRO with Wasserstein ambiguity sets, concerning performance guarantees and reformulations in particular. They show that many Wasserstein DRO models can be reformulated as convex programs and sometimes even linear programs. They discuss a DRNVP with a Wasserstein distance of order 1. 
    \item \cite{DRNV_Wasserstein}: a recent paper on a data-driven single-period single-item DRNVP with a Wasserstein distance ambiguity set. For the Wasserstein distance of order 1, they derive the optimal solution using duality properties to evaluate the objective of the inner problem, similarly to how we solve a $\phi$-divergence model. They find that the DRO solution is the solution resulting from the SAA approach. They provide a tractable reformulation that can be used to obtain the optimal solution in the case of the order being larger than 1. They study the risk-neutral newsvendor, which has a standard expected cost objective. They also study a risk-averse newsvendor, who aims to minimise the maximum CVaR. They cite the reason for using DRO instead of DF newsvendor is that it may not be realistic to have enough data to make the required estimates for DF. They also state that using inaccurate estimates of the parameters of demand distribution can lead to highly suboptimal solutions. Further reasons include DF problems abandoning other information such as shape of distribution, and also DF models leading to overly conservative solutions (they cite~\cite{Likelihood_RNVP} for this). They mention the benefit of DRO being the use of statistical distances to ensure closeness to the nominal distribution. However, they mention that using $\phi$-divergences does not always include all distributions that we would like to include. This is because all distributions in the resulting set must have the same support as the empirical (nominal) distribution. Hence, if we use an empirical estimate of a distribution and we do not sample all potential values, then our ambiguity set cannot contain the true distribution. This applies also to taking a discrete empirical estimate of a continuous distribution. 
\end{itemize}



==> A_fixed_dist_old.tex <==
\section{Solution for a Fixed, Continuous Distribution}

The model for a fixed distribution $F$ is referred to as MPNVP:
\begin{equation}
    (\text{MPNVP}) \quad
    \begin{cases}
        \min_{\bm{q}}C_{F}(\bm{q}) &= p\E_{F}[I^-_T] + 
    \sum_{t=1}^T \l(h\E_{F}[I^+_t] + b\E_{F}[I^-_t] + w_t q_t
    - p \E_F[X_t]\r) \\
    \sum_{t=1}^T w_t q_t &\le W, \\
    I_t &= I_{t-1} + q_t - X_t \fa t = 1, \dots, T, \\
    q_t &\ge 0 \fa t = 1,\dots,T.
    \end{cases}
\end{equation}
In order to develop a solution algorithm for this problem, we will now assume that $F$ represents a continous distribution. This allows us to use the KKT conditions to derive an algorithm. Despite this assumption, however, the algorithm we develop can also be applied to discrete distributions, and we will show that it performs well for both the Poisson and normal distributions.

\subsection{Derivatives of Objective}

Firstly, note that we have:
\begin{align}
    \E_F\l[I_t^+\r] &= \E_F\l[\max(I_t, 0)\r] \\
    &= \P(I_t \ge 0)\E_F(I_t | I_t \ge 0) \\
    &= \tilde{F}_t\l(\sum_{k=1}^t q_k\r)\l[\sum_{k=1}^t q_k - \E_{\tilde{F}_t}\l(\sum_{k=1}^t X_k \Bigg| \sum_{k=1}^t X_k \le \sum_{k=1}^t q_k\r)\r]
    % &= \P\l(\sum_{k=1}^t X_k \le \sum_{k=1}^t q_k\r)\l[\sum_{k=1}^t q_k - \E_F\l(\sum_{k=1}^t X_t \bigg| \sum_{k=1}^t X_k \le \sum_{k=1}^t q_k\r)\r]\\
    % &= \tilde{F}_t\l(\sum_{k=1}^t q_k\r)\l[\sum_{k=1}^t q_k - \frac{\int_0^{\sum_{k=1}^t q_k} x\tilde{f}_t(x) \text{d}x}{\tilde{F}_t\l(\sum_{k=1}^t q_k\r)}\r]\\
    % &= \tilde{F}_t\l(\sum_{k=1}^t q_k\r)\sum_{k=1}^t q_k - \int_0^{\sum_{k=1}^t q_k} x\tilde{f}_t(x) \text{d}x.
\end{align}
where $\tilde{F}_t$ and $\tilde{f}_t$ are the CDF and PDF of $\sum_{k=1}^t X_t$. 
Now note that we have:
\begin{equation}
    \pderiv{\tilde{F}_t\l(\sum_{k=1}^t q_k\r)}{q_j} = \begin{cases}
        \tilde{f}_t\l(\sum_{k=1}^t q_k\r) &\text{ if } j \le t,\\
        0 &\text{ otherwise}
    \end{cases}.%\\
    % \pderiv{\E_{\tilde{F}_t}\l(\sum_{k=1}^t X_k \Bigg| \sum_{k=1}^t X_k \le \sum_{k=1}^t q_k\r)}{q_j} &= \begin{cases}
    %     something &\text{ if } j \le t,\\
    %     0 &\text{ otherwise.}
    % \end{cases}
\end{equation}

To differentiate the expected values we need that:
\begin{equation}
    \E_{\tilde{F}_t}\l(\sum_{k=1}^t X_k \Bigg| \sum_{k=1}^t X_k \le \sum_{k=1}^t q_k\r) = \frac{\int_{-\infty}^{\sum_{k=1}^t q_k} u\tilde{f}_t(u) \text{d}u}{\tilde{F}_t\l(\sum_{k=1}^t q_k\r)}
\end{equation}
which means that:
\begin{align}
    \E_F[I^+_t] &= \tilde{F}_t\l(\sum_{k=1}^t q_k\r)\l[\sum_{k=1}^t q_k - \frac{\int_{-\infty}^{\sum_{k=1}^t q_k} u\tilde{f}_t(u) \text{d}u}{\tilde{F}_t\l(\sum_{k=1}^t q_k\r)}\r]\\
    &= \tilde{F}_t\l(\sum_{k=1}^t q_k\r)\sum_{k=1}^t q_k - \int_{-\infty}^{\sum_{k=1}^t q_k} u\tilde{f}_t(u) \text{d}u.
\end{align}
Applying the second fundamental theorem of calculus (derivative of indefinite integral) and the chain rule we get that:
\begin{align}
    \pderiv{}{q_j}\int_{-\infty}^{\sum_{k=1}^t q_k} u\tilde{f}_t(u) \text{d}u &= \pderiv{}{q_j}\l(\l[\int u\tilde{f}_t(u) \text{d}u\r]\Bigg|_{u=\sum_{k=1}^t q_k} -  \lim_{v\to-\infty}\l[\int u\tilde{f}_t(u) \text{d}u\r]\Bigg|_{u=v}\r) \\
    &= \pderiv{}{q_j}\l[\int u\tilde{f}_t(u) \text{d}u\r]\Bigg|_{u=\sum_{k=1}^t q_k}\\
    &=\l(\sum_{k=1}^t q_k \times \tilde{f}_t\l(\sum_{k=1}^t q_k\r)\r) \times \pderiv{}{q_j}\sum_{k=1}^t q_k \\
    &= \sum_{k=1}^t q_k \times \tilde{f}_t\l(\sum_{k=1}^t q_k\r)
\end{align}
for $j \le t$ and 0 otherwise. Therefore:
\begin{align}
    \pderiv{}{q_j}\E_F[I^+_t] &= \tilde{f}_t\l(\sum_{k=1}^t q_k\r) \sum_{k=1}^t q_k + \tilde{F}_t\l(\sum_{k=1}^t q_k\r) - \tilde{f}_t\l(\sum_{k=1}^t q_k\r) \sum_{k=1}^t q_k \\
    &= \tilde{F}_t\l(\sum_{k=1}^t q_k\r).
\end{align}

Similarly, we have:
\begin{align}
    \E_F\l[I_t^-\r] &= \E_F\l[\max(-I_t, 0)\r] \\
    &= \P(-I_t \ge 0)\E_F(-I_t | -I_t \ge 0) \\
    &= -\P(I_t \le 0)\E_F(I_t | I_t \le 0) \\
    &= -\l(1 - \tilde{F}_t\l(\sum_{k=1}^t q_k\r)\r)\l[\sum_{k=1}^t q_k - \E_{\tilde{F}_t}\l(\sum_{k=1}^t X_k \Bigg| \sum_{k=1}^t X_k \ge \sum_{k=1}^t q_k\r)\r]\\
    &= -\l(1 - \tilde{F}_t\l(\sum_{k=1}^t q_k\r)\r)\l[\sum_{k=1}^t q_k - \frac{\int_{\sum_{k=1}^t q_k}^\infty u\tilde{f}_t(u) \text{d}u}{1-\tilde{F}_t\l(\sum_{k=1}^t q_k\r)}\r] \\
    % &= \l(1 - \tilde{F}_t\l(\sum_{k=1}^t q_k\r)\r)\l[\sum_{k=1}^t q_k - \frac{\int_{\sum_{k=1}^t q_k}^\infty x\tilde{f}_t(x) \text{d}x}{1-\tilde{F}_t\l(\sum_{k=1}^t q_k\r)}\r]\\
    % &= \l(1-\tilde{F}_t\l(\sum_{k=1}^t q_k\r)\r)\sum_{k=1}^t q_k - \int_{\sum_{k=1}^t q_k}^\infty x\tilde{f}_t(x) \text{d}x.
    &= \l(\tilde{F}_t\l(\sum_{k=1}^t q_k\r) - 1\r)\sum_{k=1}^t q_k + \int_{\sum_{k=1}^t q_k}^\infty u\tilde{f}_t(u) \text{d}u.
\end{align}
Applying the same calculus as before, we find:
\begin{align}
    \pderiv{}{q_j}\int_{\sum_{k=1}^t q_k}^\infty u\tilde{f}_t(u) \text{d}u &=  \pderiv{}{q_j}\l(\int_{\sum_{k=1}^t q_k}^\infty u\tilde{f}_t(u) \text{d}u\r) \\
    &= - \pderiv{}{q_j}\l[\int u\tilde{f}_t(u) \text{d}u\r]\Bigg|_{u=\sum_{k=1}^t q_k} \\
    &= - \sum_{k=1}^t q_k \times \tilde{f}_t\l(\sum_{k=1}^t q_k\r).
\end{align}
Hence:
\begin{align}
    \pderiv{}{q_j} \E_F[I^-_t] &= \tilde{f}_t\l(\sum_{k=1}^t q_k\r)\sum_{k=1}^t q_k + \l(\tilde{F}_t\l(\sum_{k=1}^t q_k\r) - 1\r) - \sum_{k=1}^t q_k\times \tilde{f}_t\l(\sum_{k=1}^t q_k\r)\\
    &= \tilde{F}_t\l(\sum_{k=1}^t q_k\r) - 1
\end{align}
for $j \le t$, 0 otherwise. Hence, we have:
\begin{align}
    \pderiv{}{q_j} C_F(\bm{q}) &= p\l(\tilde{F}_T\l(\sum_{k=1}^T q_k\r) - 1\r) + \sum_{t=j}^T\l[(h + b)\tilde{F}_t\l(\sum_{k=1}^t q_k\r) - b\r] + w_j \\
    &= \sum_{t=j}^T\l[(h + b + p\mathds{1}\{t=T\})\tilde{F}_t\l(\sum_{k=1}^t q_k\r) - b\r] + w_j - p
\end{align}

\subsection{Lagrangian and KKT Conditions}

The Lagrangian of MPNVP without considering the non-negativity constraints is:
\begin{equation}
    L(\bm{q}, \lambda) = C_F(\bm{q}) + \lambda \l(\sum_{t=1}^T w_t q_t - W\r).
\end{equation}
The KKT conditions are therefore:
\begin{align}
    \pderiv{}{q_j} C_F(\bm{q}^*) + \lambda w_j &= 0 \fa j = 1,\dots,T,\label{eq:KKT_deriv}\\
    \sum_{t=1}^T w_t q^*_t &\le W \label{eq:KKT_cap}, \\
    \lambda\l(\sum_{t=1}^T w_t q^*_t - W\r) &= 0 \label{eq:KKT_lam0}, \\
    \lambda &\ge 0 \label{eq:KKT_lam_nonneg}%\\
    %q^*_1,\dots,q^*_T &\ge 0. \label{eq:KKT_q_nonneg}
\end{align}
We can find a solution to~\eqref{eq:KKT_deriv} by setting:
\begin{equation}\label{eq:KKT_sol}
\l.\begin{aligned}
        q^*_1 &= \tilde{F}^{-1}_1\l(\frac{b - (1+\lambda)(w_1 - w_2)}{h+b}\r)\\
        q^*_t &= \tilde{F}^{-1}_t\l(\frac{b - (1+\lambda)(w_t - w_{t+1})}{h+b}\r) - \tilde{F}^{-1}_{t-1}\l(\frac{b - (1+\lambda)(w_{t-1} - w_{t})}{h+b}\r) \fa t \in \{2,\dots, T-1\}\\
        q^*_T &=  \tilde{F}^{-1}_T\l(\frac{b - (1+\lambda)w_T + p }{h+b+p}\r) - \tilde{F}^{-1}_{T-1}\l(\frac{b - (1+\lambda)(w_{T-1} - w_{T})}{{h+b}}\r).
    \end{aligned}
    \r\}
\end{equation}
Then we have:
\begin{equation}\label{eq:sum_of_qs}
    \sum_{k=1}^t q^*_k = \begin{cases}
        \tilde{F}^{-1}_t\l(\frac{b - (1+\lambda)(w_t - w_{t+1})}{h+b}\r) &\text{ if } t < T,\\
        \tilde{F}^{-1}_T\l(\frac{b - (1+\lambda)w_T + p}{h+b+p}\r) &\text{ if } t= T.
    \end{cases}
\end{equation}
this means that adjusting $\lambda$ adjusts every solution not just the final order quantity. Plugging~\eqref{eq:KKT_sol} in to the Lagrangian's derivative, we get:
\begin{align*}
    \pderiv{}{q_j} L(\bm{q}, \bm{\lambda}) =& \sum_{t=j}^{T-1} \l[b - (1+\lambda)(w_t - w_{t+1})- b\r] + \l[b - (1+\lambda)w_T + p - b\r] - p + (1+\lambda)w_j\\
    =&\ \sum_{t=j}^{T-1}\l[(1+\lambda)(w_{t+1} - w_t )\r]  - (1+\lambda)w_T + (1+\lambda)w_j  \\
    =& \  (1+\lambda)(w_T - w_j) - (1+\lambda)(w_T - w_j)\\
    =& \ 0.
\end{align*}
For our solution to be valid, we require:
\begin{align}
    \frac{b - (1+\lambda)(w_t - w_{t+1})}{h+b} &\le 1 \\
    \implies \lambda &\ge \frac{-h}{w_t - w_{t+1}} - 1 \fa t \in \{1,\dots,T-1\},  
\end{align}
and 
\begin{align}
    \frac{b - (1+\lambda)(w_t - w_{t+1})}{h+b} &\le 0 \\
    \implies \lambda &\le \frac{b}{w_t - w_{t+1}} - 1 \fa t \in \{1,\dots,T-1\}. \label{eq:lam1} 
\end{align}
For the final day, we require:
\begin{align}
    \lambda & \ge -\frac{h}{w_T} - 1,\\
    \lambda & \le \frac{b+p}{w_T} - 1 \label{eq:lam2}.
\end{align}
If we assume that $w_t \ge w_{t+1} \fa t$ then we simply require~\eqref{eq:lam1} and~\eqref{eq:lam2}.

% \subsection{An Alternate Solution Formula}

% The solution in~\eqref{eq:KKT_sol} corresponds to making all adjustments for the budget constraint in the final day's order. This may not work in practice, since it may not be possible to meet the budget constraint only by reducing the final day's order. Suppose that, for a given $\lambda$ we select $\lambda_1,\lambda_2,\dots,\lambda_T$ such that $\sum_{t=1}^T \lambda_t = \lambda$. Then, we can define a new solution via:

% \begin{equation}\label{eq:KKT_sol_adj}
% \l.\begin{aligned}
%         q^*_1 &= \tilde{F}^{-1}_1\l(\frac{b + (\lambda_1 - \lambda_2) -(w_1 - w_2)}{h+b}\r)\\
%         q^*_t &= \tilde{F}^{-1}_t\l(\frac{b + (\lambda_t - \lambda_{t+1}) - (w_t - w_{t+1})}{h+b}\r) - \tilde{F}^{-1}_{t-1}\l(\frac{b + (\lambda_{t-1} - \lambda_{t}) - (w_{t-1} - w_{t})}{h+b}\r) \fa t \in \{2,\dots, T-1\}\\
%         q^*_T &=  \tilde{F}^{-1}_T\l(\frac{b +(\lambda_T - \lambda)  - w_T + p }{h+b+p}\r) - \tilde{F}^{-1}_{T-1}\l(\frac{b + (\lambda_{T-1} - \lambda_{T}) - (w_{T-1} - w_{T})}{{h+b}}\r).
%     \end{aligned}
%     \r\}
% \end{equation}
% Then we have:
% \begin{equation}\label{eq:sum_of_qs_adj}
%     \sum_{k=1}^t q^*_k = \begin{cases}
%         \tilde{F}^{-1}_t\l(\frac{b + (\lambda_{t} - \lambda_{t+1})  - (w_t - w_{t+1})}{h+b}\r) &\text{ if } t < T,\\
%         \tilde{F}^{-1}_T\l(\frac{b +(\lambda_T - \lambda) - w_T + p}{h+b+p}\r) &\text{ if } t= T.
%     \end{cases}
% \end{equation}
% Therefore, we have:
% \begin{align*}
%     \pderiv{}{q_j} L(\bm{q}, \bm{\lambda}) =& \sum_{t=j}^{T-1} \l[b - \lambda_t - (w_t - w_{t+1})- b\r] + \l[b - \lambda_T - w_T + p - b\r] + w_j - p + \lambda\\
%     =&\ \sum_{t=j}^{T-1}\l[(w_{t+1} - w_t )\r]  - w_T + w_j + \lambda - \sum_{t=1}^T \lambda_t \\
%     =& \ 0.
% \end{align*}


\subsection{Papers on Iterative Solution Algorithms}

We cannot guarantee that the solution in~\eqref{eq:KKT_sol} satisfies the budget constraint and the non-negativity constraints. \cite{ALFARES2005465} have a similar issue, and they present an algorithm for solving their model which sets orders to zero if they have a negative term in the objective. They then iteratively increase $\lambda$ until either one of their orders becomes negative or the solution becomes feasible. If an order becomes negative, they fix it at zero and start again. This is similar to the work that is done by~\cite{ABDELMALEK2005296}, who also study a multi-product newsvendor problem with a budget constraint. They cite the motivation for their research being that relaxing non-negativity constraints can lead to infeasible solutions when solving using the KKT methods. The motivation comes from~\cite{Lau1996TheNP}, who found this in their numerical examples.

The method given by~\cite{ABDELMALEK2005296} consists of dividing the solution space into three regions based on the tightness of the budget constraint. Each region warrants a different solution method. The three regions are as follows:
\begin{enumerate}
    \item The budget is large and the solution is the same as the unconstrained problem.  In this case we can solve by solving the KKT conditions with no non-negativity constraints and no budget constraints.
    \item The budget is medium and the constraint is binding, however there are not any negative orders. This can be solved without the non-negativity constraints.
    \item The budget is very tight and if the non-negativity constraints are relaxed negative order quantities may be obtained, and therefore some products have to be deleted from the original list. 
\end{enumerate}
The budget thresholds are defined as follows. Let $B_1$ be the budget below which implies that non-negativity constraints must be imposed. Let $B_2$ be the budget below which the budget constraint must be imposed. The larger budget, $B_2$ is found from solving the problem unconstrained and calculating the amount spent. In our model, this would be:
\begin{equation}
    B_2 = \sum_{t=1}^T w_t q^*_t(0),
\end{equation}
where $q^*_t(\Lambda)$ is the value of $q^*_t$ obtained by evaluating the KKT solution with $\lambda = \Lambda$. The logic here is that if the budget is larger than this then the unconstrained optimum (i.e.\ $q^*$ with $\lambda = 0$) meets the budget constraint and hence is optimal for the constrained problem. 

The definition of $B_1$ is a bit more complex. The first step is to find the smallest $\lambda$ such that $q^*_t(\lambda) \ge 0$ holds, for each $t$. Call this value $\lambda_t$. This can be obtained by simply rearranging the inequality $q^*_t(\lambda_t) \ge 0$ in the multi-product case. Then we take $\lambda^- = \min_{t} \lambda_t$ as the largest $\lambda$ such that all orders remain non-negative. Then we take the lower budget as:
\begin{equation}
    B_1 = \sum_{t=1}^T w_t q^*_t(\lambda^-).
\end{equation}
If our budget is above this threshold then the newsvendor can make order all items without exceeding the budget. There is no need to make any negative orders. However, if the budget is below $B_1$ then this $\lambda$ cannot be selected and a larger one must be chosen. This leads to at least one order being negative and hence an infeasible solution. \cite{ABDELMALEK2005296} propose a methodology for solving the problem when $B \le B_1$. If $B_1 \le B \le B_2$ or $B \ge B_2$ then standard methods apply. 

The method proposed by~\cite{ABDELMALEK2005296} can be summarised as follows. 
\begin{enumerate}
    \item Find multipliers associated with $q_t(\lambda) = 0$ i.e.\ $\lambda_1,\dots, \lambda_T$.
    \item Evaluate $B_1, B_2$ to find the range in which $B$ lies.
    \begin{enumerate}
        \item If $B \le B_1$ or $B_1 \le B \le B_2$ then go to 4.
        \item If $B \ge B_2$ then go to 3.
    \end{enumerate}
    \item Order $\lambda_t$ based on increasing size (lowest means lowest marginal profit).
    \begin{enumerate}
        \item Find $\lambda_j$, the smallest value of $\lambda_t$.
        \item Remove item $j$ from list of items so there are now $R < N$ items in the list.
        \item Calculate $q^*(\lambda_j)$ and the lower bound on the budget required for including item $j$ in the list:
        $$B^R_{1, j} = \sum_{t=1}^T w_t q^*_t(\lambda_j).$$
        \item If $B \le B^R_{1, j}$ then go to 4 because the non-negativity constraints can be relaxed.
        \item Else, go back to a.
    \end{enumerate}
    \item Solve using KKT conditions.
    \item Return solution.
\end{enumerate}

This is the idea that~\cite{ALFARES2005465} apply to their problem. Their algorithm is as follows.
\begin{enumerate}
    \item Set $\lambda = 0$ (i.e.\ no budget constraint) and solve using KKT conditions, setting negative solutions to zero.
    \item If budget constraint is met then go to 5. Else go to 3.
    \item Starting from $\lambda = 0$ increase $\lambda$ iteratively until the first occurence of either of the following:
    \begin{enumerate}
        \item A decision becomes negative. Go to step 4.
        \item Budget constraint met. Go to step 5.
    \end{enumerate}
    \item Set the negative decision variable to zero, remove from the set of items and go to step 1.
    \item Return solution.
\end{enumerate}
Essentially, the steps can be explained as follows. First, attempt to solve with no budget constraint and no non-negativity constraints. Use the KKT solution if it is feasible, else set that decision to zero. If the budget constraint is met we are done. If it's not, we need to add it. So we gradually increase $\lambda$ until either the solution becomes optimal or it becomes infeasible. If it becomes infeasible, we take away one of the variables and start again with a new set of items. \textbf{It would be good to discuss this to see if we can use it for our problem. }


\subsection{An Adaptation of the Alfares and Elmorra Algorithm: FD}

The~\cite{ALFARES2005465} algorithm solves the multi-product newsvendor to optimality in the presence of the budget constraint. The idea of their budget constraint is to start by solving with $\lambda = 0$ and then iteratively increase $\lambda$ until either the solution meets the budget constraint or one of the orders has a negative expected profit. In the latter case, this item is removed from the list and its order set to zero permanently. 

The main difference between our model and theirs is the structure of the optimal KKT solution that results from the inventory tracking. Their solution is of the form:
\begin{equation}
    x_\tau = F^{-1}(P_\tau) \fa \tau \in \{1,\dots,N\}.
\end{equation}
This means that orders for different items do not affect one another. However, our solution is of the form:
\begin{equation}\label{eq:q_t_simple}
    q^*_t = \tilde{F}^{-1}_t(P_t) - \tilde{F}^{-1}_{t-1}(P_{t-1}),
\end{equation}
where the subtraction of $\tilde{F}^{-1}_{t-1}(P_{t-1})$ is done to ensure that 
\begin{equation}\label{eq:important_relation}
    \sum_{k=1}^t q^*_k = \tilde{F}^{-1}_t(P_t).
\end{equation}
This relation holding true is what ensures that our KKT conditions are met. In the algorithm of~\cite{ALFARES2005465}, when an item is removed and set to zero, this is because its marginal profit has become negative. This means that if we continue to increase $\lambda$ then this value will become negative and stay negative. 

We can apply similar logic to our problem, with one slight difference. When Alfares and Elmorra set one variable to zero, the other variables can be found via their respective formulas and the corresponding derivatives will still be zero. However, if we set $q^*_{t-1} = 0$ then the value of $q^*_t$ from~\eqref{eq:q_t_simple} will not give~\eqref{eq:important_relation}. In fact, $q^*_{t-1}$ being zero means that 
\begin{align}
    \sum_{k=1}^t q^*_k &= \sum_{k=1}^{t-2} q^*_k + q^*_t\\
    &= \tilde{F}^{-1}_{t-2}(P_{t-2}) + ( \tilde{F}^{-1}_t(P_t) - \tilde{F}^{-1}_{t-1}(P_{t-1})).
\end{align}
This means that in order to satisfy~\eqref{eq:important_relation}, the optimal value of $q^*_t$ becomes $\tilde{F}^{-1}_t(P_t) - \tilde{F}^{-1}_{t-2}(P_{t-2})$. Hence, when we remove a day from the set of days, we need to adjust the remaining solutions. Suppose we have a set $\m{T}^0$ of days that have been set to zero permanently. Then, when re-calculating our next solution we use:
\begin{align}
    \tilde{q}^*_0 &= \begin{cases}
        \tilde{F}^{-1}_1\l(\frac{b - (1+\lambda)(w_1 - w_2)}{h+b}\r) &\text{ if } 0 \notin \m{T}^0\\
        0 &\text{ if } 0 \in \m{T}^0
    \end{cases}\\
    \tilde{q}^*_t &= \begin{cases}
         \tilde{F}^{-1}_t\l(\frac{b - (1+\lambda)(w_t - w_{t+1})}{h+b}\r) - \sum_{k=1}^{t-1} \tilde{q}^*_k &\text{ if } t \notin \m{T}^0\\
        0 &\text{ if } t \in \m{T}^0
    \end{cases}
    \fa t \in \{2,\dots,T-1\}\\
    \tilde{q}^*_T &= \begin{cases}
        \tilde{F}^{-1}_T\l(\frac{b - (1+\lambda)w_T + p }{h+b+p}\r) - \sum_{k=1}^{T-1}\tilde{q}^*_k  &\text{ if } T \notin \m{T}^0\\
        0 &\text{ if } T \in \m{T}^0
    \end{cases}.
\end{align}
With this in mind, we present our adaptation of the algorithm from~\cite{ALFARES2005465}. We will refer to this algorithm as Fixed Distribution (FD). To make things clearer, let us denote by $q^*(\lambda)$ the value obtained from evaluating~\eqref{eq:KKT_sol} with Lagrange multiplier $\lambda$. Similarly we define $\tilde{q}^*(\lambda)$.

\begin{enumerate}
    \item Set $\m{T}^0 = \{\}$.
    \item Take $q = (\max\{\tilde{q}^*_1(0), 0\},\dots,\max\{\tilde{q}^*_T(0), 0\})$, i.e.\ $\tilde{q}^*(0)$ but setting negative values to zero.
    \item If $\sum_{t=1}^T w_t q_t \le W$ then go to step 7. If $\sum_{t=1}^T w_t q_t > W$ then if $\m{T}^0 = \{\}$  go to step 4 and otherwise go to step 5. 
    \item The budget constraint is binding. Compute upper bounds on $\lambda$, i.e.\ 
    \begin{equation}
        \lambda^{\text{UBs}} = \l\{\frac{b}{w_t - w_{t+1}} - 1 \fa t \in \{1,\dots,T-1\}\r\} \cup \l\{\frac{b+p}{w_T} - 1\r\}
    \end{equation}
    and set $\lambda^{\text{UB}} = \min\{\lambda^{\text{UBs}}\}$. Then $\lambda \le \lambda^{\text{UB}}$ ensures that the inverse CDFs are all defined at $\lambda$. Go to step 5.
    \item Starting from $\lambda=0$, gradually increase $\lambda$ until the first occurrence of one of the following:
    \begin{enumerate}
        \item The resulting $\tilde{q}^*(\lambda)$ has $\tilde{q}^*_k(\lambda) < 0$ for some $k$. In this case go to step 6.
        \item The resulting $\tilde{q}^*$ has $\sum_{t=1}^T w_t \tilde{q}^*(\lambda) \le W$. In this case go to step 7.
        \item $\lambda = \lambda^{\text{UB}}$. In this case, increasing $\lambda$ any further will make the KKT solution invalid. Choose $k = \argmin_{t} q^*_t(\lambda)$ and find the set:
            $$\m{K} = \{k \in \m{T}\setminus \m{T}^0: \lambda = \lambda^{\text{UBs}}_k\},$$
        and set $k = \argmin_{t \in \m{K}} q^*_t(\lambda)$. This day must be the least profitable out of the days in $\m{K}$ that cannot be reduced further.  Go to step 6.
    \end{enumerate}
    \item For each day $t \in \m{T} \setminus \m{T}^0$, calculate a lower bound on the cost resulting from setting $q_t = 0$ and adding $t$ to $\m{T}^0$. Specifically, calculate $\tilde{q}^*(\lambda)$ with $\lambda$ being equal to the value obtained in step 5, under each scenario for the next version of $\m{T}^0$. Select $k$ to be the day with the highest upper bound resulting from adding it to $\m{T}^0$. Set $\m{T}^0 = \m{T}^0 \cup \{k\}$ and go to step 2.
    \item Return $\tilde{q}^*(\lambda)$.
\end{enumerate}

The current version of the algorithm uses a line search to find the optimal value of $\lambda$ in Step 5. Note that, in practice, we will use a tolerance parameter for checking $\sum_{t=1}^T w_t q_t \le W$. In the implementation of the above algorithm, this constraint is replaced by $\sum_{t=1}^T w_t q_t - W \le \varepsilon_W$, where $\varepsilon_W$ is specified by the user.

\subsection{Testing FD}

% We tested this algorithm on 64000 problem instances with normal demands. We compared it with the two algorithms in Scipy's optimisation package, \texttt{SLSQP} (SLSQP) and \texttt{trust-constr} (TC). We make the following observations from the results:
% \begin{enumerate}
%     \item Our algorithm took an average of 0.45 seconds to finish running, SLSQP took 0.29 seconds and TC took 3 seconds on average. 
%     \item All 3 algorithms had the same objective value in 71\% of cases. 
%     \item Our algorithm had the same as or a better objective value than the other 2 in 91\% of cases. 
%     \item TC had the same as or a better objective value than the other 2 in 78\% of cases. 
%     \item SLSQP had the same as or a better objective value than the other 2 in 98\% of cases. 
%     \item SLSQP does not respect the budget tolerance. In 27\% of instances, the budget constraint violation was higher than the budget tolerance specified. 
%     \item There is no way to specify a budget tolerance in SLSQP, but there is in TC and our algorithm.
% \end{enumerate}
% We can conclude that SLSQP is the best algorithm if we do not want to be able to control the tolerance for the budget constraint. However, if we would like to control this, then our algorithm is clearly the best option. We cannot guarantee that the budget constraint will be strictly met if we use SLSQP, with violations averaging $3.8 \times 10^{-8}$. TC has a tolerance parameter that can be controlled by the user, so this algorithm is a better point of comparison for our algorithm. In fact, TC is much slower than our algorithm and still does not guarantee that the budget tolerance is respected. The budget tolerance was exceed in 27 instances by TC. It was not exceeded at all by our algorithm.

In order to establish the performance of FD, we tested is on 1536 problem instances. We obtained these by varying all parameters and considering problems with $T \in \{2,\dots,5\}$. We selected 2 mean vectors randomly for each $T$. Each combination of $T$ and a mean was run for both normal and Poisson demands. Since our algorithm is a heuristic, we compare it with 3 other methods that might be applied to solve MPNVP. These methods are as follows:

\begin{enumerate}
    \item SLSQP: Sequential Least Squares Quadratic Programming~\citep{SLSQP}. This is an algorithm that can be found in Python's baseline package for scientific computing, Scipy~\citep{2020SciPy-NMeth}.
    \item TC: Trust Constraint~\citep{trust_constr}. This is another algorithm that can be found in Scipy.
    \item PLA: Piecewise Linear Approximation. This entails using a piecewise linear approximation to the objective function, allowing it to be solved by off the shelf LP/MIP solvers. 
\end{enumerate}

We now summarise the results of our experiments. Figure~\ref{fig:FD_times} shows the times taken by each algorithm under normal and Poisson demands. The plots sow that FD and SLSQP are the fastest algorithms for both normal and Poisson demands. On average, for normal demands, FD took 0.24 seconds and SLSQP took 0.27 seconds. For Poisson demands, FD took 0.38 seconds whereas SLSQP took 0.61 seconds. Hence, our results suggest that FD is the fastest algorithm on average. Furthermore, our results suggest that TC is by far the slowest algorithm.

\begin{figure}[htbp!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Alfares/normal_tt.png}
        \caption{}
        \label{fig:FD_normal_times}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Alfares/poisson_tt.png}
        \caption{}
        \label{fig:FD_poisson_times}
    \end{subfigure}
    \caption{Boxplots summarising times taken by the 4 algorithms}
    \label{fig:FD_times}
\end{figure}

To understand the performance of the algorithms, we define an optimality gap as follows. In each instances, we treat the best solution as optimal. This allows us to define a percentage optimality gap as follows:
$$100 \times \frac{C_{F}(\bm{q}^x) - \min_{y \in \m{X}} C_F(\bm{q}^y)}{\min_{y \in \m{X}} C_F(\bm{q}^y)},$$
where $x \in \m{X} = \{\text{FD}, \text{PWL}, \text{SLSQP}, \text{TC}\}$ represents an algorithm, and $\bm{q}^x$ is the solution returned by algorithm $x$. Given this definition, we summarise the gaps in Figure~\ref{fig:optgaps_alf}. This plot shows that FD is typically within 2.5\% of the best solution for normal demands. SLSQP and TC perform the best here. However, for Poisson demands, FD and PWL are the best algorithms in terms of objective value.  It is important to mention that, while SLSQP performs well for Poisson demands, in 678 out of 768 instances with Poisson demands, its solution was not integer. In addition there is no way to enforce integer variables within this algorithm. Hence, FD and PLA have this as an advantage over SLSQP: if the distribution is discrete, their solutions are integer.

\begin{figure}[htbp!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Alfares/normal_percent_opt_gap.png}
        \caption{}
        \label{fig:FD_normal_gaps}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Alfares/poisson_percent_opt_gap.png}
        \caption{}
        \label{fig:FD_poisson_gaps}
    \end{subfigure}
    \caption{Boxplots summarising percentage optimality gaps of the 4 algorithms}
    \label{fig:optgaps_alf}
\end{figure}

The final result we would like to mention is the exceedance of the budget. TC is very similar to SLSQP, apart from that TC allows us to specify a tolerance for exceeding the budget. SLSQP does not allow this. Hence, we present the number of times each algorithm exceeded the budget tolerance along with the maximum amount by which the budget was exceeded. These results are shown in Table~\ref{tab:exceedances}, which shows that FD never exceeded the budget tolerance while SLSQP did in over 200 instances. In fact, FD is the only algorithm that never exceeded the budget constraint by more than the tolerance. The reason why FD's maximum exceedance is $9.98\times 10^{-11}$ is because we used a tolerance of $10^{-10}$ in some instances. SLSQP also has the maximum exceedance among all algorithms.

\begin{table}[htbp!]
    \centering
    \input{images_tables/Final Alfares/exceedances}
    \caption{Summary of budget exceedance by each algorithm}
    \label{tab:exceedances}
\end{table}

From these results, we can conclude four main points. Firstly, FD is the fastest algorithm out of all that we tested. Secondly, FD is typically close the best solution in general, and performs better than SLSQP and TC for Poisson demands. Thirdly, SLSQP and TC do not return integer solutions for the Poisson distribution in general. There is also no way to enforce this. Despite FD being designed for continuous distributions, when the demand random variable is discrete, its solution will be integer. This is an important point, as when demand is discrete the order quantity should also be. Finally, FD is the only algorithm that can be guaranteed not to exceed the budget constraint by more than some user-specified tolerance. 

==> A_normal_old.tex <==
\section{DRO Model with Normal Demands}

The first parametric DRO model that we study is the one resulting from independent normal demands. Suppose we have a set $\Omega$ of pairs $\bm{\omega} = (\bm{\mu}, \bm{\sigma})$
such that each $\bm{\omega}$ gives a unique multivariate normal distribution. This means there is a unique CDF $F$ for each $\bm{\omega}$ and so we can replace $F$ with $\bm{\omega}$.
Then the DRO model is:
\begin{equation}\label{eq:MPNVP_DRO_obj}
    \min_{\bm{q}}\max_{\bm{\omega}\in \Omega}C_{\bm{\omega}}(\bm{q}) = p\E_{\bm{\omega}}[I^-_T] + 
    \sum_{t=1}^T \l(h\E_{\bm{\omega}}[I^+_t] + b\E_{\bm{\omega}}[I^-_t] + w_t q_t- p \E_{\bm{\omega}}[X_t]\r) 
\end{equation}
s.t.\ constraints~\eqref{eq:MPNVP_1}-\eqref{eq:MPNVP_3}.

\subsection{Objective Function}

Since  $\bm{X} \sim N(\bm{\mu}, \bm{\sigma})$ and the $X_t$'s are independent,
we have $X_t \sim N(\mu_t, \sigma_t)$. Furthermore, let $q =
\sum_{t=1}^T q_t$ represent the total ordering quantity and let $X =
\sum_{t=1}^T X_t$ be the total demand. Then we have:
\begin{equation}\label{eq:X_dist}
    X \sim N\l(\sum_{t=1}^T \mu_t, \sum_{t=1}^T \sigma^2_t\r) = N(\mu, \sigma^2),
\end{equation}
where $\mu = \sum_{t=1}^T \mu_t$ and $\sigma^2 = \sum_{t=1}^T \sigma^2_t$.
Furthermore, since $I_t = \sum_{k=1}^t (q_k - X_k)$, we have:
\begin{equation}
    I_t \sim N\l(\sum_{k=1}^t (q_k - \mu_k), \sum_{k=1}^t \sigma^2_k\r) \fa t = 1,\dots,T,
\end{equation}
and in particular:
\begin{equation}
    I_T \sim N(q - \mu, \sigma^2).
\end{equation}
Therefore, we have:
\begin{align}
    \E_{\bm{\omega}}[I^+_t] &= \E_{\bm{\omega}}[\max\{I_t, 0\}]\\
    &= \P(I_t \ge 0)\E_{\bm{\omega}}[I_t | I_t \ge 0] \\
    &= \Phi(-\alpha_t) \l(\sum_{k=1}^t(q_k - \mu_k) + \sqrt{\sum_{k=1}^t \sigma_k^2} \frac{\phi(\alpha_t)}{1-\Phi(\alpha_t)}\r) \\
    &= \Phi(-\alpha_t)\sum_{k=1}^t(q_k - \mu_k) + \phi(\alpha_t)\sqrt{\sum_{k=1}^t \sigma_k^2},
\end{align}
where $\alpha_t = \frac{-\sum_{k=1}^t(q_k - \mu_k)}{\sqrt{\sum_{k=1}^t
\sigma_k^2}}$. Finally, we have:
\begin{align}
    \E_{\bm{\omega}}[I^-_t] &= \E_{\bm{\omega}}[\max\{-I_t, 0\}]\\
    &= \P(-I_t \ge 0)\E_{\bm{\omega}}[-I_t | -I_t \ge 0] \\
    &= \Phi(\alpha_t) \l(-\sum_{k=1}^t(q_k - \mu_k) + \sqrt{\sum_{k=1}^t \sigma_k^2} \frac{\phi(-\alpha_t)}{1-\Phi(-\alpha_t)}\r) \\
    &= \Phi(\alpha_t)\sum_{k=1}^t(\mu_k - q_k) + \phi(\alpha_t)\sqrt{\sum_{k=1}^t \sigma_k^2},
\end{align}
These formulas have been obtained using the law of total expectation in
combination with the formulas for the expected values of a truncated normal
variable. This means we can write the objective function as:
\begin{dmath}
    C_{\bm{\omega}}(\bm{q}) \hiderel{=} \sum_{t=1}^T\l\{
    h\l[\Phi(-\alpha_t)\sum_{k=1}^t(q_k - \mu_k) +
    \phi(\alpha_t)\sqrt{\sum_{k=1}^t \sigma_k^2}\r] +
    (b + p\mathds{1}\{t\hiderel{=} T\})\l[\Phi(\alpha_t)\sum_{k=1}^t(\mu_k - q_k) +
    \phi(\alpha_t)\sqrt{\sum_{k=1}^t \sigma_k^2}\r] + w_t q_t - p \mu_t\r\}
    = \sum_{t=1}^T\l\{(h(\Phi(\alpha_t) - 1) +  (b +  p\mathds{1}\{t\hiderel{=}
    T\})\Phi(\alpha_t))\sum_{k=1}^t(\mu_k - q_k) + (h + b +
    p\mathds{1}\{t\hiderel{=} T\})\phi(\alpha_t)\sqrt{\sum_{k=1}^t\sigma^2_k} +
    w_t q_t - p \mu_t\r\} 
    = \sum_{t=1}^T\l\{((b +  p\mathds{1}\{t\hiderel{=}
    T\} + h)\Phi(\alpha_t) - h)\sum_{k=1}^t(\mu_k - q_k) + (h + b +
    p\mathds{1}\{t\hiderel{=} T\})\phi(\alpha_t)\sqrt{\sum_{k=1}^t\sigma^2_k} +
    w_t q_t- p \mu_t\r\} 
\end{dmath}
or
\begin{dmath}
    C_{\bm{\omega}}(\bm{q}) \hiderel{=}
     \sum_{t=1}^T\l\{(a_t \Phi(\alpha_t) - h)\sum_{k=1}^t(\mu_k - q_k)
    + a_t \phi(\alpha_t)\sqrt{\sum_{k=1}^t \sigma_k^2} +
    q_t w_t- p \mu_t\r\}.
\end{dmath}
where $\mathds{1}\{t=T\}$ is 1 if $t=T$ and 0 otherwise, and $a_t = b +
p\mathds{1}\{t=T\} + h$.
% We have two parts of the objective, the expected revenue and the
% expected cost. Their difference is the objective, the expected profit.
% Let's call the profit function $P$, the revenue function $R$ and the cost
% function $C$. Then, expanding the expected values, we have:
% \begin{align}
%     \E_{\bm{\omega}}(R(\bm{q})) &= p \l[\Phi(\beta)\mu - \sigma\phi(\beta) + q\Phi(-\beta)\r], \\
%     \E_{\bm{\omega}}(C_{\bm{\omega}}(\bm{q})) &= \sum_{t=1}^T \l[\l(h- (h+b)\Phi(\alpha_t)\r)\sum_{k=1}^t(q_k - \mu_k) + (h + b)\phi(\alpha_t)\sqrt{\sum_{k=1}^t \sigma_k^2} + w_t q_t\r],\\
%     \E_{\bm{\omega}}(P_{\bm{\omega}}(\bm{q})) &= \E_{\bm{\omega}}(R(\bm{q})) - \E_\omega(C_{\bm{\omega}}(\bm{q})).
% \end{align}
% Using the above, we write the objective as:
% \begin{dmath}\label{eq:long_DRNVP_obj}
%     \max_{\bm{q}}\E_{\bm{\omega}}(P_{\bm{\omega}}(\bm{q})) = \l\{p \l[\Phi(\beta)\mu - \sigma\phi(\beta) + q\Phi(-\beta)\r] - \sum_{t=1}^T \l[\l(h- (h+b)\Phi(\alpha_t)\r)\sum_{k=1}^t(q_k - \mu_k) + (h + b)\phi(\alpha_t)\sqrt{\sum_{k=1}^t \sigma_k^2} + w_t q_t\r]\r\}
% \end{dmath}
% From Section~\ref{sec:NV_derivs}, we know that $\E_{\bm{\omega}}(R(\bm{q}))$ is
% increasing in $\mu$ and decreasing in $\sigma$. However, here we are also
% concerned with the derivatives with respect to each $\mu_t$ and $\sigma_t$.


\subsection{Derivatives of Objective Function}\label{sec:normal_theory}

In order to differentiate, we consider $\mu_1,\dots,\mu_T$ and $\sigma_1, \dots,
\sigma_T$ and look at where each value appears. Let $\tau \in \{1,\dots,T\}$.
Then $\mu_\tau$ and $\sigma_\tau$ appear in the $t^{\text{th}}$ term of the sum
for each $t \ge \tau$. In fact, recalling that $\alpha_t =
\frac{-\sum_{k=1}^t(q_k - \mu_k)}{\sqrt{\sum_{k=1}^t \sigma_k^2}}$, we have
\begin{align}
    \pderiv{\alpha_t}{\mu_\tau} &= \begin{cases}
        0 & \text{ if } \tau > t, \\
        \frac{1}{\sqrt{\sum_{k=1}^t\sigma^2_k}}, & \text{ if } \tau \le t.
    \end{cases}
    \\
    \pderiv{\alpha_t}{\sigma_\tau} &= \begin{cases}
        0 & \text{ if } \tau > t,\\
        \frac{\sum_{k=1}^t(q_k - \mu_k)}{\sigma_\tau\l(\sum_{k=1}^t \sigma^2_k \r)^{\frac{3}{2}}} &\text{ if } \tau \le t.
    \end{cases}
\end{align}
Hence, $\alpha_t$ is increasing in $\mu_\tau$ for all $\tau$. Also, $\alpha_t$
is increasing in $\sigma_\tau$ for all $\tau$ if $\sum_{k=1}^t q_k \ge
\sum_{k=1}^t \mu_k$. Using the chain rule, we have:
\begin{align}
    \pderiv{\Phi(\alpha_t)}{\mu_\tau} &= \frac{\phi(\alpha_t)}{\sqrt{\sum_{k=1}^t\sigma^2_k}} \\
    \pderiv{\Phi(\alpha_t)}{\sigma_\tau} &= \frac{\sum_{k=1}^t(q_k - \mu_k)}{\sigma_\tau\l(\sum_{k=1}^t \sigma^2_k \r)^{\frac{3}{2}}} (-\alpha_t\phi(\alpha_t)) 
\end{align} 
for $x_\tau \in \{\mu_\tau, \sigma_\tau\}$. Therefore, $\Phi(\alpha_t)$ is
increasing in $\mu_\tau \fa \tau \in \m{T}$. Since we can write:
\begin{equation}
    \frac{\sum_{k=1}^t(q_k - \mu_k)}{\sigma_\tau\l(\sum_{k=1}^t \sigma^2_k \r)^{\frac{3}{2}}} = \frac{-\alpha_t}{\sigma_\tau \sum_{k=1}^t \sigma^2_k}
\end{equation}
we have that $\Phi(\alpha_t)$ is increasing in $\sigma_\tau$ if $\alpha_t \le 0$
i.e.\ if $\sum_{k=1}^t q_k \ge \sum_{k=1}^t \mu_k$ (this could be obtained
without derivatives, since $\alpha_t$ is increasing in $\sigma_\tau$ while
negative and decreasing while positive). Furthermore, we have:
\begin{align}
    \pderiv{\phi(\alpha_t)}{\mu_\tau} &= \frac{1}{\sqrt{\sum_{k=1}^t\sigma^2_k}} (-\alpha_t\phi(\alpha_t))\\
    \pderiv{\phi(\alpha_t)}{\sigma_\tau} &= \frac{-\alpha_t}{\sigma_\tau \sum_{k=1}^t \sigma^2_k} (-\alpha_t\phi(\alpha_t))  \\
    &= \frac{1}{\sigma_\tau \sum_{k=1}^t \sigma^2_k}\alpha_t^2 \phi(\alpha_t) 
\end{align} 
Hence, $\phi(\alpha_t)$ is increasing in $\mu_\tau$ if $\alpha_t \le 0$ i.e.\
$\sum_{k=1}^t q_k \ge \sum_{k=1}^t \mu_k$. Also, $\phi(\alpha_t)$ is increasing
in $\sigma_\tau$ for all $\tau$. Now, differentiating the objective we have:
\begin{dmath}
    \pderiv{C_{\bm{\omega}}(\bm{q})}{\mu_\tau} \hiderel{=} \sum_{t=\tau}^T\l\{
    (a_t \Phi(\alpha_t) - h) + a_t \frac{\phi(\alpha_t)}{\sqrt{\sum_{k=1}^t \sigma^2_k}}\sum_{k=1}^t(\mu_k -
    q_k) - a_t \frac{\alpha_t \phi(\alpha_t)}{\sqrt{\sum_{k=1}^t \sigma^2_k}}\sqrt{\sum_{k=1}^t \sigma^2_k}
    \r\}
\end{dmath}
and we can simplify this to:
\begin{align}
    \pderiv{C_{\bm{\omega}}(\bm{q})}{\mu_\tau} &= \sum_{t=\tau}^{T}\l\{
    - h + a_t\l(\Phi(\alpha_t)  + \frac{\phi(\alpha_t)}{\sqrt{\sum_{k=1}^t
    \sigma^2_k}}\sum_{k=1}^t(\mu_k - q_k)\r) - a_t \alpha_t \phi(\alpha_t) - p
    \r\}\\
    &= \sum_{t=\tau}^T \l\{-h + a_t\l(\Phi(\alpha_t)+\alpha_t\phi(\alpha_t)\r) - a_t\alpha_t
    \phi(\alpha_t) - p\r\}\\
    &= \sum_{t=\tau}^T \l\{a_t\Phi(\alpha_t) - h - p\r\} \label{eq:MPNVP_mu_deriv}
\end{align}

% To find a root of this derivative, we find $\bm{\mu}^*$ such that:
% \begin{equation}
%     \l.\sum_{t=\tau}^T \l\{a_t\Phi(\alpha_t) - h\r\} \r\rvert_{\bm{\mu} = \bm{\mu}^*} = 0 \fa \tau \in \m{T}.
% \end{equation}
% we can solve this by finding $\alpha^*_t$ such that:
% \begin{equation}
%     a_t \Phi(\alpha^*_t) = h \fa t \in \m{T},
% \end{equation}
% and using $\alpha^*_t$ to obtain $\bm{\mu}^*$.
% For now, let $z_t = \Phi^{-1}\l(\frac{h}{a_t}\r)$ and let $s_t =
% \sqrt{\sum_{k=1}^t\sigma^2_t}$ to save on typing/reading. Note that, by
% definition of $\alpha^*_t$, we have $\alpha^*_t = z_t$. Starting with $t=1$ we
% have:
% \begin{align}
%     a_1 \Phi(\alpha^*_1) &= h \\
%     \frac{\mu^*_1 - q_1}{s_1} &= z_1 \\
%     \mu^*_1 &= z_1s_1 + q_1.
% \end{align}
% Then for $t=2$, using that $\mu^*_1 - q_1 = z_1 s_1$:
% \begin{align}
%     a_2 \Phi(\alpha^*_2) &= h \\
%     \frac{(\mu^*_1 - q_1) +(\mu^*_2 - q_2)}{s_2} &= z_2 \\
%     \mu^*_2 &= s_2z_2 - z_1s_1 + q_2.
% \end{align}
% and generally:
% \begin{align}
%     \mu^*_1 &=  z_1 s_1 + q_1,\\
%     \mu^*_t &= s_t z_t - z_{t-1}s_{t-1} + q_t \fa t \in \{2,\dots,T\}.
% \end{align}
% To prove this via induction, suppose it holds for some $k \in \{2,\dots,T\}$. We
% have already shown it to hold for $k=2$. Then we have:
% \begin{align}
%     a_{k+1} \Phi(\alpha^*_{k+1}) &= h \\
%     \alpha^*_{k+1} &= z_{k+1}\\
%     \frac{s_{k}\alpha^*_{k} + (\mu^*_{k+1} - q_{k+1})}{s_{k+1}} &= z_{k+1} \\
%     \mu^*_{k+1} &= s_{k+1}z_{k+1} - \alpha^*_k s_{k} + q_{k+1} \\
%     &= s_{k+1}z_{k+1} - z_k s_k + q_{k+1}.
% \end{align}
Furthermore, with $s_t = \sqrt{\sum_{k=1}^t\sigma^2_t}$ we have:
\begin{equation}
    \frac{\partial^2 C_{\bm{\omega}}(\bm{q})}{\partial \mu^2_\tau} = \sum_{t=\tau}^T a_t \frac{\phi(\alpha_t)}{s_t} > 0
\end{equation}
meaning that this $\bm{\mu}^*$ is a minimum. Since the second derivative is
positive everywhere, the objective is convex in each $\mu_\tau$, with a unique
minimum at $\mu^*_{\tau}$. This means the maximum cost is obtained either at the
minimum or maximum values for $\mu_\tau$ for each $\tau$.

We also have:
\begin{align}
    \pderiv{C_{\bm{\omega}}(\bm{q})}{\sigma_\tau} &= \sum_{t=\tau}^T\l\{
    a_t\l(\frac{-\alpha_t\phi(\alpha_t)}{\sigma_\tau \sum_{k=1}^t\sigma^2_k}\r)\sum_{k=1}^t(\mu_k - q_k) + \frac{a_t \phi(\alpha_t)}{\sigma_\tau\sqrt{\sum_{k=1}^t\sigma^2_k}} + a_t\sqrt{\sum_{k=1}^t\sigma^2_k}\frac{\alpha^2_t\phi(\alpha_t)}{\sigma_\tau \sum_{k=1}^t \sigma^2_k}     
    \r\}\\
    &= \sum_{t=\tau}^T\l\{a_t\l(\frac{-\alpha^2_t \phi(\alpha_t)}{\sigma_\tau \sqrt{\sum_{k=1}^t\sigma^2_k}}\r) + \frac{a_t\phi(\alpha_t)}{\sigma_\tau \sqrt{\sum_{k=1}^t\sigma^2_k}} + a_t \frac{\alpha^2_t}{\sigma_\tau \sqrt{\sum_{k=1}^t\sigma^2_k}}\r\}\\
    &= \sum_{t=\tau}^T \frac{a_t \phi(\alpha_t)}{\sigma_\tau \sqrt{\sum_{k=1}^t\sigma^2_k}}\label{eq:MPNVP_sig_deriv}\\
    & > 0 \fa \tau \in \m{T}.
\end{align}
Hence, $C_{\bm{\omega}}(\bm{q})$ is increasing in $\sigma_\tau$ for all $\tau
\in \m{T}$. This means that the worst case distribution gives each day the
highest standard deviation it can have.



\subsection{Piecewise Linear Approximation}

Since the objective of our problem is nonlinear, and also not quadratic, we
use a Piecewise Linear Approximation (PLA) to the problem to solve it. In order to create a PLA to the
model, we must define a PLA to the entire non-linear part of the model. Let us
define $g_t(\alpha_t)$ as the non-linear part of the cost for day $t$. This function can
be written as
\begin{equation*}
    g_t(\alpha_t) = \sqrt{\sum_{k=1}^t \sigma_k^2}\l\{(a_t \Phi(\alpha_t) - h) \alpha_t  + a_t \phi(\alpha_t) \r\}, \ t = 1,\dots,T.
\end{equation*}
We use the following procedure to create a PLA of the model:
\begin{enumerate}
    \item Create a set of points $z_1,\dots,z_J$ that act as $\alpha_t$.
    where $\varepsilon$ is referred to as the \textit{gap}. 
    \item Apply $g_t$ to these points to get a sample of values
    $g_t(z_i)$ for $i=1,\dots,I$ and $t=1,\dots,T$.  
    \item Define piecewise linear approximation of $g_t$ for $t=1,\dots,T$:
    \begin{equation}\label{eq:PWL_CDF}
        G_t(z) = \begin{cases}
            \frac{z-z_{2}}{z_1 - z_{2}}g_t(z_1) + \frac{z-z_1}{z_{2} - z_1} g_t(z_{2}) &\text{ if } z_1 \le z \le z_{2}\\
            \qquad \vdots \\
            \frac{z-z_{i+1}}{z_i - z_{i+1}}g_t(z_i) + \frac{z-z_i}{z_{i+1} - z_i} g_t(z_{i+1}) &\text{ if } z_i\le z \le z_{i+1}\\
            \qquad \vdots \\
            \frac{z-z_{n}}{z_{n-1} - z_{n}}g_t(z_{n-1}) + \frac{z-z_{n-1}}{z_{n} - z_{n-1}} g_t(z_{n}) &\text{ if } z_{n-1}\le z \le z_{n}
        \end{cases}
    \end{equation}
    \item Define dummy variables $\tilde{\alpha}_t$ and $\tilde{g}_t$, where $\tilde{g}_t$ represents $g_t(\alpha_t)$.
    \item Construct piecewise linear approximation of model:
    \begin{equation}\label{eq:PWL_obj}
        \min_{q, \tilde{g}, \tilde{\alpha}}   \tilde{C}_{\bm{\omega}}(\bm{q}) = \sum_{t=1}^T\l\{\tilde{g}_t + q_t w_t - p \mu_t\r\}
    \end{equation}
    s.t.
    \begin{align}
        \sum_{t=1}^T w_t q_t \le W,\\
        \tilde{\alpha}_t = \frac{\sum_{k=1}^t (\mu_k -
        q_k)}{\sqrt{\sum_{k=1}^t\sigma^2_k}} \fa t \in \m{T} \label{eq:fix_alpha}\\
        \tilde{g}_t = G_t(\tilde{\alpha}_t) \fa t \in \m{T} \label{eq:fix_g}\\
        q_t \ge 0 \fa t \in \m{T}. \label{eq:PWL_lastconstraint}.
    \end{align}
    Here, \eqref{eq:fix_alpha} ensures that $\tilde{\alpha}_t = \alpha_t$. We do not technically need a dummy variable for $\alpha_t$ as it is linear in the $q_k$, but Gurobi requires the PLA function $G_t$ to be evaluated at a dummy variable. Then, \eqref{eq:fix_g} ensures that $\tilde{g}_t$ is equal to the PLA of $g_t$ evaluated at the dummy variable $\tilde{\alpha}_t$. 
\end{enumerate}

\subsection{Piecewise Linear DRO Model}

We can construct a DRO version of the piecewise linear model via the following. Firstly,
we define $I = |\Omega|$ and define the index $i=1,\dots,I$ to represent the
index of an $\omega \in \Omega$. Secondly, create dual-indexed dummy variables
$\tilde{\alpha}^i_t$ and $\tilde{g}^i_t$ such
that an index $i$ corresponds to the value of the variable when the distribution
is given by $\bm{\omega}^i \in \Omega$. Here, $\bm{\omega}^i = (\bm{\mu}^i,
\bm{\sigma}^i)$ is the $i$th element of $\Omega$. Thirdly, define a dummy
variable $\theta$ to represent the worst-case cost. Then, our model is given by:
\begin{align}
    \min_{q, \tilde{g}, \tilde{\alpha}} \quad  &\theta \label{eq:DRO_PWL_obj} \\
    \text{s.t. } &\theta \ge \sum_{t=1}^T\l\{\tilde{g}^i_t + q_t w_t - p \mu^i_t\r\} \fa i = 1,\dots,I\\
    &\sum_{t=1}^T w_t q_t \le W,\\
    &\tilde{g}^i_t = G_t(\tilde{\alpha}^i_t) \fa t \in \m{T}, \fa i = 1,\dots,I\\
    &\tilde{\alpha}^i_t = \frac{\sum_{k=1}^t (\mu^i_k -
    q_k)}{\sqrt{\sum_{k=1}^t(\sigma^i_{k})^2}} \fa t \in \m{T}, \fa i = 1,\dots,I\\
    &q_t \ge 0 \fa t \in \m{T}. \label{eq:DRO_PWL_lastconstraint}
\end{align}

\subsection{Extreme Distributions}

In order to construct a cutting surface algorithm, we need to find the most
extreme distributions. As we have proven, the objective is increasing in
$\sigma_t$ for all $t \in \T$ for a fixed $\bm{\mu}$. We also found that the
objective is convex in $\mu_t$ for a fixed $\bm{\sigma}$. The question then
arises of how to combine these results to find the most extreme $\bm{\omega}$
values. Let us define the sets of all distinct $\bm{\mu}$ and $\bm{\sigma}$
vectors as $M$ and $S$. I.e.
\begin{align}
    M &= \l\{\bm{\mu} \in \R^T \ | \ \exists \ \bm{\sigma} \in \R^T: (\bm{\mu}, \bm{\sigma}) \in \Omega\r\}\\
    S &= \l\{\bm{\sigma} \in \R^T \ | \ \exists \ \bm{\mu} \in \R^T: (\bm{\mu}, \bm{\sigma}) \in \Omega\r\}.
\end{align}
From $M$ and $S$ we can extract the most extreme $\bm{\mu}$'s and the most
extreme $\bm{\sigma}$'s individually using the results we found from the
derivatives of the objective. To be more specific, we would take those
$\bm{\sigma}$ that maximise $\sum_{t=1}^T \sigma_t$, since these are the
$\bm{\sigma}$ that do not have any $\sigma_t$'s that can be increased further.
We would also look for $\bm{\mu}$'s that have some or all days equal to their
maximum or minimum values. However, it may not be feasible for these extreme
$\bm{\mu}$ and extreme $\bm{\sigma}$ to occur at the same time, in the same way
that it may not be possible for all $\sigma_t$'s to be maximised together. It is
difficult to see how to extract the extreme distributions.

In order to do this, we might consider using two steps. Firstly, for each
$\bm{\mu}$ we can find the $\bm{\sigma}$ with the largest sum. This corresponds
to finding the most extreme distribution if $\bm{\mu}$ is fixed, and can be seen
as eliminating dominated distributions. We define the set:
\begin{equation} \label{eq:dominated_sigmas}
    \Omega^{\text{ext}}_1 = \l\{(\bm{\mu}, \bm{\sigma}) \in \Omega: \sum_{t=1}^T \sigma_t = \max_{(\bm{\mu}, \tilde{\bm{\sigma}}) \in \Omega} \sum_{t=1}^T \tilde{\sigma}_t\r\}.
\end{equation}
This step corresponds to eliminating dominated $\bm{\sigma}$ for each
$\bm{\mu}$. The second step eliminates pairs from $\Omega^{\text{ext}}_1$ where
$\bm{\mu}$ is dominated when the corresponding $\bm{\sigma}$ is fixed. We can
characterise this by finding the maximum and minimum for each $\mu_t$
conditional on $\bm{\sigma}$. Then, we can remove any pairs from
$\Omega^{\text{ext}}_1$ that do not have any $\mu_t$ equal to their maximum or
minimum. 
\begin{align}
    \mu^{\max}_t(\bm{\sigma}) = \max_{(\bm{\tilde{\mu}}, \bm{\sigma}) \in \Omega^{\text{ext}}_1} \tilde{\mu}_t\\
    \mu^{\min}_t(\bm{\sigma}) = \min_{(\bm{\tilde{\mu}}, \bm{\sigma}) \in \Omega^{\text{ext}}_1} \tilde{\mu}_t 
\end{align}
\begin{equation} \label{eq:dominated_mus}
    \Omega^{\text{ext}}_2 = \l\{(\bm{\mu}, \bm{\sigma}) \in \Omega^{\text{ext}}_1 \ | \
    \exists t \in \T: \mu_t \in \{\mu^{\min}_t(\bm{\sigma}), \mu^{\max}_t(\bm{\sigma})\}\r\}.
\end{equation}
We can write this in a simpler form as a single set using~\eqref{eq:extreme_distributions}.
\begin{equation}\label{eq:extreme_distributions}
    \Omega^{\text{ext}} = \l\{(\bm{\mu}, \bm{\sigma}) \in \Omega \ \Bigg |\ \l(\sum_{t=1}^T \sigma_t = \max_{(\bm{\mu}, \tilde{\bm{\sigma}}) \in \Omega} \sum_{t=1}^T \tilde{\sigma}_t\r) \land \l(\exists t \in \T: \mu_t \in \{\mu^{\min}_t(\bm{\sigma}), \mu^{\max}_t(\bm{\sigma})\}\r)\r\}
\end{equation}

\subsection{Cutting Surface Algorithm}\label{sec:normal_CS}

The cutting surface algorithm for this problem is as follows. 
\begin{enumerate}
    \item Initialise by choosing initial set of one distribution $\Omega^0 =
    \{\bm{\omega}^0\}$, optimality tolerance $\varepsilon$, $k^{\max}$, and the
    gap $\delta$ between successive $z$ points for the piecewise linear
    approximation.
    \item Construct set of extreme distributions $\Omega^{\text{ext}}$ using~\eqref{eq:extreme_distributions}.
    \item Set $k=0$.
    \item While $k \le k^{\max}$:
    \begin{enumerate}
        \item Solve piecewise linear approximation to the DRO model, i.e.\ the
        model in~\eqref{eq:DRO_PWL_obj}-\eqref{eq:DRO_PWL_lastconstraint} using
        the set $\Omega^k$, to get solution $(\bm{q}^k, \tilde{\bm{\omega}})$.
        \item Use true objective function to find objective value $\theta^k = C_{\tilde{\bm{\omega}}}(\bm{q}^k)$.
        \item Fixing $\bm{q} = \bm{q}^k$, evaluate the expected costs
        $C_{\bm{\omega}}(\bm{q}^k)$ for $\bm{\omega} \in \Omega^{\text{ext}}$.
        \item Find worst-case cost $C^k = \max_{\bm{\omega} \in
        \Omega^{\text{ext}}} C_{\bm{\omega}}(\bm{q}^k)$ and worst-case
        distribution $\bm{\omega}^k \in \argmax_{\bm{\omega} \in
        \Omega^{\text{ext}}} C_{\bm{\omega}}(\bm{q}^k)$.
        \item If $C^k \le \theta^k + \frac{\varepsilon}{2}$ or $\bm{\omega}^k \in
        \Omega^k$ then set $k=k^{\max}$. 
        \item Else set $\Omega^{k+1} = \Omega^k \cup \{\bm{\omega}^k\}$ and $k =
        k+1$.
    \end{enumerate}
    \item Return solution $(\bm{q}^k, \bm{\omega}^k)$. 
\end{enumerate}
Note that, in step 4, CS uses the true objective function to evaluate $y^k$ and to select a worst-case distribution for $y^k$. Since PLA uses the piecewise linear objective function, CS may give stronger solutions than PLA.

% \subsection{Testing CS on a Simple Ambiguity Set}

% \subsubsection{Ambiguity Set}

% We first consider a simple ambiguity set. Suppose that the sets $M$ and $S$ are given by:
% \begin{align}\label{eq:M_S}
%     M &= \{\bm{\mu}: \mu_t \in \{1,\dots,\mu^{\max}_t\} \fa t = 1,\dots,T\}\\
%     S &= \{\bm{\sigma}: \sigma_t \in\{1,\dots,\sigma^{\max}_t\} \fa t = 1,\dots,T\}.
% \end{align}
% Then, the simplest ambiguity set contains all combinations of $\bm{\mu} \in M$ and $\bm{\sigma} \in S$:
% \begin{equation}\label{eq:simple_Omega}
%     \Omega = \{(\bm{\mu}, \bm{\sigma}): \bm{\mu} \in M \land \bm{\sigma} \in S\}.
% \end{equation}
% According to our theoretical results, for any fixed $\bm{\mu}$, the worst-case parameter must have $\bm{\sigma} = \bm{\sigma}^{\max}$. This is possible here since $(\bm{\mu}, \bm{\sigma}^{\max}) \in \Omega$ for any $\bm{\mu}$. Furthermore, the worst-case distribution must have $\mu_t \in \{\mu^{\min}_t, \mu^{\max}_t\}$.

% \subsubsection{Experimental Design and Results}

% Although this ambiguity set is not what would be used in practice, it allows us to test the basic assumptions of our CS algorithm. From here on, we refer to the method of solving the DRO model via the PLA of the model given in~\eqref{eq:DRO_PWL_obj}-\eqref{eq:DRO_PWL_lastconstraint} as PLA. We construct test instances using the following parameters:
% \begin{enumerate}
%     \item $T \in \{2,\dots,4\}$
%     \item $\mu^{\max}_t \in \{1,\dots,4\} \fa t$
%     \item $\sigma^{\max}_t \in \{1,\dots,4\} \fa t$
%     \item $\varepsilon \in \{0.1, 0.01, 0.001\}$
%     \item $p \in \{1,2\}$
%     \item $h \in \{1,2\}$
%     \item $b \in \{1,2\}$
%     \item $W = 40$
% \end{enumerate}
% Based on these inputs, solved 894 instances with both CS and the PLA. For these instances, we summarise the results below. Firstly, we present the average times taken by each method. Table~\ref{tab:CP_times_by_T} shows the average times taken by CS and the PLA. This shows that the PLA scales very poorly with $T$. Even for $T=4$, the PLA takes 1 hour and 17 minutes to finish running. This is almost 1 hour longer than PLA took for $T=2$. CS, on the other hand, takes only 4 minutes and 38 seconds. This is only 2 minutes and 24 seconds longer than CS took when $T=2$. 
% \begin{table}[htbp!]
%     \centering
%     \input{images_tables/CP_times_by_T}     
%     \caption{Average times taken by $T$ for simple ambiguity set.}   
%     \label{tab:CP_times_by_T}
% \end{table}
% We also report the times taken by $\varepsilon$. This parameter gives the gap between the $z_i$ values used for the piecewise linear approximation of the objective. Higher values of $\varepsilon$ leads to a better approximation at the cost of more complex constraints. The results indicate that smaller $\varepsilon$ leads to greatly increase solution times for both methods. For PLA, when $\varepsilon=0.001$, the average time taken exceeds two hours. For CS, the average time here is only 9 minutes, but this is much slower than its average time of 6 seconds when $\varepsilon = 0.1$.
% \begin{table}[htbp!]
%     \centering
%     \input{images_tables/CP_times_by_gap}
%     \caption{Average times taken by $\varepsilon$ for simple ambiguity set.}
%     \label{tab:CP_times_by_gap}
% \end{table}

% We also present the number of times that CS found the worst-case parameter for its chosen $\bm{q}$. This is done by brute-force evaluation of the true expected cost for every $\bm{\omega} \in \Omega$. We can confirm that both CS and PLA found the worst-case parameter for their chosen $\bm{q}$ in \textbf{every instance}. This indicates that using a PLA of the objective function does not hinder the algorithms' selection of the worst-case parameter.

% With respect to selecting $\bm{q}$, can compare the true worst-case cost of CS's solution with that of PLA. Figure~\ref{fig:obj_diff_by_T_CP} shows the objective differences by $T$. The difference is obtained by subtracting CS's objective value from PLA's. This boxplot indicates that both methods produce very similar decisions for all $T$. In general, it also indicates that CS performs slightly worse than PLA for all $T$. Figure~\ref{fig:obj_diff_by_eps_CP} suggsets that the same holds for $\varepsilon$. However, the differences are very small in general, and CS offers a significant reduction in solution times.
 
% \begin{figure}[htbp!]
%     \centering
%     \begin{subfigure}[t]{0.45\textwidth} \centering
%         \includegraphics[width=\textwidth]{images_tables/CP_obj_diff_by_T.png}
%         \caption{Boxplot of objective difference by $T$}
%         \label{fig:obj_diff_by_T_CP}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{images_tables/CP_obj_diff_by_gap.png} 
%         \caption{Boxplot of objective difference by $\varepsilon$}
%         \label{fig:obj_diff_by_eps_CP}
%     \end{subfigure}
%         \caption{Boxplots of objective difference}
%     \label{fig:obj_diff_CP}
%     % \caption{}
% \end{figure}

\subsection{Confidence Sets for the True Parameters}

Suppose that the true demand distribution for day $t$ is given by $N(\mu^0_t, (\sigma^0_t)^2)$ and that we have access to $N$ samples, $\bm{x}^n = (x^n_1,\dots,x^n_T) \ (n=1,\dots,N)$, from the true demand distribution. We can use these samples to create MLEs of the parameters $\hat{\bm{\mu}} = (\hat{\mu}_1,\dots,\hat{\mu}_T)$ and $\hat{\bm{\sigma}} = (\hat{\sigma}_1,\dots,\hat{\sigma}_T)$. The likelihood function for the data is:
\begin{align*}
    \m{L}(\bm{x}|\bm{\omega}) &= \prod_{n=1}^N f_{\bm{X}}(\bm{x}| \bm{\omega}) \\
    &= \prod_{n=1}^N \prod_{t=1}^T \frac{1}{\sigma_t\sqrt{2\pi}}\exp\l(-\frac{1}{2\sigma^2_t}(x^n_t - \mu_t)^2\r)\\
    &\propto \l(\prod_{t=1}^T(\sigma_t)^{-1}\r)^N \times \exp\l(-\sum_{n=1}^N\sum_{t=1}^T\frac{1}{2\sigma^2_t}(x^n_t - \mu_t)^2\r).
\end{align*}
The log-likelihood is:
\begin{align*}
    \ell(\bm{\omega}) &= -N \sum_{t=1}^T \log(\sigma_t) - \sum_{n=1}^N\sum_{t=1}^T \frac{1}{2\sigma^2_t}(x^n_t - \mu_t)^2.
\end{align*}
Taking derivatives, we find:
\begin{align*}
    \pderiv{\ell(\bm{\omega})}{\mu_t} &= \frac{1}{\sigma^2_t}\sum_{n=1}^N (x^n_t - \mu_t) \\
    \pderiv{\ell(\bm{\omega})}{\sigma_t} &= -\frac{N}{\sigma_t} + \frac{1}{\sigma^3_t}\sum_{n=1}^N (x^n_t - \mu_t)^2 \\
    \frac{\partial^2 \ell(\bm{\omega})}{\partial \mu_t \partial \sigma_t} &= -\frac{2}{\sigma^3_t}\sum_{n=1}^N(x^n_t - \mu_t) \\
    \frac{\partial^2 \ell(\bm{\omega})}{\partial \mu^2_t} &= -\frac{N}{\sigma^2_t} \\
    \frac{\partial^2 \ell(\bm{\omega})}{\partial \sigma_t \partial \mu_t} &= -\frac{2}{\sigma^3_t}\sum_{n=1}^N(x^n_t - \mu_t) \\
    \frac{\partial^2 \ell(\bm{\omega})}{\partial \sigma^2_t} &= \frac{N}{\sigma^2_t} - \frac{3}{\sigma^4_t}\sum_{n=1}^N(x^n_t - \mu_t)^2,
\end{align*}
and all other second partial derivatives are zero. As expected, this yields the MLEs:
\begin{align}
    \hat{\mu}_t &= \frac{1}{N}\sum_{n=1}^N x^n_t \label{eq:mu_MLE} \\
    \hat{\sigma}_t &= \sqrt{\frac{1}{N} \sum_{n=1}^N (x^n_t - \hat{\mu}_t)^2}.\label{eq:sig_MLE}
\end{align}
The expected values of these expressions are given by:
\begin{align*}
    \E\l(\frac{\partial^2 \ell(\bm{\omega})}{\partial \mu_t \partial \sigma_t}\r) &= 0 \\
    \E\l(\frac{\partial^2 \ell(\bm{\omega})}{\partial \mu^2_t}\r) &= -\frac{N}{\sigma^2_t} \\
    \E\l(\frac{\partial^2 \ell(\bm{\omega})}{\partial \sigma_t \partial \mu_t}\r) &= 0 \\
    \E\l(\frac{\partial^2 \ell(\bm{\omega})}{\partial \sigma^2_t}\r) &= \frac{-2N}{\sigma^2_t}.
\end{align*}
Therefore, the Fisher information matrix is given by:
\begin{align}
    I_{\E}(\bm{\omega}) &= \begin{pmatrix}
        \frac{N}{\sigma^2_1} & 0 & \dots & \dots & \dots &\dots & \dots & 0 \\
        0 & \frac{N}{\sigma^2_2} & 0 & \dots & \dots & \dots & \dots &  0 \\
        \vdots &  & \ddots & & & & & \vdots \\
        0 & \dots & 0 & \frac{N}{\sigma^2_T} & 0   & \dots& \dots & 0 \\
        0 & \dots & \dots & 0 & \frac{2N}{\sigma^2_1} & 0 & \dots & 0 \\
        0 & \dots & \dots & \dots & 0 & \frac{2N}{\sigma^2_2}  & \dots & 0 \\
        \vdots & & & & &  &\ddots & \vdots \\
         0 & \dots & \dots & \dots & \dots & \dots & 0 &   \frac{2N}{\sigma^2_T}\\
    \end{pmatrix}
\end{align}
Hence, we have that (for large $N$):
\begin{equation}
    (\hat{\bm{\omega}} - \bm{\omega}^0)I_{\E}(\hat{\bm{\omega}})(\hat{\bm{\omega}} - \bm{\omega}^0)^T \sim \chi^2_{2T}
\end{equation}
or, equivalently:
\begin{equation}
    \sum_{t=1}^T\l(\frac{N}{\hat{\sigma}^2_t}\l(\hat{\mu}_t - \mu^0_t\r)^2 + \frac{2N}{\hat{\sigma}^2_t}\l(\hat{\sigma}_t - \sigma^0_t\r)^2\r) \sim \chi^2_{2T}.
\end{equation}
Thus, given a discrete set $\Omega$ of potential values for $\bm{\omega}$, we can create a discrete subset of an approximate $100(1-\alpha)\%$ confidence set for $\bm{\omega}^0$ using~\eqref{eq:normal_conf}.
\begin{equation}\label{eq:normal_conf}
    \Omega_{\alpha} = \l\{(\bm{\mu}, \bm{\sigma}) \in \Omega: \sum_{t=1}^T\l(\frac{N}{\hat{\sigma}^2_t}\l(\hat{\mu}_t - \mu_t\r)^2 + \frac{2N}{\hat{\sigma}^2_t}\l(\hat{\sigma}_t - \sigma_t\r)^2\r) \le \chi^2_{2T, 1-\alpha} \r\}.
\end{equation}
In order to construct~\eqref{eq:normal_conf}, we first need a discrete baseline ambiguity set $\Omega$ such that $\Omega_\alpha \subseteq \Omega$. There is no immediate way to create this. For example, we could do this in a simple fashion by defining a range $\{1,\dots,\mu^{\max}_t\}$ for each $\mu_t$ and similarly for each $\sigma_t$ and then use a Cartesian product. However, not only will this set be very large but it also may not be a fine enough discretisation to ensure that some values in $\Omega_\alpha$ are in $\Omega$. A more logical way in which to construct $\Omega$ is as follows. Given that $\hat{\mu}_t$ and $\hat{\sigma}_t$ are asymptotically normal, we can create approximate confidence intervals for these parameters individually:
\begin{align}
    \mu^{CI}_t = \l\{\mu_t: \hat{\mu}_t - z_{1-\frac{\alpha}{2}}\frac{\hat{\sigma}_t}{\sqrt{N}} \le \mu_t \le \hat{\mu}_t + z_{1-\frac{\alpha}{2}}\frac{\hat{\sigma}_t}{\sqrt{N}}\r\} \\
    \sigma^{CI}_t = \l\{\sigma_t: \hat{\sigma}_t - z_{1-\frac{\alpha}{2}}\frac{\hat{\sigma}_t}{\sqrt{2N}} 
    \le \sigma_t \le \hat{\sigma}_t + z_{1-\frac{\alpha}{2}}\frac{\hat{\sigma}_t}{\sqrt{2N}} \r\}
\end{align}
We could then create a baseline ambiguity set $\Omega$ that only contains $\bm{\omega}$ such that all elements lie in their corresponding confidence intervals. Let us refer to the upper and lower boundaries of the individual confidence intervals as $\mu^l_t, \mu^u_t$ and $\sigma^l_t, \sigma^u_t$ for each $t = 1,\dots,T$. Then, we can create discretised confidence intervals of the form:
\begin{align}
    \tilde{\mu}^{CI}_t = \l\{\mu^l_t + m\frac{\mu^u_t - \mu^l_t}{M - 1}, \quad m = 0,\dots, M - 1 \r\} \\
    \tilde{\sigma}^{CI}_t = \l\{\sigma^l_t + m\frac{\sigma^u_t - \sigma^l_t}{M - 1}, \quad m = 0,\dots,M-1
    \r\},
\end{align}
for some discretisation parameter $M$. This creates a discretisation of each interval, each containing $M$ values. Then we can take a baseline ambiguity set of the form:
\begin{equation}\label{eq:normal_base}
    \Omega = \l\{(\bm{\mu}, \bm{\sigma}): \mu_t \in \tilde{\mu}^{CI}_t \land \sigma_t \in \tilde{\sigma}^{CI}_t \fa t = 1,\dots,T\r\}.
\end{equation}
Then, the set given by~\eqref{eq:normal_conf} can be viewed as a discrete subset of the approximate 95\% confidence set, containing $\bm{\omega}$ such that each univariate parameter would pass a univariate hypothesis test at the 5\% level, and that $\bm{\omega}$ itself would pass a multivariate hypothesis test at the 5\% level. This ensures that $\bm{\omega}$ is a realistic vector and also that each individual parameter is realistic when studied alone.

\input{5_results}

==> A_oneperiod.tex <==
\section{One-period Newsvendor Model}

\subsection{Model and Distributionally Robust Model}

As given by~\cite{ANDREWBUTTERS2019}, the one-period newsvendor problem can be
defined as follows. At the start of the period, the newsvendor must decide on
the number of units $q$ of stock to order at a unit price of $w$. The retail
price per unit of stock is $p$. We assume that demand $X$ for the product is
unknown at the time of decision making, but that it is a non-negative random
variable (RV) distributed according to a cumulative distribution function (CDF)
$F:[0, \infty) \to [0,1]$. For demand realisations $x$ of demand $X$, if $x > q$
then $q$ units are sold. If $x \le q$ then $x$ units are sold and $q - x$ are
lost. Then, the newsvendor must choose $q$ to maximise expected profits via
solving the following stochastic model:
\begin{equation}
    \max_{q} \E_F[\pi(q)] = \int_{0}^q px \ \text{d}F(x) + \int_{q}^{\infty} pq\ \text{d}F(x) - wq,
\end{equation}
where $\int_{0}^q px \ \text{d}F(x) + \int_{q}^{\infty} pq \ \text{d}F(x)$ is
the expected return and $wq$ is the cost of the units ordered. We can also write
$\E_F[\pi(q)]$ as:
\begin{align}
    \E_F[\pi(q)] &= p\int_0^{\infty} \min(q, x) \text{d}F(x) - wq \\
    &= p\E_F[\min(q, X)] - wq.
\end{align}
As found by~\cite{Newsboy1}, the optimal solution of this problem for a fixed
distribution with CDF $F$ is given by:
\begin{equation}
    q_F = F^{-1}\l(1-\frac{w}{p}\r).
\end{equation}
In the DRO model, we do not make the assumption that the cumulative distribution  function (CDF) $F$ is  known but that $F$ lies in some set $\m{F}$. The distributionally robust model is given in~\eqref{eq:robust_news}.
\begin{equation}\label{eq:robust_news}
    \max_q \min_{F\in\m{F}} \E_F[\pi(q)].
\end{equation}

\subsection{Distribution-free Solution}

As referenced earlier, the distribution-free model~\citep{oneperiodrobustsol} is the model given in~\eqref{eq:robust_news} where $\m{F} = \{F: \E_F(X) = \mu,  \text{Var}_F(X) = \sigma^2\}$. The solution to this problem is:
\begin{equation}
    q^* = \begin{cases}
        0 &\text{ if } \frac{w}{p}\l(1+\frac{\mu^2}{\sigma^2}\r) > 1\\
        \mu + \frac{\sigma}{2}\frac{1-\frac{2w}{p}}{\sqrt{\frac{2w}{p}\l(1-\frac{w}{p}\r)}} &\text{ otherwise.}
    \end{cases}
\end{equation}


\subsection{Distributionally Robust Model with Normal Demand}\label{sec:DRNVP}

Let us not assume that $F$ is known but assume that $X \sim N(\mu, \sigma^2)$
for some \textbf{unknown} mean and some \textbf{unknown} variance $\sigma^2$.
Suppose that we have a set $\Omega$ of parameter pairs $\omega = (\mu,
\sigma^2)$ such that each $\omega$ uniquely defines a normal distribution. We
can write the DRNVP as:
\begin{equation}\label{eq:normal_robust_news}
    \max_q \min_{\omega \in \Omega} \E_{\bm{\omega}}[\pi(q)],
\end{equation}
and we have:
\begin{align}
    \E_{\bm{\omega}}[\min(q, X)] &= \E_{\bm{\omega}}(X | X \le q)\P(X\le q) +  q \P(q < X) \\
    &= \E_{\bm{\omega}}(X|X \le q)F(q) + q(1-F(q)).
\end{align}
Using the mean and variance of a normal distribution truncated above at $q$, we
have:
\begin{equation}
    \E_{\bm{\omega}}(X|X\le q) = \mu - \sigma \frac{\phi(\beta)}{\Phi(\beta)},
\end{equation}
where $\beta =  \frac{q - \mu}{\sigma}$, $\phi$ is the probability density
function (PDF) of the standard normal distribution and $\Phi$ is the CDF of said
distribution. Therefore, we can write:
\begin{align}
    \E_{\bm{\omega}}[\pi(q)] &= p\l[\l(\mu - \sigma\frac{\phi(\beta)}{\Phi(\beta)}\r)
    F(q) + q(1-F(q))\r] - wq \\
    &= p\l[\l(\mu - \sigma\frac{\phi(\beta)}{\Phi(\beta)}\r)\Phi(\beta) + q\Phi(-\beta)\r] - wq \\
    &= p\l[\Phi(\beta)\mu - \sigma\phi(\beta) + q\Phi(-\beta)\r] - wq.
\end{align}

\subsubsection{Derivatives of Objective}\label{sec:NV_derivs}

In order to construct a cutting surface (CS) algorithm for this problem, we must
first study the behaviour of $\E_{\bm{\omega}}[\pi(q)]$ as a function of $\mu$ and
$\sigma$ for a fixed $q$. This will allow us to create a rule for generating a
subset $\tilde{\Omega}$ for use in the distribution separation problem, inside
the CS algorithm. We first study the behaviour as a function of $\mu$. We have:
\begin{align}
    \pderiv{\beta}{\mu} &= -\frac{1}{\sigma},\\
    \pderiv{\phi(\beta)}{\mu} &= \pderiv{\beta}{\mu}\pderiv{\phi(\beta)}{\beta} \\
    &= -\frac{1}{\sigma} \times (-\beta\phi(\beta)) \\
    &= \frac{\beta}{\sigma}\phi(\beta)
\end{align}
and hence:
\begin{align}
    \pderiv{\E_{\bm{\omega}}(\min(q, X))}{\mu} &= \Phi(\beta) + \mu\pderiv{\beta}{\mu}\phi(\beta) - \sigma \pderiv{\phi(\beta)}{\mu} - q\pderiv{\beta}{\mu}\phi(-\beta) \\
    &= \Phi(\beta) - \frac{\mu}{\sigma} \phi(\beta) - \beta\phi(\beta) + \frac{q}{\sigma}\phi(-\beta)\\
    &= \Phi(\beta) - \l(\frac{\mu}{\sigma}+ \beta - \frac{q}{\sigma}\r)\phi(\beta) \\
    &= \Phi(\beta).
\end{align}
Hence, $\E_{\bm{\omega}}(\min(q, X))$ is increasing in $\mu$. We can also analyse the
derivative in $\sigma$ as follows. 
\begin{align}
    \pderiv{\beta}{\sigma} &= \frac{\mu - q}{\sigma^2} = -\frac{\beta}{\sigma},\\
    \pderiv{\phi(\beta)}{\sigma} &= \pderiv{\beta}{\sigma}\pderiv{\phi(\beta)}{\beta} \\
    &= \frac{\mu - q}{\sigma^2} \times (-\beta\phi(\beta)) \\
    &= -\frac{\beta}{\sigma} \times  (- \beta \phi(\beta))\\
    &= \frac{\beta^2}{\sigma}\phi(\beta).
\end{align}
Hence:
\begin{align}
    \pderiv{\E_{\bm{\omega}}(\min(q, X))}{\sigma} &= \mu\pderiv{\beta}{\sigma}\phi(\beta) - \phi(\beta) - \sigma \pderiv{\phi(\beta)}{\sigma} - q\pderiv{\beta}{\sigma}\phi(-\beta) \\
    &= -\frac{\mu \beta}{\sigma}\phi(\beta) - \phi(\beta) -\beta^2\phi(\beta) + \frac{q\beta}{\sigma} \phi(-\beta) \\
    &= \phi(\beta)\l(\frac{q\beta}{\sigma} - \phi(\beta) - \frac{\mu\beta}{\sigma} - \beta^2\r) \\
    &= \phi(\beta)\l(\beta\frac{q-\mu}{\sigma} - 1 - \beta^2\r) \\
    &= \phi(\beta)\l(\beta^2 - 1 - \beta^2\r) \\
    &= - \phi(\beta).
\end{align}
Hence, $\E_{\bm{\omega}}(\min(q, X))$ is decreasing in $\sigma$.

\subsubsection{Extreme Distributions for the Inner Problem}\label{sec:inner}

The results in Section~\ref{sec:NV_derivs} imply that, for a fixed $q$, the
worst-case distribution of demand will have either a mean of $\mu_{\min} =
\min_{({\mu}, {\sigma}) \in \Omega}{\mu}$ or a standard deviation of
$\sigma_{\max} = \max_{({\mu}, {\sigma}) \in \Omega}{\sigma}$ or both. If
$(\mu_{\min}, \sigma_{\max}) \in \Omega$ then the worst case distribution is
given by this choice of parameters. In the cases where it is not, we must
compare distributions arising from $\mu = \mu_{\min}$ and those arising from
$\sigma = \sigma_{\max}$. Therefore, we define the set of extreme parameters
in~\eqref{eq:NV_extremes}:
\begin{equation}\label{eq:NV_extremes}
    \Omega_{\text{ext}} = \l\{(\mu, \sigma) \in \Omega: \mu = \mu_{\min} \lor \sigma = \sigma_{\max}\r\}.
\end{equation}
This is the set that will be used to solve the distribution separation (inner)
problem in the cutting surface algorithm. Solving the outer separation problem,
i.e.\ generating a $q$ solution to solve the DRO problem on some subset of
$\Omega$, is not so simple. 

\subsubsection{Turning Point Approach (Informal Section)}

We have the set of potential worst-case distributions $\Omega_{\text{ext}}$,
which can be reduced down to just two, i.e.\ $\Omega'_{\text{ext}} = \{\omega_1,
\omega_2\}$ where $\omega_1$ has $\mu = \mu_\min$ and $\sigma$ the highest it
can be given this is true, and $\omega_2$ is created similarly but with $\sigma$
the highest it can be. For each $q$, the worst-case distribution is $\omega_q
\in \Omega'_{\text{ext}}$. We aim to find a mapping between $q$ and $\omega_q$
so that we can get a closed form expression for the inner objective for a fixed
$q$. What we discussed is the possibility that there is a ``turning point''
before which one of the distributions is optimal and after which the other one
is. Now we aim to find the turning point, which is (appears to be) the solution
of:
\begin{equation}\label{eq:turning_point}
    \E_{\omega_1}[\pi(q)] = \E_{\omega_2}[\pi(q)].
\end{equation} 
where, in the case of $\Omega$ being defined as in~\eqref{eq:Omega_test}, we
have $\omega_1 = (\mu_\min, \sigma_\max - 1)$ and $\omega_2 = (\mu_\min + 1,
\sigma_\max)$. In Figure~\ref{fig:intersect}, we show the expected profit for
each $q$ in a small range, for each of the two extreme $\omega$ values.

We can see from Figure~\ref{fig:intersect} that to the left of the turning point
the worst-case $\omega$ is $(2,5)$, and to the right it is $(1,4)$. The turning
point can be found by solving~\eqref{eq:turning_point}, which might be
extremely difficult. Note that this function only looks linear because it's over
a small range. We also have examples like in Figure~\ref{fig:dominated}, where
one $\omega$ dominates the other. 
\begin{figure}[htbp!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth} \centering
        \includegraphics[width=\textwidth]{intersection_EV}
        \caption{A case where the intersect is around 0.118}
        \label{fig:intersect}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{dominated_EV}
        \caption{An example of where there is no intersection point}
        \label{fig:dominated}
    \end{subfigure}
    \caption{Expected profit for each $q$, plotted for each extreme $\omega$ in two different instances}
    \label{fig:intersect_plots}
    % \caption{}
\end{figure}

Let's refer to the intersection point as $q^{\text{TP}}$, if it exists. I believe that
finding $q^{\text{TP}}$ is a very hard problem that we cannot solve easily. If we could
find it, it would give us the inner objective. However, I cannot think of a way
to solve~\eqref{eq:turning_point} due to the lack of simplification that can be
done. Attempting to solve this using Sympy yields no results.


\textbf{Numerically Finding Turning Points}

I ran some experiments to try to find the turning points numerically. Due to my
initial results suggesting that the turning point was always the same when it
was positive, I increased the size of the experiments. The values used are as
follows:
\begin{itemize}
    \item $p \in \{1,\dots,10\}$,
    \item $w \in \{1, \dots, 9\}$ with $w < p$,
    \item $\mu_{\min} \in \{0,1\}$,
    \item $\mu_{\max} \in \{\mu_{\min} + 1,\dots, 15\}$,
    \item $\sigma_{\min} = 1$,
    \item $\sigma_{\max} \in \{2, \dots, 15\}$ ($\sigma_{\max} > 1$ because if
    $\sigma_\max = 1$ then problem is trivial).
\end{itemize}
I tested those cases where $\mu_{\min} = 0$ separately as this seems to change
the behaviour. I can summarise the results as below:
\begin{enumerate}
    \item The lines only intersected at some $q^{\text{TP}} \ge 0$ when $\sigma_{\max} \in
    \{1,\dots,5\}$.
    \item The turning point $q^{\text{TP}}$ seems to only depend on $\sigma_{\max}$, and
    there was one turning point for each $\sigma_{\max} \in \{1,\dots,5\}$.
    \item For any other $\sigma_{\max}$ value, one $\omega$ always dominated th
    other. In particular, $(1, \sigma_{\max} - 1)$ dominated $(2, \sigma_\max)$.
    \item If $\mu = 0$ is allowed to be picked, then there is always a dominated
    $\omega$. In particular, $(1, \sigma_{\max})$ dominated when $\sigma_{\max}
    = 1$ and otherwise $(0, \sigma_{\max} - 1)$ dominated. 
\end{enumerate}
Going into the turning points further, we have Figure~\ref{fig:TP_vals}. The
plot suggests that any $\sigma_{\max} > 5$ have $q^{\text{TP}} < 0$. 
\begin{figure}[htbp!]
    \centering
    \includegraphics[width=0.6\textwidth]{TP_vals_all}
    \caption{}
    \label{fig:TP_vals}
\end{figure}
There appears to be a linear relationship between $q^{\text{TP}}$ and $\sigma_{\max}$, but
it is not simple to find $q^{\text{TP}}$.

\subsubsection{Bisection Search Algorithm}

A simple bisection search algorithm can be used to find the turning point. The
algorithm we use is given below. We define, for two pairs of parameters
$\omega_1, \omega_2$, a function:
\begin{equation}
    \Delta(q; \omega_1, \omega_2) = \E_{\omega_1}[\pi(q)] -
    \E_{\omega_2}[\pi(q)]
\end{equation}
and we will find the point at which $\Delta_{\omega_1, \omega_2}(q) = 0$. 
\begin{enumerate}
    \item Initialise parameters $a, b, k_{\max}, \epsilon$ and set $k=0$.
    \item Find the set of the most extreme distributions via the following steps:
    $$\mu_{\text{ext}} = \{(\mu, \sigma) \in \Omega: \mu = \mu_{\min}\},\sigma_{\text{ext}} = \{(\mu, \sigma) \in \Omega: \sigma = \sigma_{\max}\}$$
    $$\Omega'_{\text{ext}} = \argmax_{(\mu, \sigma) \in \mu_{\text{ext}}} \sigma
    \cup \argmin_{(\mu, \sigma) \in \sigma_{\text{ext}}} \mu = \{\omega_1, \omega_2\}.$$
    This means that if $\mu = \mu_\min$ then $\sigma$ is as close to
    $\sigma_{\max}$ as it can be, and similarly for when $\sigma =
    \sigma_{\max}$.
    \item Calculate endpoint differences $\Delta(a; \omega_1, \omega_2)$ and $\Delta(b; \omega_1, \omega_2)$.
    \item Find dominating distributions on each side:
    \begin{enumerate}
        \item If $\sign{\Delta(a; \omega_1, \omega_2)} =
        -1$ then the worst distribution on the left is $\omega_1$. Set
        $\omega^l = \omega_1$. Otherwise $\omega^l = \omega_2$.
        \item If $\sign{\Delta(b; \omega_1, \omega_2)} =
        -1$ then the worst distribution on the right is $\omega_1$. Set
        $\omega^r = \omega_1$. Otherwise $\omega^r = \omega_2$.
    \end{enumerate} 
    \item If $\omega^l = \omega^r$ then set $q^{\text{TP}} = 0$ indicating there is no
    positive turning point, and go to 8. Else, set $c = \frac{a+b}{2}$ and go to
    5.
    \item While $\frac{b-a}{2} \ge \epsilon$ and $k < k_{\max}$:
    \begin{enumerate}
        \item Set $c = \frac{a+b}{2}$.
        \item Calculate $\Delta(x; \omega_1, \omega_2)$ for $x \in \{a,b,c\}$.
        \item If $\sign{\Delta(c; \omega_1, \omega_2)} = \sign{\Delta(a;
        \omega_1, \omega_2)}$ then set $a = c$.
        \item If $\sign{\Delta(c; \omega_1, \omega_2)} = \sign{\Delta(b;
        \omega_1, \omega_2)}$ then set $b = c$.
        \item If $\Delta(c; \omega_1, \omega_2) = 0$ then break.
        \item Set $k = k + 1$.
    \end{enumerate}
    \item If $k < k_{\max}$ then $q^{\text{TP}} = c$. Else $q^{\text{TP}} = \text{``NA''}$.
    \item Return $q^{\text{TP}}$, $\omega^l$, $\omega^r$.
\end{enumerate}

\subsubsection{Turning Point Solver}

We can use the bisection algorithm to create a solver for this problem. In order
to see the justification for this, we observe Figure~\ref{fig:TP_examples}.
\begin{figure}[htbp!]
    \centering
    \begin{subfigure}[t]{0.40\textwidth} \centering
        \includegraphics[width=\textwidth]{TP_between_peaks}
        \caption{A case where the intersect is between the individual peaks}
        \label{fig:intersect_between_peaks}
    \end{subfigure}
    \begin{subfigure}[t]{0.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{TP_after_peaks}
        \caption{A case where the intersect is after the individual peaks}
        \label{fig:intersect_after_peaks}
    \end{subfigure}
    \caption{Expected profit for each $q$, plotted for each extreme $\omega$ in two different instances}
    \label{fig:TP_examples}
    % \caption{}
\end{figure}

Figure~\ref{fig:intersect_between_peaks} shows an example where $q^{\text{TP}}$
is between the optimal solutions for the individual distributions. In this case,
we see that the worst-case cost on the left of $q^{\text{TP}}$ lies on
$\omega_2$'s line and to the right it lies on $\omega_1$'s line. It is clear
that $q^{\text{TP}}$ has the highest worst-case expected cost. However,
Figure~\ref{fig:intersect_after_peaks} shows a case where this is not the case.
The worst-case distributions on either side are the same, but $q^{\text{TP}}$
has the a lower worst-case cost than both of the two optimal solutions. It is
clear here that the $q$ with the best worst-case expected cost is the optimal
solution when the distribution is $\omega_2$. This would then be given by
$F^{-1}_{\omega_2}\l(1-\frac{w}{p}\r)$. Hence, in our solver we need to check
whether $q^{\text{TP}}$ lies between the two peaks or not.

The bisection solver algorithm is given below.
\begin{enumerate}
    \item Use the bisection search algorithm to find $q^{\text{TP}}$, $\omega^l$, $\omega^r$.
    \item If $\omega^l = \omega^r$ or $q^{\text{TP}} \le 0$ then $\omega^{\text{opt}}
    = \omega^l$ and $q^{\text{opt}} = 0$ and go to 6. Else proceed to 3.
    \item Calculate individual optimal solutions:
    \begin{align}
        q^l &= F^{-1}_{\omega^l}\l(1-\frac{w}{p}\r)\\
        q^r &= F^{-1}_{\omega^r}\l(1-\frac{w}{p}\r).
    \end{align}
    \item If $q^l \le q^{\text{TP}} \le q^r$ then $q^{\text{opt}} = q^{\text{TP}}$ and we are
    indifferent, so set $\omega^{\text{opt}} = \omega^l$ and go to 6. Else
    proceed.
    \item If $q^l \le q^{\text{TP}}$ and $q^r \le q^{\text{TP}}$ then the optimal solution lies on
    the left so set $q^{\text{opt}} = q^l$ and $\omega^{\text{opt}} = \omega^l$.
    Else set $q^{\text{opt}} = q^r$ and $\omega^{\text{opt}} = \omega^r$.
    \item Return $q^{\text{opt}}$ and $\omega^{\text{opt}}$.
\end{enumerate}

\subsubsection{Brute-force Algorithm}\label{sec:brute_force}

\begin{enumerate}
    \item Find a discrete set containing candidate solutions for $q$, for
    example take some step-size $j$ and maximum value $Q$ and take the set:
    \begin{equation}\label{eq:Q_BF}
        \m{Q} = \l\{j, 2j, 3j, \dots, \l\lfloor \frac{Q}{j}\r\rfloor j\r\}.
    \end{equation}
    \item For $q \in \m{Q}$:
    \begin{enumerate}
        \item Compute $\E_\omega[\pi(q)]$ for each $\omega \in \Omega$.
        \item Find worst-case profit, $\min_{\omega}\E_\omega[\pi(q)]$, and
        worst-case distribution $\omega^q = \argmin_{\omega}\E_\omega[\pi(q)]$.
    \end{enumerate}
    \item Find $q^* = \argmax_{q \in \m{Q}} \E_{\omega^q}[\pi(q)]$. 
    \item Return $q^*$, $\omega^{q^*}$, $\E_{\omega^{q^*}}[\pi(q^*)]$.
\end{enumerate}


\subsubsection{Testing the Turning Point Solver}

We use a combinatorial set of 8820 problems. The results from the bisection
solver are compared with the results of the brute-force algorithm of
Section~\ref{sec:brute_force} using the candidate set defined in~\eqref{eq:Q_BF}
with $j = 0.001$ and $Q = 20$. For given values of $\mu_\min$, $\mu_\max$,
$\sigma_\min$, $\sigma_\max$, we define $\Omega$ using~\eqref{eq:Omega_test}.
\begin{equation}\label{eq:Omega_test}
    \Omega = \{(\mu, \sigma): \mu \in \{1,\dots,\mu_{\max}\}, \sigma \in \{1,\dots,\sigma_{\max}\}\} \setminus \{(\mu_\min, \sigma_\max)\}.
\end{equation} 
The parameters used to test the algorithms are given below.
\begin{itemize}
    \item $p \in \{1,\dots,10\}$,
    \item $w \in \{1, \dots, 9\}$ with $w < p$,
    \item $\mu_\min = 1$ and $\sigma_\min = 1$,
    \item $\mu_{\max} \in \{\mu_\min + 1,\dots,15\}$,
    \item $\sigma_{\max} \in \{\sigma_\min + 1, \dots, 15\}$,
    \item $k_{\max} = 1000$,
    \item $\epsilon = 10^{-6}$,
    \item $a = 0$ and $b = 30$.
\end{itemize}
We round the turning points to 3 decimal places to align with the decimal places
of elements in $\m{Q}$. We choose whether to round up or down by comparing the
two resulting two solutions and seeing which has the highest worst-case cost.
This is to avoid rounding causing a difference between solutions where there
shouldn't be.

\large{\textbf{Results}}
\normalsize

The results can be summarised as follows:
\begin{enumerate}
    \item In every instance of 8820, the bisection solver algorithm returned the
    same $q$ solution as the brute force algorithm.
    \item The bisection solver returned a different $\omega$ in 98 instances,
    but these instances were those where the turning point was optimal and so
    both extreme distributions were the worst.
    \item In all cases, the brute force algorithm returned one of the two
    extreme distributions used by the bisection solver. 
    \item The brute force algorithm took 690 seconds (11 min 30 sec) on average.
    \item The bisection solver algorithm took 0.026 seconds on average.
\end{enumerate}

\subsection{CS Algorithm for One-period Newsvendor Problem}

    \subsection{Solving The Outer Problem}

At the first iteration, where we have a set
of parameters $\Omega_0 = \{\omega_0\} = \{(\mu_0, \sigma_0)\}$, we know the
solution to be $q_0 = F_{\omega_0}^{-1}\l(1-\frac{w}{p}\r)$, where
$F_{\omega_0}$ is the CDF of $N(\mu_0, \sigma_0^2)$. This first iteration is
simple. Now consider iteration $k$ with ambiguity set $\Omega_{k-1}$. We are
solving:
\begin{equation}\label{eq:CS_kth_problem}
    \max_q \min_{\omega \in \Omega_{k-1}} \E_{\omega}[\pi(q)].
\end{equation}
Now let $F_\omega$, where $\omega = (\mu, \sigma)$, be the CDF of $N(\mu,
\sigma^2)$. For each $\omega$ in $\Omega_{k-1}$, the optimal solution in $q$ is
$\max\l(F^{-1}_{\omega}\l(1-\frac{w}{p}\r), 0\r)$ if $\omega$ is fixed.  We take
the maximum between the inverse CDF and zero because if the inverse CDF is
negative then this means the expected profit is decreasing for all $q \ge 0$ and
so the maximum over $\R^+$ occurs when $q = 0$. Assuming $q_k$ is the DRO
solution of the problem at iteration $k$, then we have found $\tilde{\omega}$
such that:
\begin{equation}\label{eq:omega_worst}
    \tilde{\omega} = \argmin_{\omega \in \Omega_{k-1}} \E_{\omega}[\pi(q_k)]
\end{equation}
i.e.\ $\tilde{\omega}$ is the worst-case distribution for $q_k$. Then, does this
mean that:
\begin{equation}\label{eq:q_best}
    q_k = \argmax_q \E_{\tilde{\omega}}[\pi(q)]
\end{equation}
is also true? If it is, then we must have $q_k =
\max\l(F^{-1}_{\tilde{\omega}}\l(1-\frac{w}{p}\r), 0\r)$.
Hence, to find the optimal solution we would just have to search in the set:
\begin{equation}\label{eq:Q_k}
    \m{Q}_k = \l\{q : q=\max\l\{F^{-1}_{\omega}\l(1-\frac{w}{p}\r),
    0\r\} \text{ for some } \omega \in \Omega_{k-1}\r\}.
\end{equation}
Note that we take the maximum between the inverse CDF value and zero because if
it is optimal to order negative units then the best we can do is order 0.

\textbf{
What I am wondering here is that if $(q, \tilde{\omega})$ is the DRO solution of
the model, then we know $\tilde{\omega}$ is the worst-case distribution for $q$,
but is $q$ the profit-maximising solution for some fixed $\omega$?  I made the
CS algorithm assuming the optimal was always satisfying~\eqref{eq:q_best}
and~\eqref{eq:omega_worst}.}
% \textbf{(not sure this is actually true now)}
% which must mean that $q_k = F^{-1}_{\tilde{\omega}}\l(1-\frac{w}{p}\r)$. Hence,
% when searching for the optimal solution to the outer problem, we only need to
% consider solutions in the set:
% \begin{equation}
%     \m{Q}_k = \l\{q : q=\max\l\{F^{-1}_{\omega}\l(1-\frac{w}{p}\r),
%     0\r\} \text{ for some } \omega \in \Omega_{k-1}\r\}.
% \end{equation}
% This can be used to solve the full problem, although it may be somewhat slow.

% \textbf{Notes to Chris and Vikram:} 
% \begin{enumerate}
%     \item This set originally contained $q\in \R^+$ such that $q =
%     F^{-1}_{\omega}\l(1-\frac{w}{p}\r)$ for some $\omega \in \Omega_{k-1}$ but I
%     was getting cases where the solution returned by CS was positive, where the
%     optimal solution was zero. This happened in cases where the worst-case
%     distribution gave $F^{-1}_{\omega}\l(1-\frac{w}{p}\r) < 0$ and so this
%     distribution was not considered in $\m{Q}_k$. It seems as though in cases
%     where the worst-case distribution gives negative $q$ via the inverse CDF,
%     that the optimal solution is then zero.
%     \item After doing some more initial testing, it seems as though it is not
%     the case that the optimal solution is $q =
%     F^{-1}_{\omega}\l(1-\frac{w}{p}\r)$ for some $\omega \in \Omega_{k-1}$. This
%     is because $q$ is not the best $q$ for a fixed distribution.
% \end{enumerate}

\subsection{CDF-Based Heuristic}

We can define a set $\m{Q}$ of candidate solutions using~\eqref{eq:Q_k}, applied
to all distributions in $\Omega$.
\begin{equation}\label{eq:Q_CDFs}
    \m{Q} = \l\{q: q=\max\l\{F^{-1}_{\omega}\l(1-\frac{w}{p}\r),
    0\r\} \text{ for some } \omega \in \Omega\r\}.
\end{equation}
 Then, a brute force approach to solving the DRNVP is as follows.
\begin{enumerate}
    \item Find the set $\m{Q}$ as in~\eqref{eq:Q_CDFs}.
    \item For $q \in \m{Q}$:
    \begin{enumerate}
        \item Compute $\E_\omega[\pi(q)]$ for each $\omega \in \Omega$.
        \item Find worst-case profit, $\min_{\omega}\E_\omega[\pi(q)]$, and
        worst-case distribution $\omega^q = \argmin_{\omega}\E_\omega[\pi(q)]$.
    \end{enumerate}
    \item Find $q^* = \argmax_{q \in \m{Q}} \E_{\omega^q}[\pi(q)]$. 
    \item Return $q^*$, $\omega^{q^*}$, $\E_{\omega^{q^*}}[\pi(q^*)]$.
\end{enumerate}

\subsection{Cutting Surface Algorithm}

Based on the results from previous sections, we have the following
cutting surface algorithm for the DRNVP. Here, we define $\varepsilon$ as the
optimality tolerance for the algorithm, and $k_{\max}$ as the maximum number of
iterations of the algorithm that we run.
\begin{enumerate}
    \item Initialise parameters $\omega_0, w, p, \varepsilon, k_{\max}$ and set $\Omega_0
    = \{\omega_0\}$ and $k=1$.
    \item While $k \le k_{\max}$:
    \begin{enumerate}
        \item Solve outer problem $\max_q \min_{\omega \in \Omega_{k-1}} \E_{\omega}[\pi(q)].$
        \begin{enumerate}
            \item Find a set $\m{Q}_k$ of candidate solutions, either using the
            inverse CDF approach from~\eqref{eq:Q_k} or the brute force approach
            from~\eqref{eq:Q_BF}.  
            % $$\m{Q}_k = \l\{q:
            % q=\max\l\{F^{-1}_{\omega}\l(1-\frac{w}{p}\r), 0\r\} \text{ for some
            % } \omega \in \Omega_{k-1}\r\}.$$
            \item For $q \in \m{Q}_k$:
            \begin{enumerate}
                \item Compute $\E_\omega[\pi(q)]$ for each $\omega \in \Omega_{k-1}$.
                \item Find worst-case profit $\min_{\omega}\E_\omega[\pi(q)]$ and
                worst-case distribution $\omega^q = \argmin_{\omega}\E_\omega[\pi(q)]$.
            \end{enumerate}
            \item Find the optimal $q$, i.e.\ $q_k = \argmax_{q \in \m{Q}_k} \E_{\omega^q}[\pi(q)]$. 
            \item Store outer objective $t_k = \max_{q \in \m{Q}_k} \E_{\omega^q}[\pi(q)]$.
        \end{enumerate}
        \item Solve inner problem for $q$ being fixed at $q_k$.
        \begin{enumerate}
            \item Construct set of extreme parameters/distributions:
            $$\Omega_{\text{ext}} = \l\{(\mu, \sigma) \in \Omega: \mu = \mu_{\min}
            \lor \sigma = \sigma_{\max}\r\}.$$
            \item Compute expected profit $P^{\omega} = \E_\omega[\pi(q_k)]$ for
            each $\omega \in \Omega_{\text{ext}}$.
            \item Find worst-case distribution $\omega_k = \min_{\omega \in
            \Omega_{k-1}} P^{\omega}$. 
        \end{enumerate}
        \item If $\omega_k \in \Omega_{k-1}$ or $t_k - P^{\omega_k} \le
        \frac{\varepsilon}{2}$ return $q_k, \omega_k$ and end algorithm.
        \item Otherwise set $\Omega_k = \Omega_{k-1} \cup \{\omega_k\}$, set $k
        = k + 1$ and go to (a).
    \end{enumerate}
    \item Return $q_k, \omega_k$.
\end{enumerate}
Note that, in step 4., $t_k \ge P^{\omega_k}$ as $\omega_k$ is the
worst-case distribution for $q_k$, meaning it has the expected lowest profit over all distributions.

\subsubsection{Testing CS}

To test the CS algorithm, we carry out some initial experiments (\textit{these
are initial right now, they might be extended further for the paper}). We
construct a set of inputs combinatorially using the following ranges:
\begin{itemize}
    \item $p \in \{1,\dots,10\}$,
    \item $w \in \{1, \dots, 9\}$ with $w < p$,
    \item $\mu_{\max} \in \{5,\dots,15\}$,
    \item $\sigma_{\max} \in \{5, \dots, 15\}$,
    \item $k_{\max} = 10$,
    \item $\varepsilon = 0.01$,
\end{itemize}
where $\mu_{\max}$ and $\sigma_{\max}$ are used to create the ambiguity set
$\Omega$ via equation~\eqref{eq:Omega_test}.
The last two are the same in all cases as CS typically finishes after finding a
duplicate, not because of $k$ or the optimality gap. Note that we do not allow
$w \ge p$ as if we did then there would be no profit to be made. The above list
creates a set of 5455 problems.  


==> A_poisson_old.tex <==
\section{DRO Model with Poisson Demands}

If the demands are independent Poisson random variables, i.e.\ $X_t \sim \text{Pois}(\lambda^0_t)$ for unknown $\bm{\lambda}^0$. Then we have:
\begin{equation}
    f_{X_t}(x_t) = \P(X_t = x_t) = \frac{(\lambda^0_t)^{x_t}\exp{(-\lambda^0_t)}}{(x_t)!} \quad (x_t \ge 0).
\end{equation}
We also have that $\sum_{k=1}^t X_k \sim \text{Pois}\l(\sum_{k=1}^t \lambda_k\r)$ for $t=1,\dots,T$. 

\subsection{Objective Function}

In order to evaluate the objective function, we need to evaluate $\E_{\bm{\lambda}}[I^+_t]$ and $\E_{\bm{\lambda}}[I^-_t]$. Recall that:
\begin{align}
    \E_{\bm{\lambda}}[I^+_t] &= \E_{\bm{\lambda}}[\max\{I_t, 0\}] \\
    \E_{\bm{\lambda}}[I^-_t] &= \E_{\bm{\lambda}}[\max\{-I_t, 0\}] 
\end{align}
where $I_t =  \sum_{k=1}^t(q_t - X_t)$, $\P(I_t \ge 0) = \P\l(\sum_{k=1}^t X_k \le \sum_{k=1}^t q_k\r)$ and $\E_{\bm{\lambda}}[I_t|I_t \ge 0] = \sum_{k=1}^t q_k - \E_{\bm{\lambda}}[\sum_{k=1}^t X_k| \sum_{k=1}^t X_k \le \sum_{k=1}^t q_k]$. To simplify notation, let us define $Q_t = \sum_{k=1}^t q_k$ and $\Lambda_t = \sum_{k=1}^t \lambda_k$. Now we have:
\begin{align}
    \P\l(I_t \ge 0\r) &= \P\l(\sum_{k=1}^t X_k \le Q_t\r) \\
    &= \tilde{F}_t\l(Q_t\r) \\
    &= \sum_{x=0}^{Q_t} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!}
\end{align}
and similarly we have:
\begin{align}
    \P\l(-I_t \ge 0\r) &= \P\l(I_t \le 0\r)\\
    &= \P\l(Q_t \le \sum_{k=1}^t X_k\r) \\
    &= 1 - \tilde{F}_t(Q_t - 1)\\
    &= 1 - \sum_{x=0}^{Q_t - 1} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!},
\end{align}
where $\tilde{f}_t$ and $\tilde{F}_t$ are the PMF and CDF of $\sum_{k=1}^t X_t$. Now, we can calculate the expected values as follows. 
\begin{align}
    \E_{\bm{\lambda}}[\max\{I_t, 0\}] &= \E_{\bm{\lambda}}\l[\max\l\{Q_t - \sum_{k=1}^t X_k, 0\r\}\r] \\
    &= \sum_{x = 0}^{\infty} \max\{Q_t - x, 0\} \tilde{f}_{t}(x) \\
    &= \sum_{x=0}^{Q_t} (Q_t - x) \tilde{f}_t(x)\\
    &= Q_t\tilde{F}_t(Q_t) - \sum_{x=0}^{Q_t} x \frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x)!} \\
    &= Q_t\tilde{F}_t(Q_t) - \sum_{x=1}^{Q_t}  \frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x-1)!} \\
    &= Q_t \tilde{F}_t(Q_t) - \Lambda_t\sum_{x=1}^{Q_t}  \frac{(\Lambda_t)^{x-1}\exp{(-\Lambda_t)}}{(x-1)!} \\
    &= Q_t \tilde{F}_t(Q_t) - \Lambda_t\tilde{F}_t(Q_t-1).
\end{align}
Similarly:
\begin{align}
    \E_{\bm{\lambda}}[\max\{-I_t, 0\}] &= \sum_{x = 0}^{\infty} \max\{x - Q_t, 0\} \tilde{f}_{t}(x) \\
    &= \sum_{x=Q_t + 1}^{\infty}(x-Q_t)\tilde{f}_t(x) \\
    &= -Q_t(1-\tilde{F}_t(Q_t)) + \sum_{x=Q_t+1}^{\infty} x\frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x)!}\\
    &= -Q_t(1-\tilde{F}_t(Q_t)) + \Lambda_t - \sum_{x=0}^{Q_t} x\frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x)!}\\
    &= -Q_t(1-\tilde{F}_t(Q_t)) + \Lambda_t - \sum_{x=1}^{Q_t} \frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x-1)!}\\
    &= -Q_t(1-\tilde{F}_t(Q_t)) +  \Lambda_t(1-\tilde{F}_t(Q_t-1)). 
\end{align}
This gives the following objective function (with $a_t = b +
p\mathds{1}\{t=T\} + h$):
\begin{align}
    C_{\bm{\lambda}}(\bm{q}) &= p\E_{\bm{\lambda}}[I^-_T] +  \sum_{t=1}^T(h \E_{\bm{\lambda}}[I^+_t] +  b\E_{\bm{\lambda}}[I^-_t] + w_t q_t - p \E_{\bm{\lambda}}[X_t]) \\
    &= \sum_{t=1}^T(h \E_{\bm{\lambda}}[I^+_t] +  (b + p\mathds{1}\{t=T\})\E_{\bm{\lambda}}[I^-_t] + w_t q_t - p \E_{\bm{\lambda}}[X_t]) \\
    &= \sum_{t=1}^T\l(h (Q_t \tilde{F}_t(Q_t) - \Lambda_t\tilde{F}_t(Q_t-1)) +  (b + p\mathds{1}\{t=T\})(-Q_t(1-\tilde{F}_t(Q_t)) \r.\nonumber\\ &\l. \quad +\Lambda_t(1-\tilde{F}_t(Q_t-1))) + w_t q_t - p \lambda_t\r) \\
    &= \sum_{t=1}^T\l(a_t Q_t \tilde{F}_t(Q_t) - \Lambda_t a_t \tilde{F}_t(Q_t-1) + (b+p\mathds{1}\{t=T\})(\Lambda_t - Q_t) + w_t q_t - p \lambda_t\r).
\end{align}


\subsection{Derivatives of Objective Function}

In order to select the worst-case $\bm{\lambda}$, we differentiate the objective function. We have that:
\begin{align}
    \pderiv{\tilde{F}_t(Q_t)}{\lambda_k} &=  \pderiv{}{\lambda_k}\l(\sum_{x=0}^{Q_t} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!}\r)\\
    &= \sum_{x=0}^{Q_t} \frac{-\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x + \exp\l(-\Lambda_t\r)x\l(\Lambda_t\r)^{x-1}}{x!}\\
    &= \sum_{x=1}^{Q_t}\frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^{x-1}}{(x-1)!} - \sum_{x=0}^{Q_t} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!} \\
    &= \sum_{x=0}^{Q_t - 1}\frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^{x}}{x!} - \sum_{x=0}^{Q_t} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!} \\
    &= - \frac{\exp(-\Lambda_t)(\Lambda_t)^{Q_t}}{Q_t!}\\
    &= -\tilde{f}_t(Q_t)
\end{align}
for $k \le t$. Similarly,
\begin{equation}
    \pderiv{\tilde{F}_t(Q_t - 1)}{\lambda_k} =  -\tilde{f}_t(Q_t-1) \quad (k \le t).
\end{equation}
Hence, we have:
% \begin{align}
%     \pderiv{C_{\bm{\lambda}}(\bm{q})}{\lambda_k} &= \sum_{t=k}^T\l(
%         -Q_ta_t\tilde{f}_t(Q_t) - a_t\tilde{F}_t(Q_t-1) + \Lambda_t a_t \tilde{f}_t(Q_t - 1) + b+p\mathds{1}\{t=T\}
%     -p\r) \\
%     &= \sum_{t=k}^T\l(b+p\mathds{1}\{t=T\} - a_t \tilde{F}_t(Q_t-1) - p\r)
% \end{align}
\begin{align}
    \pderiv{C_{\bm{\lambda}}(\bm{q})}{\lambda_k} &= \sum_{t=k}^T\l(
        - a_t Q_t \tilde{f}_t(Q_t) + \Lambda_t a_t \tilde{f}_t(Q_t - 1) - a_t \tilde{F}_t(Q_t - 1) + (a_t - h) - p 
    -p\r) \\
    &= \sum_{t=k}^T\l(- a_t \tilde{F}_t(Q_t - 1) + (a_t - h) - p\r) \label{eq:cancel_poisson}
\end{align}
where~\eqref{eq:cancel_poisson} is true because:
\begin{align}
    Q_t \tilde{f}_t(Q_t) &= Q_t \frac{\exp(-\Lambda_t) (\Lambda_t)^{Q_t}}{Q_t!}\\
    &= \frac{\exp(-\Lambda_t) (\Lambda_t)^{Q_t}}{(Q_t - 1)!}\\
    &= \Lambda_t \tilde{f}_t(Q_t-1).
\end{align}
This does not immediately suggest monotonicity. However, we have:
\begin{align}
    \frac{\partial^2 C_{\bm{\lambda}}(\bm{q})}{\partial \lambda^2_k} &= \sum_{t=k}^T a_t \tilde{f}_t(Q_t - 1)  \\
    &\ge 0 \fa k = 1,\dots,T.
\end{align}
Therefore, the objective function is convex in $\lambda_k$ for each $k$. Hence, the worst-case $\lambda_k$ will either be the smallest in the ambiguity set or the largest (when all other $\lambda_j$ are fixed). Therefore, we can construct a set of extreme distributions for a given $\Omega$ as follows:
\begin{equation}\label{eq:poisson_extreme}
    \Omega^{\text{ext}} = \l\{\bm{\lambda} \in \Omega \bigg| \exists t \in \{1,\dots,T\}: \lambda_t \in \l\{ \min_{\bm{\nu} \in \Omega} \nu_t, \max_{\bm{\nu} \in \Omega} \nu_t\r\}\r\}.
\end{equation}
The cutting surface algorithm is therefore the same as the one in Section~\ref{sec:normal_CS}, but using~\eqref{eq:poisson_extreme} as the set of extreme distributions.

\subsection{DRO Model and Piecewise Linear Approximation}

The DRO model for Poisson demands is given by:
\begin{align}
    \min_{\bm{q}}&\max_{\bm{\lambda} \in \Omega} C_{\bm{\lambda}}(\bm{q}) = \sum_{t=1}^T\l(a_t Q_t \tilde{F}_t(Q_t) - \Lambda_t a_t \tilde{F}_t(Q_t-1) + (a_t - h)(\Lambda_t - Q_t) + w_t q_t - p \lambda_t\r)\label{eq:poisson_obj}\\
    \text{s.t. } & \sum_{t=1}^T w_t q_t \le W,\\
    & q_t \in \mathbb{N}^0  \fa t \in \{1,\dots,T\}.\label{eq:poisson_last}
\end{align}
Due to the fact that the decision variable $Q_t$ appears in the upper limit of the sum defining $\tilde{F}_t(Q_t)$:
\begin{equation}
    \tilde{F}_t(Q_t) = \sum_{x=1}^{Q_t} \tilde{f}_t(x),
\end{equation}
this formulation cannot be expressed as an LP. An alternative would be to use the original form of the objective function, i.e.\ 
\begin{equation}
    C_{\bm{\lambda}}(\bm{q}) = p\E_{\bm{\lambda}}[I^-_T] + 
    \sum_{t=1}^T \l(h\E_{\bm{\lambda}}[I^+_t] + b\E_{\bm{\lambda}}[I^-_t] + w_t q_t- p \E_{\bm{\lambda}}[X_t]\r),
\end{equation}
and express expected values explicitly in the form $\E_{\bm{\lambda}}[I^-_t] = \sum_{x=0}^\infty \max\{x - Q_t\}\tilde{f}_t(x)$. However, this is an infinite sum and cannot be simplified without invoking the CDF as we have done to obtain the objective in~\eqref{eq:poisson_obj}. Hence, we will again use piecewise linear approximations to solve our model. In particular, we use a reformulation of the form:
\begin{align}
    \min \ &\theta \\
    \text{s.t. } & \theta \ge \tilde{C}_{\bm{\lambda}}(\bm{q}) \fa \bm{\lambda} \in \Omega\\
    &\sum_{t=1}^T w_t q_t \le W \\
    & q_t \ge 0 \fa t=1,\dots,T.
\end{align}

\subsection{Maximum Likelihood Estimation and Confidence Sets}

Suppose that we draw $N$ samples $\bm{x}^n = (x^n_1,\dots,x^n_T)$ from $\bm{X}$. Then, the MLEs are given by:
\begin{equation}\label{eq:poisson_MLE}
    \hat{\lambda}_t = \frac{1}{N} \sum_{n=1}^N x^n_t \quad (t=1,\dots,T).
\end{equation}
We also have that, approximately, for large $N$:
\begin{equation}
    \hat{\lambda}_t \sim \m{N}\l(\lambda^0_t, \frac{\lambda^0_t}{N}\r),
\end{equation}
or equivalently:
\begin{equation}
    \hat{\lambda}_t \sim \m{N}\l(\lambda^0_t, \frac{\hat{\lambda}_t}{N}\r).
\end{equation}
Hence, we can create univariate confidence intervals for the $\lambda^0_t$ using:
\begin{align}
    \lambda^{CI}_t &= \l\{\lambda_t: \hat{\lambda}_T - z_{1-\frac{\alpha}{2}} \sqrt{\frac{\hat{\lambda}_t}{N}} \le \lambda_t \le \hat{\lambda}_T + z_{1-\frac{\alpha}{2}} \sqrt{\frac{\hat{\lambda}_t}{N}}\r\} \quad (t=1,\dots,T).
\end{align}
As before, we can discretise the confidence intervals using:
\begin{equation}
    \tilde{\lambda}^{CI}_t = \l\{\lambda^l_t + m \frac{\lambda^u_t - \lambda^l_t}{M-1}, m=0,\dots,M-1\r\}.
\end{equation}
This allows to create a discrete base ambiguity set of the form:
\begin{equation}
    \Omega = \{\bm{\lambda}: \lambda_t \in \tilde{\lambda}^{CI}_t \fa t =1,\dots,T\}.
\end{equation}
Now, by independence of the $T$ MLEs, we have the approximate result that:
\begin{equation}
    \sum_{t=1}^T \frac{N}{\hat{\lambda_t}}(\hat{\lambda}_t - \lambda^0_t)^2 \sim \chi^2_T.
\end{equation}
Hence, we can calculate a discretisation of an approximate $100(1-\alpha)\%$ confidence set for $\bm{\lambda}^0$ using:
\begin{equation}
    \Omega_{\alpha} = \l\{\bm{\lambda} \in \Omega: \sum_{t=1}^T \frac{N}{\hat{\lambda}_t}(\hat{\lambda}_t - \lambda^0_t)^2 \sim \chi^2_{T, 1-\alpha}\r\}.
\end{equation}


==> B_5_results_old.tex <==
\subsection{Experiments on Confidence-based Ambiguity Sets}\label{sec:normal_results}

In this section, we will compare CS with PLA on ambiguity sets constructed using~\eqref{eq:normal_conf}. We will also compare the solutions from PLA with those from assuming the MLE distribution is the true distribution. In Section~\ref{sec:normal_expdes}, we describe the experimental design used. Following this, in Section~\ref{sec:normal_CSvsPWL} we we will summarise our results and assess CS as a heuristic for solving the full DRO model. We call this approach FD, and it entails using the adapted Alfares algorithm to solve the model assuming that $\bm{\omega} = \hat{\bm{\omega}}$.

\subsubsection{Experimental Design}\label{sec:normal_expdes}

In this Section, we describe the parameter values used in our testing. We will use a baseline discrete ambiguity set of the form~\eqref{eq:normal_base}. From this we will extract a confidence set using~\eqref{eq:normal_conf}. Given $\Omega_{\alpha}$, we need to define the range of points $z_j$ for $j=1,\dots,J$ that act as $\alpha^i_t$ in the piecewise linear approximation. We can define a range of points for $\alpha^i_t$ as follows. We have that:
\begin{align}
    \alpha^i_t &= \frac{\sum_{k=1}^t(\mu^i_k - q_k)}{\sqrt{\sum_{k=1}^t (\sigma^i_t)^2}}\\
    &\le \frac{\sum_{k=1}^t\mu^i_k}{\sqrt{\sum_{k=1}^t (\sigma^i_t)^2}}\\
    &=: (\alpha^i_t)^{\max}
\end{align}
for each $i = 1,\dots,I$ with $I=|\Omega_\alpha|$ and $t=1,\dots,T$. This is due to the fact that $q_k \ge 0 \fa k$.  Furthermore, we have:
\begin{align}
    \alpha^i_t &= \frac{\sum_{k=1}^t(\mu^i_k - q_k)}{\sqrt{\sum_{k=1}^t (\sigma^i_t)^2}}\\
    &\ge \frac{\sum_{k=1}^t\l(\mu^i_k - \frac{W}{w_k}\r)}{\sqrt{\sum_{k=1}^t (\sigma^i_t)^2}}\\
    &=: (\alpha^i_t)^{\min}
\end{align}
for each $i = 1,\dots,I$ and $t=1,\dots,T$. This is due to the following two facts. Firstly, the maximum value $q_k$ can take is when all other orders are zero. Secondly, this means that the budget constraint becomes $w_k q_k \le W$ i.e.\ $q_k \le \frac{W}{w_k}$. Hence, we define the points for the PLA as follows.
\begin{equation}
    z^i_t \in \l\{(\alpha^i_t)^{\min} + j\epsilon: j=0,\dots,\l\lfloor \frac{(\alpha^i_t)^{\max} - (\alpha^i_t)^{\min}}{\epsilon}\r\rfloor\r\}
\end{equation}
The reason for having a different range for each $(i,t)$ pair is that if we were to use only one, this would be the largest range of all of the individual ranges. Having one for each pair allows us to reduce the number of points in total that are used to define the piecewise linear model.  

The process that we use to test our methods on each instance is as follows.
\begin{enumerate}
    \item Obtain samples $\bm{x}^n$ for $n=1,\dots,N$ from true distribution of $\bm{X}$.
    \item Calculate MLE for each parameter using~\eqref{eq:MLEs}.
    \item Construct $\Omega$ and use MLEs to construct $\Omega_{\alpha}$.
    \item Solve the DRO problem for the instance with CS and PLA using $\Omega_{\alpha}$, and solve the MPNVP model with FD assuming $\bm{\omega} = \hat{\bm{\omega}}$.
    \item For each returned solution, compute true worst-case parameters and costs using brute force over the set $\Omega_\alpha$ using the true cost function. 
    \item Use FD with $\bm{\omega} = \bm{\omega}^0$, to obtain optimal solution under true distribution.
    \item Calculate cost of FD's MLE solution under true cost function.
\end{enumerate}
The final two steps allow us to assess the performance of the method that assumes that the MLEs are the true parameters. We will assume the true distribution in order to take samples and compute the costs. The true parameters are chosen at random from a large set of possible values. These parameters are not used by the DRO algorithms and not known to us beforehand. The parameters used in our testing are as follows:
\begin{enumerate}
    \item $T \in \{2,3,4\}$,
    \item $\mu^0_t \in \{1,\dots,20\} \fa t$,
    \item $\sigma^0_t \in \{1,\dots,10\} \fa t$,
    \item $\varepsilon \in \{0.1, 0.25, 0.50\}$ - the gap for the piecewise linear approximation points $z^i_t$,
    \item $M \in \{3,5,10\}$ - the number of points used in the discretisation of univariate confidence intervals,
    \item $N\in \{10, 25, 50\}$ - the number of samples taken from true distribution,
    \item $p, b, h \in \{100,200\}$,
    \item $W = 4000$ when $T = 2,3$ and $W = 8000$ for $T = 4$.
    \item $w_t = 100(T - t + 1)$ for $t=1,\dots,T$.
\end{enumerate}
With regards to $\bm{\mu}^0$ and $\bm{\sigma}^0$, we randomly select 3 values of $\bm{\omega}^0$ from the set defined by points 2.\ and 3.\ in this list. This is done for two reasons. Firstly, selecting only 3 keeps the number of experiments manageable. Secondly, selecting the values randomly means that we are not biasing the results by selecting them favourably. Note that we only select means and standard deviations such that $3\sigma^0_t \le \mu^0_t \fa t$, to ensure that the demand distributions are unlikely to generate negative values. We also do not consider instances where $T > 2$ and $M=10$. This is because in these cases the base ambiguity sets are too large to be feasible. The reason why we use $W = 8000$ for $T=4$ is that the optimal solution if $W = 4000$ is always $(0,0,0,40)$. This is not interesting, and increasing the budget gives a wider variety of solutions.

\subsubsection{Removing Dominated Distributions}

The size of $\Omega_{\alpha}$ can be too large for the model to be solved by PLA in a reasonable time. Recall from Theorem~\ref{thm:normal_extreme} that the objective function is increasing in $\sigma_t$ for $t=1,\dots,T$. Now consider two parameter values $\bm{\omega}^1$ and $\bm{\omega}^2$ such that:
\begin{align}
    &(\mu^1)_t = (\mu^2)_t \fa t = 1,\dots,T, \\
    &\sigma^1 \neq \sigma^2 \\
    &(\sigma^1)_t \ge (\sigma^2)_t \fa t = 1,\dots,T. 
\end{align}
In other words, there is at least one $t$ such that $(\sigma^1)_t > (\sigma^2)_t$ and there is no $t$ such that $(\sigma^1)_t < (\sigma^2)_t$. Since, for a fixed $\mu$, the objective function is increasing in each $\sigma_t$, this means that $\bm{\omega}^2$ is \textit{dominated} by $\bm{\omega}^1$. Hence, $\bm{\omega}^2$ can never be a worse parameter than $\bm{\omega}^1$. Since this parameter can never be the worst-case, it can be removed from $\Omega_{\alpha}$ and the solution to the model will not change. In our experiments, in order to reduce the computational burden for PLA, we will remove all dominated distributions prior to solving. For each solution, we will find the worst-case cost over the entirety of $\Omega_{\alpha}$ after solving the models. This allows us to verify that this pre-computation step never removed the true  worst-case parameter.

\subsubsection{Performance of MLE Approaches}\label{sec:MLE_performance}

In this section, we assess the performance of the MLE approaches as a heuristic for solving the model under the true distribution. In particular, we study how close to optimality the solutions resulting from the MLE distributions are, and how well the MLE distribution's cost function approximates the true objective function. We ran the MLE approaches on the 756 instances generated by the inputs from Section~\ref{sec:normal_expdes}. We present boxplots summarising the performance of the MLE approach in Figure~\ref{fig:FD_performance}. Let $\hat{\bm{q}}$ be the solution obtained from applying FD assuming $\bm{\omega} = \bm{\hat{\omega}}$. We will summarise our results using boxplots, with outliers (points further than 1.5IQR above the 75th percentile or below the 25th percentile) removed. Figure~\ref{fig:FD_optgap} shows the absolute percentage optimality gap of $\hat{\bm{q}}$ when compared with the optimal $\bm{q}$ under $\bm{\omega}_0$. In other words, it shows:
$$100 \times \l\lvert\frac{\min_{\bm{q}} C_{\bm{\omega}_0}(\bm{q})
- C_{\bm{\omega}_0}(\hat{\bm{q}})}{\min_{\bm{q}} C_{\bm{\omega}_0}(\bm{q})}\r\rvert.$$
This plot shows that $\hat{\bm{q}}$ is quite close to optimality under $\bm{\omega}_0$. For the smallest samples, i.e.\ $N=10$, it typically was no further than 10\% from optimal. The optimality gap reduces as $N$ increases.  However, Figure~\ref{fig:FD_APE} shows that the MLE distribution can result in poor approximations of the cost of $\hat{\bm{q}}$. The value shown here is calculated as:
$$100 \times \l\lvert\frac{C_{\bm{\omega}_0}(\hat{\bm{q}})
- C_{\hat{\bm{\omega}}}(\hat{\bm{q}})}{C_{\bm{\omega}_0}(\hat{\bm{q}})}\r\rvert.$$
The plot shows that for $N=10$, the APE of the MLE estimate of $C_{\bm{\omega}_0}(\hat{\bm{q}})$ can often reach almost 40\%. The accuracy of the estimate increases with $N$, but even for $N=50$ we see errors of over 15\%.

\vspace{-1em}
\begin{figure}[htbp!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Normal/MLE_FD_opt_gap.png}
        \caption{Percentage optimality gap of $\bm{\hat{q}}$ as a solution of model under $\bm{\omega}^0$}
        \label{fig:FD_optgap}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Normal/MLE_FDvsTrue_APE.png}
        \caption{Absolute percentage error of $C_{\hat{\bm{\omega}}}(\hat{\bm{q}})$ as an estimator of $C_{\bm{\omega}_0}(\hat{\bm{q}})$}
        \label{fig:FD_APE}
    \end{subfigure}
    \caption{Boxplots summarising performance of FD in comparison with true optimal solution}
    \label{fig:FD_performance}
\end{figure}
In addition, these errors can be even more extreme than shown here, due to outliers being removed from the plot. In some instances, the APE was as high as 15,600\%. This occurred in 2-period instances with $N=25$, where the true distribution was given by $\bm{\omega}_0 = ((9, 16) , (3, 4))$. The MLE obtained was $\hat{\bm{\omega}} = ((8.823, 16.346), (1.922, 3.708))$. The MLE distribution led to a solution $\hat{\bm{q}} = (7.888, 17.281)$ with an estimated expected cost of $-386.06$. The cost of this decision under the true distribution was $-2.46$, indicating a much worst solution than was suggested. 
In addition to this, we found that in 21 instances, the MLE solution gave an order quantity that was predicted to make a profit but ultimately resulted in a loss. The most extreme example of this happened again when $\bm{\omega}_0 = ((9, 16) , (3, 4))$. In this instance, $N=10$ samples were used and the MLE obtained was $\hat{\bm{\omega}} = ((9.172, 17.192), (2.421, 3.001))$. The order made by FD was $\hat{\bm{q}} = (8.123, 18.241)$, which had an expected cost of $-479.12$. The cost of this order under the true distribution was $52.42$, and the optimal cost under this distribution was $-5.42$. This shows that using the MLE solution would have resulted in a loss where a profit was possible. Interestingly, this happened for all values of $N$ and was not restricted to $N=10$. In general, we found that the MLE approach was likely to underestimate the cost of its chosen $\bm{q}$. This was the case in 62\% of instances. We found the opposite result, that is the MLE distribution predicting a cost when in fact a profit would be obtained, in 3 instances. This is perhaps preferable to the case where a profit is wrongly predicted. However, in reality it would cause the newsvendor not to take this action or perhaps spend more money on storage or staffing, unnecessarily. 

We can also confirm that this is not simply due to the performance of FD as a heuristic for the MPNVP model. In order to assess this, we also used PLA with an ambiguity set given by $\Omega = \{\hat{\bm{\omega}}\}$ to solve the problem. We present the percentage difference between FD's objective value under the MLE and PLA's objective value under the MLE, in Figure~\ref{fig:normal_FDvsPLA}. This figure shows that the two algorithms' solutions were typically within -1.5 and 1\% of one another. It also shows that FD can sometimes give better solutions than PLA (positive values indicate this). We can also confirm that the same results that we found from using FD also hold when PLA is used. Namely, the algorithm predicted a profit when there would in fact be a cost in 16 instances and it underestimated the cost of its decision in 59\% of instances. Interestingly, we find that PLA's solutions are closer in objective value to the optimum under $\bm{\omega}_0$ than FD's, but its cost predictions are worse. 

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{images_tables/Final Normal/MLE_PWLvsFD.png}
    %\caption{Percentage difference between the costs of FD and PLA's solutions under $\hat{\bm{\omega}}$}
    \caption{}
    \label{fig:normal_FDvsPLA}
\end{wrapfigure}

From the results shown here, we can make three key conclusions. Firstly, using the MLE distribution will typically lead to solutions that are reasonably close to optimal under the true distribution. Secondly, we can conclude that the MLE distribution can lead to poor estimates of associated costs associated with a given $\bm{q}$. In particular, solving using the MLEs can lead to the suggestion that the resulting decision will lead to a positive profit when it will actually lead to a positive cost. Finally, we can conclude that using the MLE distribution is likely to lead to an underestimation of the cost associated with the selected decision.

It is clear that using DRO would avoid the wrongful prediction of positive profits. Since the DRO objective is the worst-case cost, the newsvendor would be made aware of the fact that a decision could lead to a loss. This would not happen if using the MLE approach. For the aforementioned instance, where $\hat{\bm{q}}$ had a predicted cost of $-479.12$ and an actual cost of 52.4, the cost that would be associated with this decision under the DRO model was 374.855. This means that the decision maker would be completely aware that this decision could lead to a loss. Of course, the DRO objectives will also be higher than those under the true distribution. However, the newsvendor would be aware that this was a worst-case cost, and hence they would not expect this to be the cost obtained. In fact, due to the MLE approach not being able to suggest that these decisions could result in a loss, it is very reasonable to optimise a more pessimistic objective function. 

\subsubsection{Performance of DRO Algorithms}\label{sec:normal_CSvsPWL}

Each algorithm was given a maximum time of four hours in which to build and solve its model. We now present the average times taken over all instances. Of the {756} instances we ran, PWL timed out in {108} instances. CS did not time out in any instance. The times taken are summarised in Figure~\ref{fig:normal_timestaken}. Note that the values shown are the time taken before the algorithm either returned a solution or timed out. Figure~\ref{fig:normal_timestaken} shows the magnitude of improvements in solution times from using CS over PLA. PLA took 16 minutes and 29 seconds on average, whereas CS took just 3 seconds. The 25\% and 75\% quantiles for PLA's time taken are 4.3 seconds and 6 minutes and 9 seconds. For CS, these values are 0.72 seconds and 3.3 seconds. In addition, PLA took up to a maximum of 2 hours and 43 minutes before it was either cancelled or finished running, whereas CS always finished running in less than 25 seconds. PLA's maximum time is shorter than the time limit of 4 hours because pre-computation is included in its total time, but here we only present runtimes.

\begin{figure}[htbp!]
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=1.01\textwidth]{images_tables/Final Normal/PLA_tt.png}
        \caption{Time taken by PLA}
        \label{fig:normal_PLA_tt}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Normal/CS_tt.png}
        \caption{Times taken by CS}
        \label{fig:normal_CS_FD_tt}
    \end{subfigure}
    \caption{Boxplots of times taken by PLA and CS}
    \label{fig:normal_timestaken}
\end{figure}

We can now look at the factors affecting these times. From our analysis, the main factor affecting PLA's times is {$M$}. For large $M$, the base ambiguity set $\Omega$ becomes very large. Therefore, even constructing $\Omega_\alpha$ takes quite some time. To highlight the effect of $M$ on PLA and CS, we present boxplots grouped by $M$ in Figures~\ref{fig:normal_timestaken_by_M_PLA} and~\ref{fig:normal_timestaken_by_M_CS}. Since $M=10$ was only run for $T=2$, we separate these plots into two. Figure~\ref{fig:normal_PLA_tt_by_M} shows that PLA begins to solve slowly for $M=5$ when $T > 2$, and in fact this is where all of PLA's timeouts occurred. Figure~\ref{fig:normal_PLA_tt_by_M2} shows that PLA takes negligible time until $M=10$ when $T=2$, where it starts to take up to two minutes. The effect of $M$ on CS is not so drastic. As shown in Figure~\ref{fig:normal_CS_tt_by_M_2}, for $T=2$, CS's times are quite consistent over all values of $M$. For $T>2$, Figure~\ref{fig:normal_CS_tt_by_M} shows that CS does take longer for $M = 5$ than for $M=3$, but this difference is much less noticeable than for PLA. 

\begin{figure}[htb!]
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.97\textwidth]{images_tables/Final Normal/PLA_times_by_M.png}
        \caption{Times for $T>2$}
        \label{fig:normal_PLA_tt_by_M}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.97\textwidth]{images_tables/Final Normal/PLA_times_by_M_2.png}
        \caption{Times for $T=2$}
        \label{fig:normal_PLA_tt_by_M2}
    \end{subfigure}
    \caption{Boxplots of times taken by PLA, grouped by $M$}
    \label{fig:normal_timestaken_by_M_PLA}
\end{figure}

\begin{figure}[htb!]
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.97\textwidth]{images_tables/Final Normal/CS_times_by_M.png}
        \caption{Times for $T>2$}
        \label{fig:normal_CS_tt_by_M}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.97\textwidth]{images_tables/Final Normal/CS_times_by_M_2.png}
        \caption{Times for $T=2$}
        \label{fig:normal_CS_tt_by_M_2}
    \end{subfigure}
    \caption{Boxplots of times taken by CS, grouped by $M$}
    \label{fig:normal_timestaken_by_M_CS}
\end{figure}

As might be expected, the solution times for PLA and CS are also affected by $T$. We present the average times taken by $T$ in Figure~\ref{fig:normal_timestaken_by_T}. This figure shows both algorithms take a noticeably larger time for $T=4$. However, CS scales much better with $T$ than PLA. Our results suggest CS would be easily applicable to larger problems, while PLA is likely to take multiple hours for anything larger than $T=4$.

\begin{figure}[htbp!]
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.97\textwidth]{images_tables/Final Normal/PLA_times_by_T.png}
        \caption{Time taken by PLA, grouped by $T$}
        \label{fig:normal_PLA_tt_by_T}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Normal/CS_times_by_T.png}
        \caption{Times taken by CS, grouped by $T$}
        \label{fig:normal_CS_tt_by_T}
    \end{subfigure}
    \caption{Boxplots of times taken by PLA and CS, grouped by $T$}
    \label{fig:normal_timestaken_by_T}
\end{figure}

We now assess the performance of CS as a heuristic for solving the full DRO model. This is done via comparing its objective values and returned $\bm{\omega}$ values with those from PLA. We first present the number of times that CS and PLA obtained the worst-case parameters for their chosen $\bm{q}$. We present these values for PLA as well as CS since both algorithms use a reduced ambiguity set. Hence, studying these results allows us to confirm that the reduced set contains the true worst-case for each solution. We present the optimality counts in Table~\ref{tab:normal_worstcase}. Note that these counts are given only over the instances where both algorithms finished running. 

CS chose the worst-case parameters for its selected $\bm{q}$ in 84\% of instances. Its performance is consistent over all values of $T$.  PLA chose the worst-case parameters in every instance. This is expected, since despite the fact that the approximate objective can lead to the wrong worst-case parameter, we use the true objective function to generate the cost of PLA's solution after it finishes running. The main purpose of this is to confirm that our removal of dominated distributions did not remove the worst-case parameter in any instance. CS failed to select the worst-case parameters in 121 instances.

 \begin{table}[htbp!]
    \centering
    \input{images_tables/Final Normal/worst_case_by_T}
    \caption{Number of instances in which algorithms selected true worst case parameters.}   
    \label{tab:normal_worstcase}
\end{table}

Table~\ref{tab:normal_worstcase} only shows the number of times CS chose the worst-case parameters. In order to gain a better understanding of its performance, we can study two quantities:
\begin{enumerate}
    \item Percentage $\bm{\omega}$-gap: The percentage difference between the worst-case cost for $\bm{q}^{\text{CS}}$ and the cost obtained under the $\bm{\omega}$ returned by CS. Defined as:
    $$100\times \frac{\max_{\bm{\omega} \in \Omega_\alpha} C_{\bm{\omega}}(\bm{q}^{\text{CS}}) - C_{\bm{\omega}^{\text{CS}}}(\bm{q}^{\text{CS}})}{\max_{\bm{\omega} \in \Omega_\alpha}C_{\bm{\omega}}(\bm{q}^{\text{CS}})}.$$
    \item Percentage $\bm{q}$-gap: The percentage difference between the worst-case cost attained by $\bm{q}^{\text{CS}}$ and that attained by $\bm{q}^{\text{PLA}}$. Defined as:
    $$100 \times \frac{\max_{\bm{\omega} \in \Omega_\alpha} C_{\bm{\omega}}(\bm{q}^{\text{PLA}}) - \max_{\bm{\omega} \in \Omega_\alpha} C_{\bm{\omega}}(\bm{q}^{\text{CS}})}{\max_{\bm{\omega} \in \Omega_\alpha} C_{\bm{\omega}}(\bm{q}^{\text{PLA}})}.$$
\end{enumerate}
Note that positive values (lower expected cost) for the $\bm{\omega}$-gap implies that CS gave a suboptimal $\bm{\omega}$. Negative values (higher worst-case expected cost) for the $\bm{q}$-gap imply that CS gave a suboptimal $\bm{q}$. Figure~\ref{fig:normal_gaps} summarises the percentage gaps using boxplots. The first thing to notice is that the $\bm{\omega}$-gaps were so commonly zero that everything non-zero was considered as an outlier. On average, the percentage $\bm{\omega}$-gap was 0.099\%. This shows that CS's chosen parameters were very close in cost to the worst-case for its chosen $\bm{q}$. The 25\% and 75\% quantiles of the $\bm{\omega}$-gap were both 0. We see from Figure~\ref{fig:normal_q_gap} that CS's chosen $\bm{q}$ had a worst-case cost that was very close to PLA's, in general. The percentage optimality gaps typically do not exceed 0.003\%. The overall average percentage $\bm{q}$-gap was $-0.29\%$, suggesting that CS is very near optimal with respect to $\bm{q}$ on average. The 25\% and 75\% quantiles for this gap were $-1.3\times 10^{-5}$ and 0. We also see that the $\bm{q}$-gap was slightly more variable for $T=2$. This is not due to $T=2$, however, but due to the instances where $M=10$ that were only run for $T=2$. This is indicated by Figure~\ref{fig:normal_q_gap_by_M}. This does not, however, affect CS's $\bm{\omega}$-gap.
\begin{figure}[htbp!]
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Normal/percent_omega_gap_by_T.png}
        \caption{}
        \label{fig:normal_omega_gap}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Normal/percent_q_gap_by_T.png}
        \caption{}
        \label{fig:normal_q_gap}
        %\hspace*{-5em}
    \end{subfigure}
    \newline
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Normal/percent_omega_gap_by_M.png}
        \caption{}
        \label{fig:normal_omega_gap_by_M}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Normal/percent_q_gap_by_M.png}
        \caption{}
        \label{fig:normal_q_gap_by_M}
    \end{subfigure}
    \caption{Summary of percentage gaps}
    \label{fig:normal_gaps}
\end{figure}

CS even performed better than PLA in 107 instances. Since CS can be viewed as a heuristic for solving the full model that PLA solves, this may be unexpected. This occurs due to one of two reasons. Firstly, the approximate objective used by PLA can see CS's solution as the same or worse than its own, when in reality it is better.  To see this, we consider a toy example. In one two-day instance when CS had a better solution than PLA, PLA returned a solution $( 16.32, 19.2)$. This solution had a worst-case cost of $135.62$ according to the approximate objective function. This was also the true worst-case cost of PWL's solution. Running CS on the same instance, we get a solution of $(16.52, 18.99)$. This has a true worst-case cost of $129.55$, i.e.\ better than PLA's solution. However, evaluating CS's solution using PLA's objective function, the approximation leads to the incorrect worst-case parameter and and approximate worst-case cost of $139.74$. Hence, PLA saw this solution as suboptimal. When this solution was generated by CS, however, the true cost function was used to decide whether or not it was optimal. This meant that CS's stopping criterion was triggered, when it would not have been if the piecewise linear objective was used. Secondly, Gurobi's presolve can affect solution quality, either by worsening PLA's solution and hence leading to CS giving a better solution than PLA, or by either worsening or improving CS's solution. We found examples of all three of these situations in our results. When presolve was the cause of CS performing better than PLA, the differences in objective values were very small. In addition, this phenomenon still occurs when presolve is turned off.  Hence, its main cause is likely the approximation of the objective function. We found that the number of instances where CS performed better than PLA was increasing with $\varepsilon$, meaning that the worse the piecewise linear approximation is, the more likely CS is to be better than PLA. 

% This is due to the approximation used by the two algorithms. PLA optimises the the piecewise linear approximation to the newsvendor objective directly. While CS also does this inside each master problem, it does not use the approximate objective in its stopping criteria. This may lead to CS having better solutions to the actual model than PLA. To see this, we consider a toy example. In one two-day instance when CS had a better solution than PLA, PLA returned a solution $( 16.32, 19.2)$. This solution had a worst-case cost of $135.62$ according to the approximate objective function. This was also the true worst-case cost of PWL's solution. Running CS on the same instance, we get a solution of $(16.52, 18.99)$. This has a true worst-case cost of $129.55$, i.e.\ better than PLA's solution. However, evaluating CS's solution using PLA's objective function, we get an approximate worst-case cost of $139.74$. Hence, this solution has a higher worst-case cost than PLA's solution under the approximate objective. Hence, CS can yield better solutions than PLA because the piecewise linear objective function sees CS's solutions as worse.

% The cause for PLA's suboptimality was the approximation used in most instances. However, some of Gurobi's methods can also lead to small differences in solution quality. For example, we run the presolve method on our full models. This can cause either better or worse solutions. In another two-day example, PLA's solution had a true (approximate) worst-case expected cost of $-563.21$ ($-563.21$) and CS's had a true (approximate) cost of $-563.65$ ($-563.17$). Hence, CS's solution is worse than PLA's under the approximate objective function. When run with presolve turned off, PLA's solution does not change. However, CS's solution changes, and the new solution has a true (approximate) objective value of $-563.21$ ($-563.21$). Hence, with presolve on, CS's solution is worse under the approximate objective function but better under the true objective function. Presolve can also worsen CS's solution. In another instance, PLA's solution had a true (approximate) worst-case expected cost of $2003.945$ ($2004.55$) with presolve both on and off. However, with presolve on CS's solution had a true (approximate) cost of $2003.995$ ($2004.64$), and with presolve off it had a true (approximate) cost of $2003.945$ ($2004.55$). Hence, CS's solutions were always worse than PLA's under the approximate objective function. However, CS's solution with presolve off was better than its solution without. 

From these results we can conclude 4 main points. Firstly, CS is much faster than PLA and scales much better. It never took more than 25 seconds to finish running, whereas PLA timed out in over 100 instances. Secondly, PLA performs better in selecting the worst-case parameters for a fixed $\bm{q}$. This is expected, as CS applies cardinality reduction to the ambiguity set. CS's returned parameters are very close to the worst-case in terms of cost, however. Thirdly, CS is very close to optimal with respect to its chosen $\bm{q}$. On average, it returns solutions that are only $0.29\%$ away from optimal. Finally, CS can perform better than PLA in some instances, due to the accuracy of the piecewise linear approximation and/or Gurobi's presolve procedure.

% \subsubsection{DRO vs MLE Distribution}\label{sec:normal_DROvsFD}

% In this section, we compare the solutions from our DRO model with those from assuming that $\bm{\omega} = \hat{\bm{\omega}}$ and solving the model with these parameters fixed. Figure~\ref{fig:normal_true_diffs} plots:
% \begin{equation}
%     100 \times \frac{C_{\bm{\omega}^0}(\bm{q}^{x}) - C_{\bm{\omega}^0}(\bm{q}^{\text{FD})}}{C_{\bm{\omega}^0}(\bm{q}^{\text{FD})}}
% \end{equation}
% for $x \in \{\text{PLA}, \text{CS}\}$. This allows us to compare how the DRO solutions compare with the MLE solution under the true distribution. Figure~\ref{fig:normal_true_diffs} suggests that the DRO solutions have costs that are typically between \red{0\% and 5\% higher than FD} under the true distribution. This may be expected, since DRO optimises the worst-case cost, and the worst-case distribution can be very different from the MLE distribution. However, there were \red{98 instances} in which either PLA or CS gave a better solution than FD under the true distribution. We now study these instances in order to learn when DRO solutions perform better than assuming the distribution is given by the MLEs. 
% \begin{figure}[htbp!]
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \includegraphics[width=0.95\textwidth]{images_tables/normal_conf_fast/PLAvsFD_by_T.png}
%         \caption{Percentage objective difference between PLA and FD}
%         \label{fig:normal_PLAvsFD}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \includegraphics[width=0.97\textwidth]{images_tables/normal_conf_fast/CSvsFD_by_T.png}
%         \caption{Percentage objective difference between CS and FD}
%         \label{fig:normal_CSvsFD}
%     \end{subfigure}
%     \caption{Summary of DRO vs FD objective values under true distribution}
%     \label{fig:normal_true_diffs}
% \end{figure}

==> B_6_results_old.tex <==
\subsection{Experimental Design and Results}\label{sec:poisson_results}

To test the cutting surface algorithm on Poisson demands, we run experiments on the same inputs as for the normal distribution. In every case, we take the value of $\bm{\lambda}^0$ to be equal to the value of $\bm{\mu}_0$ in the normal experiments. This allows to see the effect on our results if the only thing allowed to change is the distribution used. Note, however, that we now run the tests with $T > 2$ and $M = 10$, since the Poisson ambiguity sets are not as large. In addition, since each $q_t$ is now integer, we can simply use a $\varepsilon$ of 1 in all instances. Hence, we run our experiments for an additional 6 randomly selected values of $\bm{\lambda}^0$, in order to generate more results. As in the normal case, all boxplots have outliers (points further than 1.5IQR above the 75th percentile or below the 25th percentile) removed.


\subsubsection{Performance of MLE Solutions}

Firstly, as for the normal distribution, we assess the effect of solving the newsvendor problem using the MLE distribution. We present the APE of the MLE's cost estimate along with the optimality gap of the MLE solution in Figure~\ref{fig:FD_performance_poisson}. This figure indicates that the MLE approach is close to optimal for Poisson demands, with solutions typically not being further than 4\% from optimal. However, the cost estimates are still not accurate. For $N=10$, we can see some APEs above 25\%. Even for $N=50$, we see APEs of almost 15\%. In addition, this plot does not show outliers. There were 19 instances where the APE exceeded 100\%, and 2 where it exceeded 10000\%. In both of the most extreme instances, the true parameter was $\bm{\lambda}^0 = (10, 17)$ and both solutions were $(8, 17)$. In one instance we used $N=10$ and in the other we used $N=25$. In the instance with $N=10$, the MLE obtained was $\bm{\hat{\lambda}} = (10.8, 14.3)$. The solution produced by FD had an estimated cost of 168.97, and a true cost of 0.727, which corresponds to an APE of 23145\%. In the instance with $N=25$, the MLE was $\bm{\hat{\lambda}} = (10.24, 15.16)$. As a result of the improved MLE, the estimated cost was $75.03566$, which is closer to the true cost of 0.727. The APE for this instance was 10222\%. However, in both instances it was possible to make a profit under the true distribution. The optimal objective value under $\bm{\lambda}^0$ was $-75.93$, meaning that the MLE solution did not lead to a profit, when it was indeed possible.

\begin{figure}[htbp!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Poisson/MLE_FD_opt_gap.png}
        \caption{Percentage optimality gap of $\bm{\hat{q}}$ as a solution of model under $\bm{\lambda}^0$}
        \label{fig:FD_optgap_poisson}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Poisson/MLE_FDvsTrue_APE.png}
        \caption{Absolute percentage error of $C_{\hat{\bm{\lambda}}}(\hat{\bm{q}})$ as an estimator of $C_{\bm{\lambda}^0}(\hat{\bm{q}})$}
        \label{fig:FD_APE_poisson}
    \end{subfigure}
    \caption{Boxplots summarising performance of FD in comparison with true optimal solution}
    \label{fig:FD_performance_poisson}
\end{figure}

In addition, similarly to in the normal case, we find instances where the MLE predicts a profit for a decision that would actually attain a cost. This happened in 4 instances for the Poisson distribution, as opposed to 21 for the normal distribution. We summarise these 4 instances in Table~\ref{tab:FD_posneg}. This table shows the values of $\bm{\lambda}_0$ and $\hat{\bm{\lambda}}$ as well as the different costs associated with the MLE solution. This Table shows that, in every instance, the DRO cost was positive. This suggests that the DRO objective would always show the newsvendor that the solution could lead to a cost. In addition, in the first and last instances, the DRO cost is much closer to the truth than the MLE prediction. In one instance, DRO's cost was actually lower than the true cost. This can happen when $\bm{\lambda}^0 \notin \Omega_\alpha$. We also found that the MLE distribution predicted a cost when it would make a profit, although this only happened in two instances.

\begin{table}[htbp!]
    \centering
    \input{images_tables/Final Poisson/MLE_posneg}
    \caption{Summary of instances where FD predicted profit but actually made a cost}
    \label{tab:FD_posneg}
\end{table}

Similarly to the normal case, we can confirm that the poor accuracy is not due to FD being a heuristic for the MPNVP model.  In the Poisson case, the two algorithms are even closer to one another than in the normal case.  We found that FD returned the same solution as PLA in 921 of the 972 instances considered. In addition, the solutions from the two algorithms had the same objective values in the other 51 instances. Therefore, the two algorithms have exactly the same performance for Poisson demands. Hence, the issues presented here are likely only due to the effects of treating the MLE as the true parameter. 

% \begin{wrapfigure}{r}{0.55\textwidth}
%     \centering
%     \includegraphics[width=0.55\textwidth]{images_tables/Final Poisson/MLE_PWLvsFD.png}
%     %\caption{Percentage difference between the costs of FD and PLA's solutions under $\hat{\bm{\lambda}}$}
%     \caption{}
%     \label{fig:poisson_FDvsPLA}
% \end{wrapfigure}

In conclusion, the MLE approach performs better for Poisson demands than for normal ones, but it still has the same issues. In particular, it provides poor estimates of the cost associated with an order quantity. It is even capable of predicting a profit when a cost would be incurred, and vice versa. In addition, we confirmed that the DRO solution does not do this. In fact, in these instances the DRO cost is sometimes closer to reality than the MLE cost.


\subsubsection{Performance of DRO Algorithms}

We now present the results for the 972 instances where we solved the DRO model with Poisson demands. We will summarise the times taken by PLA and CS, along with CS's performance as a heuristic for the full model. Both algorithms were given a maximum time of 4 hours to build and solve the models. Firstly, we found that PLA timed out in 58 instances and CS did not time out in any instance. PLA took an average of 16 minutes and 36 seconds to either return a solution or time out, and its maximum time was 4 hours. CS took an average of 2 seconds, and its maximum time was 29 seconds. The times taken are shown in more detail in Figure~\ref{fig:poisson_timestaken}. These plots show the 25th and 75th percentiles of PLA to be 0.97 seconds and 52.85 seconds, respectively. For CS, these values are 0.28 and 1.31 seconds. In general, both algorithms are faster for Poisson demands. This is due to two reasons. Firstly, the fact that the gap used in the piecewise linear approximation, i.e.\ $\varepsilon$, was 1 in all cases. Secondly, due to the fact that there is only one parameter per day, the ambiguity sets are smaller here. The average size of the ambiguity set for these experiments was 1142.15, as opposed to 34223.02 for the normal experiments (before elimination of dominated parameters). 

\begin{figure}[htbp!]
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=1.01\textwidth]{images_tables/Final Poisson/PLA_tt.png}
        \caption{Time taken by PLA}
        \label{fig:poisson_PLA_tt}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Poisson/CS_tt.png}
        \caption{Times taken by CS}
        \label{fig:poisson_CS_FD_tt}
    \end{subfigure}
    \caption{Boxplots of times taken by PLA and CS}
    \label{fig:poisson_timestaken}
\end{figure}

The main variable affecting the solution times was, again, $M$. We present the times taken by $M$ in Figure~\ref{fig:poisson_timestaken_by_M}. We can see that the effect of $M$ is similar on both PLA and CS, although the increase in time taken is not so drastic for CS. The difference is most noticeable for $M=10$, and this is the value at which both algorithms start to solve more slowly. However, CS did not take more than 29 seconds in any instance. The times taken by $T$ reflect the results suggested by Figure~\ref{fig:poisson_timestaken_by_M}. This is because the reason why $M$ affects times so drastically is that it affects the size of the ambiguity set. This is also the reason why $T$ affects the times taken.
\begin{figure}[htbp!]
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.97\textwidth]{images_tables/Final Poisson/PLA_times_by_M.png}
        \caption{}
        \label{fig:poisson_PLA_tt_by_M}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.97\textwidth]{images_tables/Final Poisson/CS_times_by_M.png}
        \caption{}
        \label{fig:poisson_PLA_tt_by_M2}
    \end{subfigure}
    \caption{Boxplots of times taken, grouped by $M$}
    \label{fig:poisson_timestaken_by_M}
\end{figure}
% \begin{figure}[htbp!]
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \includegraphics[width=0.97\textwidth]{images_tables/Final Poisson/PLA_times_by_T.png}
%         \caption{}
%         \label{fig:poisson_PLA_tt_by_T}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.45\textwidth}
%         \centering
%         \includegraphics[width=0.97\textwidth]{images_tables/Final Poisson/CS_times_by_T.png}
%         \caption{}
%         \label{fig:poisson_PLA_tt_by_T2}
%     \end{subfigure}
%     \caption{Boxplots of times taken, grouped by $T$}
%     \label{fig:poisson_timestaken_by_T}
% \end{figure}

We now present the optimality of CS with respect to $\bm{\lambda}$ and $\bm{q}$. Firstly, we present the number of times each algorithm selected the worst-case parameter for its chosen $\bm{q}$ in Table~\ref{tab:poisson_worstcase}. This table shows that CS selected the worst-case $\bm{\lambda}$ for its $\bm{q}$ in every instance. As did PLA.

 \begin{table}[htbp!]
    \centering
    \input{images_tables/Final Poisson/worst_case_by_T}
    \caption{Number of instances in which algorithms selected true worst case parameters.}   
    \label{tab:poisson_worstcase}
\end{table}


The percentage $\bm{\lambda}$- and $\bm{q}$-gaps are defined as they were for the normal experiments in Section~\ref{sec:normal_CSvsPWL}, and we present summaries of these gaps in Figure~\ref{fig:poisson_gaps}. Firstly, Figure~\ref{fig:poisson_omega_gap} reflects the fact that CS always selected the worst-case parameter for its chosen $\bm{q}$. Secondly, Figure~\ref{fig:poisson_q_gap} shows that typically selected a $\bm{q}$ with a worst-case cost of less than $8\times 10^{-6}\%$ higher than PLA's. In fact, CS's $\bm{q}$ had the same worst-case expected cost as PLA's in 832 (91\%) of the 914 instances in which PLA did not time out. The overall average $\bm{q}$-gap was $-0.00012\%$,  and the minimum value of this gap was $-0.009\%$. Since CS chose the worst-case parameter in every instance, we might expect that it would be optimal in every instance. However, as discussed in Section~\ref{sec:normal_CSvsPWL}, Gurobi's presolve can affect the solutions. Furthermore, for MIP solvers, the constraint ordering is known to have a slight effect on solution quality, due to it leading to different starting points for MIP algorithms. This may be what causes the slight suboptimality of CS in 8\% of instances. 

\begin{figure}[htbp!]
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Poisson/percent_lambda_gap_by_T.png}
        \caption{}
        \label{fig:poisson_omega_gap}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{images_tables/Final Poisson/percent_q_gap_by_T.png}
        \caption{}
        \label{fig:poisson_q_gap}
        %\hspace*{-5em}
    \end{subfigure}
    \caption{Summary of percentage gaps}
    \label{fig:poisson_gaps}
\end{figure}

From the results shown here, we can conclude two main points. Firstly, CS again solves much faster than PLA. Secondly, it is very near optimal if not optimal, in general.  It is capable of selecting the worst-case parameter for its chosen $\bm{q}$ in every instance, and this $\bm{q}$ is likely to be optimal. For Poisson demands, there is no reason to use PLA over CS. 

==> C_truncated_normal.tex <==
\section{DRO Model with Zero-truncated Normal Demands}

Suppose instead that $X \sim TN(\mu, \sigma^2, 0, \infty)$ i.e.\ it is a normal distribution truncated below at 0. Let $Y \sim N(\mu, \sigma^2)$. Then we have:
\begin{align}
    X &= Y | Y > 0 \\
    F_X(x) &= \frac{F_Y(x) - F_Y(0)}{1-F_Y(0)} \\
    &= \frac{\Phi\l(\frac{x-\mu}{\sigma}\r) - \Phi(\alpha)}{1-\Phi(\alpha)}
\end{align}
where $\alpha = -\frac{\mu}{\sigma}$. 

\subsection{Objective Function and Derivatives}

With $\beta = \frac{q-\mu}{\sigma}$, we have:
\begin{align}
    \E_\omega(\min(q, X)) &= \E_\omega(X|X<q)\P(X \le q) + q\P(X > q) \\
    &= \l[\mu - \sigma\frac{\phi(\beta) - \phi(\alpha)}{\Phi(\beta) - \Phi(\alpha)}\r]\frac{\Phi(\beta) - \Phi(\alpha)}{1-\Phi(\alpha)} +  q\l(1- \frac{\Phi(\beta) - \Phi(\alpha)}{1-\Phi(\alpha)}\r)\\
    &= \frac{1}{1-\Phi(\alpha)}\l[\mu \Xi - \sigma\xi\r] + q - q\frac{\Xi}{1-\Phi(\alpha)}\\
    &= \frac{1}{1-\Phi(\alpha)}\l[(\mu-q)\Xi - \sigma \xi\r] + q,
\end{align}
where $\Xi = \Phi(\beta) - \Phi(\alpha)$ and $\xi = \phi(\beta) - \phi(\alpha)$. Therefore:
\begin{align}
    \E_\omega(\pi(q)) &= \E_\omega(p \min(X, q) - wq) \\
    &= \frac{p}{1-\Phi(\alpha)}\l[(\mu-q)\Xi - \sigma \xi\r] + q(p-w).
\end{align}
Taking derivatives using the chain rule, we find that:
\begin{align}
    \pderiv{\phi(\alpha)}{\mu} = -\frac{\mu}{\sigma^2} \phi(\alpha), \quad \quad
    &\pderiv{\phi(\alpha)}{\sigma} = \frac{\mu^2}{\sigma^3}\phi(\alpha) \\
    \pderiv{\phi(\beta)}{\mu} = \frac{q-\mu}{\sigma^2} \phi(\beta), \quad \quad  
    &\pderiv{\phi(\beta)}{\sigma} = \frac{(q-\mu)^2}{\sigma^3} \phi(\beta)\\
    \pderiv{\Phi(\alpha)}{\mu} = -\frac{1}{\sigma}\phi(\alpha), \quad \quad & \pderiv{\Phi(\alpha)}{\sigma} = \frac{\mu}{\sigma^2}\phi(\alpha) \\
    \pderiv{\Phi(\beta)}{\mu} = -\frac{1}{\sigma}\phi(\beta), \quad \quad & \pderiv{\Phi(\beta)}{\sigma} = \frac{\mu-q}{\sigma^2}\phi(\alpha).
\end{align}
Hence, we have:
\begin{align}
    \pderiv{\Xi}{\mu} &= -\frac{1}{\sigma}\phi(\beta) - \l(-\frac{1}{\sigma}\phi(\alpha)\r) = -\frac{1}{\sigma}\xi \\
    \pderiv{\Xi}{\sigma} &= \frac{\mu-q}{\sigma^2}\phi(\beta) - \frac{\mu}{\sigma^2} \phi(\alpha) = \frac{-\beta\phi(\beta) + \alpha\phi(\alpha) }{\sigma} \\
    \pderiv{\xi}{\mu} &= \frac{(q-\mu)}{\sigma^2}\phi(\beta) + \frac{\mu}{\sigma^2}\phi(\alpha) = \frac{\beta\phi(\beta) -\alpha\phi(\alpha)}{\sigma}\\
    \pderiv{\xi}{\sigma} &= \frac{(\mu-q)^2}{\sigma^3}\phi(\beta) - \frac{\mu^2}{\sigma^3}\phi(\alpha) = \frac{\beta^2\phi(\beta) - \alpha^2\phi(\alpha)}{\sigma}.
\end{align}
This means that:
\begin{align}
    \pderiv{}{\mu}\l((\mu - q)\Xi - \sigma\xi) &= (\mu - q)\pderiv{\Xi}{\mu} +\Xi - \sigma \pderiv{\xi}{\mu} \\
    &= -\frac{\mu - q}{\sigma}\xi + \Xi  - (\beta\phi(\beta) -\alpha\phi(\alpha))  \\
    &=  \beta \phi(\beta) - \beta \phi(\alpha) + \Xi -  \beta\phi(\beta) + \alpha\phi(\alpha)\\
    &= (\alpha - \beta) \phi(\alpha) + \Xi.
\end{align}
We also find that:
\begin{align}
    \pderiv{}{\sigma}\l((\mu - q)\Xi - \sigma\xi) &= (\mu - q)\pderiv{\Xi}{\sigma} - \sigma \pderiv{\xi}{\sigma} - \xi\\
    &= -\beta (-\beta\phi(\beta) + \alpha\phi(\alpha)) - \xi - (\beta^2\phi(\beta)-\alpha^2\phi(\alpha)) \\
    &= (\alpha^2 - \alpha\beta)\phi(\alpha) - \xi.
\end{align}
Also:
\begin{align}
    \pderiv{}{\mu}\frac{p}{1-\Phi(\alpha)} &= \frac{p \pderiv{\Phi(\alpha)}{\mu}}{(1-\Phi(\alpha))^2} \\
    &= -\frac{p \phi(\alpha)}{\sigma(1-\Phi(\alpha))^2}
\end{align}
and:
\begin{align}
    \pderiv{}{\sigma}\frac{p}{1-\Phi(\alpha)} &= \frac{p \pderiv{\Phi(\alpha)}{\sigma}}{(1-\Phi(\alpha))^2} \\
    &= \frac{p (\mu-q)\phi(\alpha)}{\sigma^2(1-\Phi(\alpha))^2}
\end{align}
Hence:
\begin{align*}
    \pderiv{\E_\omega(\pi(q))}{\mu} &= \pderiv{}{\mu}\l(\frac{p}{1-\Phi(\alpha)}\r)\l((\mu - q)\Xi - \sigma\xi\r) + \frac{p}{1-\Phi(\alpha)}\pderiv{}{\mu}\l((\mu - q)\Xi - \sigma\xi\r) \\
    &= \frac{- p \phi(\alpha)}{\sigma(1-\Phi(\alpha))^2}\l((\mu - q)\Xi - \sigma\xi\r) + \frac{p}{1-\Phi(\alpha)}\l((\alpha - \beta)\phi(\alpha) + \Xi\r)\\
    &= \frac{p}{1-\Phi(\alpha)}\l[\frac{\phi(\alpha)}{1-\Phi(\alpha)}\l(\frac{q-\mu}{\sigma}\Xi + \xi\r) + (\alpha - \beta)\phi(\alpha) + \Xi\r]\\
    &= \frac{p}{1-\Phi(\alpha)}\l[ \phi(\alpha)\frac{\beta \Xi + \xi}{1-\Phi(\alpha)} + (\alpha - \beta)\phi(\alpha) + \Xi\r]\\
    &= \frac{p}{1-\Phi(\alpha)}\l[\phi(\alpha)\l(\frac{\beta \Xi + \xi}{1-\Phi(\alpha)} -\frac{q}{\sigma}\r) + \Xi\r] \\
    &= \frac{p\phi(\alpha)}{1-\Phi(\alpha)}\l[\frac{\beta \Xi + \xi}{1-\Phi(\alpha)} -\frac{q}{\sigma} + \frac{\Xi}{\phi(\alpha)}\r]
    % &= \frac{p\phi(\alpha)}{1-\Phi(\alpha)}\l[\frac{(q-\mu)\Xi + \sigma \xi - q(1-\Phi(\alpha))}{\sigma(1-\Phi(\alpha))} + \frac{\Xi}{\phi(\alpha)}\r]\\
    % &= \frac{p\phi(\alpha)}{1-\Phi(\alpha)}\l[\frac{(q-\mu)(\Phi(\beta) - \Phi(\alpha)) + \sigma \xi - q + q\Phi(\alpha)}{\sigma(1-\Phi(\alpha))} + \frac{\Xi}{\phi(\alpha)}\r] \\
    % &= \frac{p\phi(\alpha)}{1-\Phi(\alpha)}\l[\frac{(q-\mu)\Phi(\beta) + \mu\Phi(\alpha) + \sigma \xi - q}{\sigma(1-\Phi(\alpha))} + \frac{\Xi}{\phi(\alpha)}\r]
\end{align*}
\textbf{This should be positive, by common sense. I will start working on proving this but it may be hard.}
Now, since $\Phi$ is increasing and $\beta \ge \alpha$ we have $\Xi \ge 0$ always. We also know that $1-\Phi(\alpha) \ge 0$ and $\phi(\alpha) \ge 0$. The terms that need more study are the first two. We might want to split this based on $\beta > 0$ and $\beta < 0$. \textbf{Can't think of how to show this is positive.}


==> images_tables/Final_Alfares/exceedances.tex <==
\begin{tabular}{lrr}
\toprule
Algorithm &  Number of exceedances &  Max exceedance \\
\midrule
       FD &                      0 &    $9.98\times 10^{-11}$ \\
      PWL &                      4 &    $7.11\times 10^{-15}$ \\
    SLSQP &                    206 &    $6.58\times 10^{-7}$ \\
       TC &                      2 &    $1.78\times 10^{-15}$ \\
\bottomrule
\end{tabular}


==> images_tables/Final_Normal/chi_times_by_T.tex <==
\begin{tabular}{rrll}
\toprule
 $T$ &  Count & Avg. Run Time (CS) & Avg. Run Time (PLA) \\
\midrule
   2 &    320 &            0:00:01 &             0:00:06 \\
   3 &    323 &            0:00:02 &             0:18:20 \\
   4 &    215 &            0:00:01 &             0:01:59 \\
\bottomrule
\end{tabular}


==> images_tables/Final_Normal/worst_case_by_T.tex <==
\begin{tabular}{lrlll}
\toprule
 $T$ &  CS No. & CS Worst-case Count (\%) & PLA No. & PLA Worst-case Count (\%) \\
\midrule
 All &     756 &            635 (83.99\%) &     648 &            648 (100.0\%) \\
   2 &     324 &            274 (84.57\%) &     324 &            324 (100.0\%) \\
   3 &     216 &            183 (84.72\%) &     216 &            216 (100.0\%) \\
   4 &     216 &            178 (82.41\%) &     108 &            108 (100.0\%) \\
\bottomrule
\end{tabular}


==> images_tables/Final_Poisson/worst_case_by_T.tex <==
\begin{tabular}{lrlll}
\toprule
 $T$ &  CS No. & CS Worst-case Count (\%) & PLA No. & PLA Worst-case Count(\%) \\
\midrule
 All &     972 &            972 (100.0\%) &     914 &            914 (100.0\%) \\
   2 &     324 &            324 (100.0\%) &     324 &            324 (100.0\%) \\
   3 &     324 &            324 (100.0\%) &     324 &            324 (100.0\%) \\
   4 &     324 &            324 (100.0\%) &     266 &            266 (100.0\%) \\
\bottomrule
\end{tabular}


==> poisson_continuous_orders.tex <==
\subsection{Objective Function}

In order to evaluate the objective function, we need to evaluate $\E_{\bm{\lambda}}[I^+_t]$ and $\E_{\bm{\lambda}}[I^-_t]$. Recall that:
\begin{align}
    \E_{\bm{\lambda}}[I^+_t] &= \E_{\bm{\lambda}}[\max\{I_t, 0\}] \\
    \E_{\bm{\lambda}}[I^-_t] &= \E_{\bm{\lambda}}[\max\{-I_t, 0\}] 
\end{align}
where $I_t =  \sum_{k=1}^t(q_t - X_t)$, $\P(I_t \ge 0) = \P\l(\sum_{k=1}^t X_k \le \sum_{k=1}^t q_k\r)$ and $\E_{\bm{\lambda}}[I_t|I_t \ge 0] = \sum_{k=1}^t q_k - \E_{\bm{\lambda}}[\sum_{k=1}^t X_k| \sum_{k=1}^t X_k \le \sum_{k=1}^t q_k]$. To simplify notation, let us define $Q_t = \sum_{k=1}^t q_k$ and $\Lambda_t = \sum_{k=1}^t \lambda_k$. Now we have:
\begin{align}
    \P\l(I_t \ge 0\r) &= \P\l(\sum_{k=1}^t X_k \le Q_t\r) \\
    &= \tilde{F}_t\l(Q_t\r) \\
    &= \sum_{x=0}^{\floor{Q_t}} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!}
\end{align}
and similarly we have:
\begin{align}
    \P\l(-I_t \ge 0\r) &= \P\l(I_t \le 0\r)\\
    &= \P\l(Q_t \le \sum_{k=1}^t X_k\r) \\
    &= 1 - \tilde{F}_t(Q_t - 1)\\
    &= 1 - \sum_{x=0}^{\floor{Q_t - 1}} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!},
\end{align}
where $\tilde{f}_t$ and $\tilde{F}_t$ are the PMF and CDF of $\sum_{k=1}^t X_t$. Now, we can calculate the expected values as follows. 
\begin{align}
    \E_{\bm{\lambda}}[\max\{I_t, 0\}] &= \E_{\bm{\lambda}}\l[\max\l\{Q_t - \sum_{k=1}^t X_k, 0\r\}\r] \\
    &= \sum_{x = 0}^{\infty} \max\{Q_t - x, 0\} \tilde{f}_{t}(x) \\
    &= \sum_{x=0}^{\floor{Q_t}} (Q_t - x) \tilde{f}_t(x)\\
    &= Q_t\tilde{F}_t(Q_t) - \sum_{x=0}^{\floor{Q_t}} x \frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x)!} \\
    &= Q_t\tilde{F}_t(Q_t) - \sum_{x=1}^{\floor{Q_t}}  \frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x-1)!} \\
    &= Q_t \tilde{F}_t(Q_t) - \Lambda_t\sum_{x=1}^{\floor{Q_t}}  \frac{(\Lambda_t)^{x-1}\exp{(-\Lambda_t)}}{(x-1)!} \\
    &= Q_t \tilde{F}_t(Q_t) - \Lambda_t\tilde{F}_t(Q_t-1).
\end{align}
Similarly:
\begin{align}
    \E_{\bm{\lambda}}[\max\{-I_t, 0\}] &= \sum_{x = 0}^{\infty} \max\{x - Q_t, 0\} \tilde{f}_{t}(x) \\
    &= \sum_{x=\ceil{Q_t}}^{\infty}(x-Q_t)\tilde{f}_t(x) \\
    &= -Q_t(1-\tilde{F}_t(Q_t)) + \sum_{x=\ceil{Q_t}}^{\infty} x\frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x)!}\\
    &= -Q_t(1-\tilde{F}_t(Q_t - 1)) + \Lambda_t - \sum_{x=0}^{\floor{Q_t} - 1} x\frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x)!}\\
    &= -Q_t(1-\tilde{F}_t(Q_t - 1)) + \Lambda_t - \sum_{x=1}^{\floor{Q_t} - 1} \frac{(\Lambda_t)^{x}\exp{(-\Lambda_t)}}{(x-1)!}\\
    &= -Q_t(1-\tilde{F}_t(Q_t - 1)) +  \Lambda_t(1-\tilde{F}_t(Q_t-2)). 
\end{align}


% \begin{align}
%     \E[X|X>a] &= \frac{\sum_{x=a+1}^{\infty} xf_X(x)}{1 - F_X(a)} \\
%     \E[X|X<a] &= \frac{\sum_{x=0}^{a-1} xf_X(x)}{F_X(a -1)}
% \end{align}
% Then we have:
% \begin{align}
%     \E_{\bm{\lambda}}[I_t|I_t \ge 0] &= Q_t - \E_{\bm{\lambda}}\l[\sum_{k=1}^t X_k \bigg| \sum_{k=1}^t X_k \le Q_t\r]\\
%     &= Q_t - \frac{\sum_{x=0}^{\floor{Q_t}} x \frac{\exp\l(\Lambda_t\r)\l(\Lambda_t\r)^x}{x!}}{\sum_{x=0}^{\floor{Q_t}}\frac{\exp\l(\Lambda_t\r)\l(\Lambda_t\r)^{x}}{x!}} \\
%     &= Q_t - \frac{\sum_{x=1}^{\floor{Q_t}}{\frac{\exp(-\Lambda_t)(\Lambda_t)^x}{(x-1)!}}}{\sum_{x=0}^{\floor{Q_t}}\frac{\exp\l(\Lambda_t\r)\l(\Lambda_t\r)^{x}}{x!}} \\
%     &= Q_t - \Lambda_t\frac{\sum_{x=0}^{\floor{Q_t - 1}} \frac{\exp(-\Lambda_t) (\Lambda_t)^{x}}{x!}}{\sum_{x=0}^{\floor{Q_t}}\frac{\exp\l(\Lambda_t\r)\l(\Lambda_t\r)^{x}}{x!}}\\
%     &= Q_t - \Lambda_t\frac{\tilde{F}_t(Q_t - 1)}{\tilde{F}_t(Q_t)}.
%     % &= Q_t - \sum_{x=0}^{\floor{Q_t - 1}} \frac{x (\Lambda_t)^{x - (Q_t - 1)}(Q_t - 1)!}{x!} \\
%     % &= Q_t - \sum_{x=1}^{Q_t - 1} \l(\Lambda_t\r)^{x - (Q_t - 1)}\frac{(Q_t - 1)!}{(x-1)!} \\
%     % &= Q_t - \sum_{x=1}^{Q_t - 1} \l(\Lambda_t\r)^{x - (Q_t - 1)}\prod_{y=x}^{Q_t - 1} y.
% \end{align}
% % With $K_t = \prod_{y=x}^{Q_t - 1} y$, we have:
% % \begin{equation}
% %     \E_{\bm{\lambda}}[I^+_t] = Q_t - \sum_{x=1}^{Q_t - 1}K_t \l(\Lambda_t\r)^{x - (Q_t - 1)}.
% % \end{equation}
% Moving on to $\E_{\bm{\lambda}}[I^-_t]$, we have:
% \begin{align}
%     \E_{\bm{\lambda}}[-I_t|I_t \le 0] &= - \E_{\bm{\lambda}}[I_t|I_t \le 0] \\
%     &= - \l(Q_t - \E_{\bm{\lambda}}\l[\sum_{k=1}^t X_k \bigg| \sum_{k=1}^t X_k \ge Q_t\r]\r)\\
%     &=  - Q_t + \frac{\sum_{x=Q_t}^{\infty} x \frac{\exp(-\Lambda_t)(\Lambda_t)^x}{x!}}{1-\sum_{x=0}^{\floor{Q_t - 1}}  \frac{\exp(-\Lambda_t)(\Lambda_t)^x}{x!}}\\
%     &=  - Q_t + \frac{\Lambda_t - \sum_{x=1}^{Q_t-1} \frac{\exp(-\Lambda_t)(\Lambda_t)^x}{(x-1)!}}{1-\sum_{x=0}^{\floor{Q_t - 1}}  \frac{\exp(-\Lambda_t)(\Lambda_t)^x}{x!}}\\
%     &=  - Q_t + \frac{\Lambda_t - \Lambda_t\sum_{x=1}^{Q_t-1} \frac{\exp(-\Lambda_t)(\Lambda_t)^{x-1}}{(x-1)!}}{1-\sum_{x=0}^{\floor{Q_t - 1}}  \frac{\exp(-\Lambda_t)(\Lambda_t)^x}{x!}}\\
%     &=  - Q_t + \Lambda_t\frac{1-\sum_{x=0}^{Q_t - 2} \frac{\exp(-\Lambda_t)(\Lambda_t)^{x}}{(x)!}}{1-\sum_{x=0}^{\floor{Q_t - 1}}  \frac{\exp(-\Lambda_t)(\Lambda_t)^x}{x!}}\\
%     &= - Q_t + \Lambda_t \frac{1 - \tilde{F}_t(Q_t - 2)}{1 - \tilde{F}_t(Q_t - 1)}.
% \end{align}
% Hence, combining these results, we have:
% Therefore, we have:
% \begin{align}
%     \E_{\bm{\lambda}}[I^+_t] &= \P(I_t \ge 0)\E_{\bm{\lambda}}[I_t|I_t \ge 0]\\
%     &= \tilde{F}_t(Q_t)\l[Q_t - \Lambda_t\frac{\tilde{F}_t(Q_t - 1)}{\tilde{F}_t(Q_t)}\r]\\
%     &= \tilde{F}_t(Q_t)Q_t - \Lambda_t\tilde{F}_t(Q_t-1).
% \end{align}
% We also have:
% \begin{align}
%     \E_{\bm{\lambda}}[I^-_t] &= \P(-I_t \ge 0)\E_{\bm{\lambda}}[-I_t|-I_t \ge 0]\\
%     &= (1-\tilde{F}_t(Q_t -1))\l[- Q_t + \Lambda_t \frac{1 - \tilde{F}_t(Q_t - 2)}{1 - \tilde{F}_t(Q_t - 1)}\r]\\
%     &= \Lambda_t(1-\tilde{F}_t(Q_t-2)) - Q_t(1 - \tilde{F}_t(Q_t - 1).
% \end{align}
This gives the following objective function (with $a_t = b +
p\mathds{1}\{t=T\} + h$):
\begin{align}
    C_{\bm{\lambda}}(\bm{q}) &= p\E_{\bm{\lambda}}[I^-_T] +  \sum_{t=1}^T(h \E_{\bm{\lambda}}[I^+_t] +  b\E_{\bm{\lambda}}[I^-_t] + w_t q_t - p \E_{\bm{\lambda}}[X_t]) \\
    &= \sum_{t=1}^T(h \E_{\bm{\lambda}}[I^+_t] +  (b + p\mathds{1}\{t=T\})\E_{\bm{\lambda}}[I^-_t] + w_t q_t - p \E_{\bm{\lambda}}[X_t]) \\
    &= \sum_{t=1}^T\l(h(Q_t \tilde{F}_t(Q_t) - \Lambda_t\tilde{F}_t(Q_t-1)) + (a_t - h)\l(-Q_t(1-\tilde{F}_t(Q_t - 1)) +   \r.\r.\nonumber \\
    &\quad \l.\l. +  \Lambda_t(1-\tilde{F}_t(Q_t-2))\r) + q_tw_t - p \lambda_t\r) \\
    &= \sum_{t=1}^T\l(h Q_t \tilde{F}_t(Q_t) + ((a_t - h) Q_t - h\Lambda_t)\tilde{F}_t(Q_t-1)  - \Lambda_t(a_t-h) \tilde{F}_t(Q_t-2) \r. \nonumber\\ 
    & \quad \l. + (a_t - h)(\Lambda_t - Q_t) + q_tw_t- p \lambda_t\r) 
\end{align}

\subsection{Derivatives of Objective Function}

In order to select the worst-case $\bm{\lambda}$, we differentiate the objective function. We have that:
\begin{align}
    \pderiv{\tilde{F}_t(Q_t)}{\lambda_k} &=  \pderiv{}{\lambda_k}\l(\sum_{x=0}^{\floor{Q_t}} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!}\r)\\
    &= \sum_{x=0}^{\floor{Q_t}} \frac{-\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x + \exp\l(-\Lambda_t\r)x\l(\Lambda_t\r)^{x-1}}{x!}\\
    &= \sum_{x=1}^{\floor{Q_t}}\frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^{x-1}}{(x-1)!} - \sum_{x=0}^{\floor{Q_t}} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!} \\
    &= \sum_{x=0}^{\floor{Q_t - 1}}\frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^{x}}{x!} - \sum_{x=0}^{\floor{Q_t}} \frac{\exp\l(-\Lambda_t\r)\l(\Lambda_t\r)^x}{x!} \\
    &= - \frac{\exp(-\Lambda_t)(\Lambda_t)^{\floor{Q_t}}}{\floor{Q_t}!}\\
    &= -\tilde{f}_t(\floor{Q_t})
\end{align}
for $k \le t$. Similarly,
\begin{equation}
    \pderiv{\tilde{F}_t(Q_t - 1)}{\lambda_k} =  -\tilde{f}_t(\floor{Q_t}-1) \quad (k \le t).
\end{equation}
Hence, we have:
% \begin{align}
%     \pderiv{C_{\bm{\lambda}}(\bm{q})}{\lambda_k} &= \sum_{t=k}^T\l(
%         -Q_ta_t\tilde{f}_t(Q_t) - a_t\tilde{F}_t(Q_t-1) + \Lambda_t a_t \tilde{f}_t(Q_t - 1) + b+p\mathds{1}\{t=T\}
%     -p\r) \\
%     &= \sum_{t=k}^T\l(b+p\mathds{1}\{t=T\} - a_t \tilde{F}_t(Q_t-1) - p\r)
% \end{align}
\begin{align}
    \pderiv{C_{\bm{\lambda}}(\bm{q})}{\lambda_k} &= \sum_{t=k}^T\l(
        -Q_t h \tilde{f}_t(\floor{Q_t}) - ((a_t - h)Q_t - h\Lambda_t) \tilde{f}_t(\floor{Q_t}-1) - h\tilde{F}_t(Q_t-1) \r. \nonumber\\
        & \quad \l. + \Lambda_t (a_t - h)\tilde{f}_t(\floor{Q_t} - 2) - (a_t - h)\tilde{F}_t(Q_t-2) + (a_t - h)
    -p\r) \\
    &=  \sum_{t=k}^T\l(
        -\l(\frac{Q_t h \Lambda_t}{\floor{Q_t}} + ((a_t - h)Q_t - h\Lambda_t)\r) \tilde{f}_t(\floor{Q_t} - 1) - h(\tilde{F}_t(Q_t-1) - \tilde{F}_t(Q_t-2)) \r. \nonumber\\
        & \quad \l. + \floor{Q_t-1} (a_t - h)\tilde{f}_t(\floor{Q_t} - 1) - a_t\tilde{F}_t(Q_t-2) + (a_t - h)
    -p\r) \\
    &= \sum_{t=k}^T\l(
        \l(\floor{Q_t-1} (a_t - h)-\frac{Q_t h \Lambda_t}{\floor{Q_t}} - ((a_t - h)Q_t - h\Lambda_t) - h\r) \tilde{f}_t(\floor{Q_t} - 1) \r. \nonumber\\
        & \quad \l. - a_t\tilde{F}_t(Q_t-2) + (a_t - h)
    -p\r) \\
    &= \sum_{t=k}^T\l(
        \l((a_t - h)(\floor{Q_t-1} - Q_t)- h\l(\frac{Q_t\Lambda_t}{\floor{Q_t}} + \Lambda_t + Q_t + 1\r)\r) \tilde{f}_t(\floor{Q_t} - 1) \r. \nonumber\\
        & \quad \l. - a_t\tilde{F}_t(Q_t-2) + (a_t - h)
    -p\r) \\
\end{align}
This does not immediately suggest monotonicity. We have:
\begin{align}
    \frac{\partial^2 C_{\bm{\lambda}}(\bm{q})}{\partial \lambda^2_k} &= \sum_{t=k}^T -h\l(\frac{Q_t}{\floor{Q_t}} + 1\r)\tilde{f}_t(\floor{Q_t} - 1)  \\
    &\ge 0 \fa k = 1,\dots,T.
\end{align}
Therefore, the objective function is convex in $\lambda_k$ for each $k$. Hence, the worst-case $\lambda_k$ will either be the smallest in the ambiguity set or the largest (when all other $\lambda_j$ are fixed).  
